Active-Dormant Attention Heads: Mechanistically Demystifying Extreme-Token Phenomena in LLMs

Practitioners have consistently observed three puzzling phenomena in transformer-based large language models (LLMs): attention sinks, value-state drains, and residual-state peaks, collectively referred to as extreme-token phenomena. These phenomena are characterized by certain so-called "sink tokens" receiving disproportionately high attention weights, exhibiting significantly smaller value states, and having much larger residual-state norms than those of other tokens. These extreme tokens give rise to various challenges in LLM inference, quantization, and interpretability. We elucidate the mechanisms behind extreme-token phenomena. First, we show that these phenomena arise in very simple architectures -- transformers with one to three layers -- trained on a toy model, the Bigram-Backcopy (BB) task. In this setting, we identify an active-dormant mechanism, where attention heads become sinks for specific input domains while remaining non-sinks for others. Our theoretical analysis of the training dynamics reveals that these phenomena are driven by a mutual reinforcement mechanism. Building on these insights, we propose strategies to mitigate extreme-token phenomena during pretraining, including replacing softmax with ReLU and Adam with SGD. Next, we extend our analysis to pretrained LLMs, including Llama and OLMo, showing that many attention heads exhibit a similar active-dormant mechanism as in the BB task, and that the mutual reinforcement mechanism also governs the emergence of extreme-token phenomena during LLM pretraining. Our results reveal that many of the static and dynamic properties of extreme-token phenomena predicted by the BB task align with observations in pretrained LLMs.

==> Sections/appendices/supporting_results.tex <==
\section{Supporting Results}

% In this appendix, we provide more supporting evidence for our conjecture in \Cref{sec:dormant_heads}.


% \subsection{Supporting Results for \Cref{sub:circuit_evidence}} \label{sub:app_supporting_circuit}


\begin{figure}[t]
  \centering
  \begin{minipage}{0.24\textwidth}
      \centering
      \subcaption{\small lower layers on \bos}
      \label{fig:appendix-ablation-bos-lower}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/bos_lower.pdf}
  \end{minipage}~
  % \hspace{-1em}
  \begin{minipage}{0.24\textwidth}
      \centering
      \subcaption{\small upper layers on \bos}
      \label{fig:appendix-ablation-bos-upper}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/bos_upper.pdf}
  \end{minipage}~
  % \hspace{-1em}
  \begin{minipage}{0.24\textwidth}
      \centering
      \subcaption{\small lower layers on \delim}
      \label{fig:appendix-ablation-delim-lower}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/delim_lower.pdf}
  \end{minipage}~
  % \vspace{-1em}
    \begin{minipage}{0.24\textwidth}
      \centering
      \subcaption{\small upper layers on \delim}
      \label{fig:appendix-ablation-delim-lower}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/delim_upper.pdf}
  \end{minipage}~
  
  \caption{\small The effect of $\MLP$ and $\Attn$ of lower and upper two layers on the norm of \bos and \delim.}
  \label{figure:appendix-ablation-massive-sup-control}
  % \vspace{-1em}
\end{figure}


\begin{figure}[t]
  \centering
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Ablations on layer $0$}
      \label{fig:appendix-ablation-massive-sup-control-0}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/bos_control/bos_massive_sup_L0.pdf}
  \end{minipage}~
  % \hspace{-1em}
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Ablations on layer $1$}
      \label{fig:appendix-ablation-massive-sup-control-1}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/bos_control/bos_massive_sup_L1.pdf}
  \end{minipage}~
  % \hspace{-1em}
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Ablations on entire layer $0$}
      \label{fig:appendix-ablation-massive-sup-control-attn}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/bos_control/L0_intervention_attn_weights.pdf}
  \end{minipage}~
  % \vspace{-1em}
  
  \caption{\small Ablations using control sample
  }
  \label{figure:appendix-ablation-massive-sup-control}
  % \vspace{-1em}
\end{figure}

\begin{figure}[t]
  \centering
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Ablations on layer $0$}
      \label{fig:appendix-ablation-massive-sup-zero-0}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/bos_zero_out/bos_massive_L0.pdf}
  \end{minipage}~
  % \hspace{-1em}
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Ablations on layer $1$}
      \label{fig:appendix-ablation-massive-sup-zero-1}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/bos_zero_out/bos_massive_L1.pdf}
  \end{minipage}~
  % \hspace{-1em}
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Ablations on entire layer $0$}
      \label{fig:appendix-ablation-massive-sup-zero-attn}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/bos_zero_out/L0_zero_attn_weights.pdf}
  \end{minipage}~
  % \vspace{-1em}
  
  \caption{\small Ablations using zeroing-out
  }
  \label{figure:appendix-ablation-massive-zero}
  % \vspace{-1em}
\end{figure}

\begin{figure}[t]
  \centering
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Ablations on layer $0$}
      \label{fig:appendix-ablation-delim-0}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/delim_no_rope/delim_massive_suppression_L0.pdf}
  \end{minipage}~
  % \hspace{-1em}
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Ablations on layer $1$}
      \label{fig:appendix-ablation-delim-1}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/delim_no_rope/delim_massive_suppression_L1.pdf}
  \end{minipage}~
  % \hspace{-1em}
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Ablations on entire layer $0$}
      \label{fig:appendix-ablation-delim-attn}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/delim_no_rope/L0_no_rope_attn_weights.pdf}
  \end{minipage}~
  % \vspace{-1em}
  
  \caption{\small Ablations using no \rope
  }
  \label{figure:appendix-ablation-delim}
  % \vspace{-1em}
\end{figure}


\subsection{Supporting Results for \Cref{sub:lots_of_dormant_heads}} \label{sub:app_supporting_lots_of_heads}


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Figures/L16_H25/attn_maps_l16h25_wiki.pdf}
    \includegraphics[width=\textwidth]{Figures/L16_H25/attn_maps_l16h25_github.pdf}
    \caption{\small\textbf{Visualizations of attention weights for Llama 2 7B Layer 16 Head 25 on both Wikipedia and GitHub data.} A continuation of \Cref{fig:attn_l16_h25_small}.}
    \label{fig:attn_l16_h25_improved}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Figures/L16_H25/attn_logits_l16h25_wiki.pdf}
    \includegraphics[width=\textwidth]{Figures/L16_H25/attn_logits_l16h25_github.pdf}
    \caption{\small\textbf{Visualizations of pre-softmax attention logits for Llama 2 7B Layer 16 Head 25 on both Wikipedia and GitHub data.} A continuation of \Cref{fig:attn_logits_l16_h25_small}.}
    \label{fig:attn_logits_l16_h25_improved}
\end{figure}

\subsection{Supporting Results for \Cref{sub:controlled_experiments}} \label{sub:app_supporting_controlled}

\subsection{Task in \citet{bietti2024birth}}
\begin{figure}[t]
  \centering
  \begin{minipage}{0.4\textwidth}
      \centering
      \subcaption{\small Data generating procedure}
      \label{fig:appendix-pretraining-dgp}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/Biette.pdf}
  \end{minipage}
  \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Layer 0 on dormant sequence}
      \label{fig:appendix-biette-attn-weights-dormant-l0}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/Biette_attn_weights_seq0_layer0.pdf}
  \end{minipage}
  \hspace{-1em}
    \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Layer 1 on dormant sequence}
      \label{fig:appendix-biette-attn-weights-dormant-l1}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/Biette_attn_weights_seq0_layer1.pdf}
  \end{minipage}
  \vspace{-1em}
  \caption{\small Using the task in \citet{bietti2024birth}}
  \label{figure:appendix-pretraining-biette-findings}
  \vspace{-1em}
\end{figure}

\begin{figure}
\centering
  \begin{minipage}{0.45\textwidth}
      \centering
      \subcaption{\small Layer 0 on active sequence}
      \label{fig:appendix-biette-attn-weights-active-l0}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/Biette_attn_weights_seq1_layer0.pdf}
  \end{minipage}
  \hspace{-1em}
    \begin{minipage}{0.45\textwidth}
      \centering
      \subcaption{\small Layer 1 on active sequence}
      \label{fig:appendix-biette-attn-weights-active-l1}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/Biette_attn_weights_seq1_layer1.pdf}
  \end{minipage}
  \vspace{-1em}
  \caption{\small Using the task in \citet{bietti2024birth}}
  \label{figure:appendix-pretraining-biette-findings-1}
  \vspace{-1em}
\end{figure}

\begin{figure}
      \centering
  \begin{minipage}{0.45\textwidth}
      \centering
      \subcaption{\small Output norm on layer 1}
      \label{fig:appendix-biette-massive}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/Biette/Biette_L3_massive.pdf}
  \end{minipage}
  \hspace{-1em}
    \begin{minipage}{0.45\textwidth}
      \centering
      \subcaption{\small Value state norm on layer 2}
      \label{fig:appendix-biette-minor}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/Biette/Biette_L3_minor.pdf}
  \end{minipage}
  \vspace{-1em}
  \caption{\small Using the task in \citet{bietti2024birth}}
  \label{figure:appendix-pretraining-biette-findings-3}
  \vspace{-1em}
\end{figure}

\subsection{The ``dormant Markov task''}
\begin{figure}[t]
  \centering
  \begin{minipage}{0.4\textwidth}
      \centering
      \subcaption{\small Data generating procedure}
      \label{fig:appendix-pretraining-dgp-dormant-markov}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_markov.pdf}
  \end{minipage}
  \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Layer 0 on dormant sequence}
      \label{fig:appendix-dormant-markov-attn-weights-dormant}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_markov/dormant_markov_attn_weights_seq0.pdf}
  \end{minipage}
  \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Layer 0 on active sequence}
      \label{fig:appendix-dormant-markov-attn-weights-active}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_markov/dormant_markov_attn_weights_seq1.pdf}
  \end{minipage}
  \vspace{-1em}
  \caption{\small Dormant markov task}
  \label{figure:appendix-pretraining-dormant-markov-1}
  \vspace{-1em}
\end{figure}

\begin{figure}
      \centering
  \begin{minipage}{0.45\textwidth}
      \centering
      \subcaption{\small Output norm on layer 1}
      \label{fig:appendix-dormant-markov-massive}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_markov/dormant_markov_L3_massive.pdf}
  \end{minipage}
  \hspace{-1em}
    \begin{minipage}{0.45\textwidth}
      \centering
      \subcaption{\small Value state norm on layer 2}
      \label{fig:appendix-dormant-markov-minor}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_markov/dormant_markov_L3_minor.pdf}
  \end{minipage}
  \vspace{-1em}
  \caption{\small Dormant markov task}
  \label{figure:appendix-pretraining-dormant-markov-findings-2}
  \vspace{-1em}
\end{figure}

==> Sections/appendices/tmp.tex <==
\frac{\partial \log\Big[\sum_{\toki=1}^\vocabsize \transition^\tokksup_\toki\exp\Big[\frac{W^\tokisup\beta^\tokisup+e^{\sink_j}\ivalue_\toki}{e^{\sink_j}+W}\Big]\Big]}{\partial \ivalue_\tok} = &~ \frac{e^{\sink_j}}{e^{\sink_j}+W} \cdot \frac{  \transition^\tokksup_\tok \exp\Big[\frac{W^\tokksup\beta^\tokksup+e^{\sink_j}\ivalue_\tok}{e^{\sink_j}+W}\Big]}{\sum_{\toki=1}^\vocabsize \transition^\toksup_\toki\exp\Big[\frac{W^\tokisup\beta^\tokisup+e^{\sink_j}\ivalue_\toki}{e^{\sink_j}+W}\Big]}\label{eqn:ds-part1} \\
\frac{\partial 

==> Sections/deprecated_sections/applications.tex <==
\section{Applications}

% \begin{itemize}
%     % \item Speed up attention computation by by-passing softmax partition function?~\yub{first step: check whether decoding is still exactly correct on large corpus.}
% \end{itemize}

==> Sections/deprecated_sections/case_study.tex <==
\section{Case Study and Motivation}\label{sec:case_study}

In this section, we will study a particular attention head in Llama 2, and use its behavior as a motivation for the more general analysis that follows.

\subsection{Preliminaries}\label{sub:prelim}

\DP{TODO @TG: Fill out a simplified notation block. Please ensure that the simplified notation is consistent with the notation in the appendix.}

\DP{TODO: mention that we pre-pend all inputs with \bos.}

A significantly more precise setup and notation is detailed in \Cref{sub:app_notation}.

\subsection{Understanding Layer 16 Attention Head 25 of Llama 2}\label{sub:case_study_l25_h16}

As motivation for our later reasoning, we will now examine the behavior of Layer 16 Attention Head 25 (abbreviated as L16H25) in Llama 2 7B, on both prose from the Wikipedia dataset \citep{wikidump} and code from the RedPajama Github dataset \citep{together2023redpajama}. This is the first attention head which we identify as a dormant head, and we want to understand its properties at a more fine-grained level. First, let us examine the difference in perplexity on samples of these two datasets obtained from the full forward pass versus a modified forward pass where the output of the attention head L16H25 is zeroed out. Specifically, we evaluate each forward pass on 32 samples of their respective datasets, where each sample is truncated to 64 tokens. We observe the results in \Cref{tab:ppl_wiki_github_l16h25}. Overall, the performance change is greater on the GitHub data than on the Wikipedia data, which signals that it may be the case that L16H25 is function-less on the Wikipedia data yet has a function on the GitHub data. To confirm our hypothesis, we plot the (post-softmax) attention weights on a few representative samples of GitHub and Wikipedia data in \Cref{fig:attn_l16_h25_small} (and \Cref{fig:attn_l16_h25_improved} in \Cref{sub:app_supporting_lots_of_heads}). We observe that L16H25 is an attention sink \citep{xiao2023efficient} on Wikipedia data. This means that for each sample, the attention head outputs roughly the same vector (or one of a few possible vectors) for each token position, acting like a bias which does not use correlations between tokens. On the other hand, on GitHub data L16H25 is not an attention sink. This discrepancy motivates the definition of a dormant head, expanded on in \Cref{sec:dormant_heads}, that a dormant head is one which does not use correlations between tokens to obtain an output (and thus is not impacted by the semantics of the input). To confirm this, we also plot the pre-softmax logits in \Cref{fig:attn_logits_l16_h25_small} (and \Cref{fig:attn_logits_l16_h25_improved} in \Cref{sub:app_supporting_lots_of_heads}). \DP{TODO: @TG could you give some reasoning here?}

\begin{table}
    \centering
    \caption{\small \textbf{Perplexity of Llama 2 7B when using an unmodified forward pass vs.~a forward pass which is modified to set the output of L16H25 to \(0\).} We observe that while the perplexity does not change substantially on Wikipedia data, it noticeably increases on Github data. This motivates the hypothesis that L16H25 is ``dormant'' for Wikipedia data and ``active'' for Wikipedia data.}
    \begin{tabular}{@{}lll@{}}
    \toprule
    \textbf{Perplexity}    & Wikipedia Dataset & Github Dataset \\ \midrule
    Unmodified forward pass                  &                   &                \\
    Modified forward pass  &                   &                \\ \bottomrule
    \end{tabular} 
    \label{tab:ppl_wiki_github_l16h25}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/L16_H25/attn_maps_l16h25_wiki_small.pdf}
    \hspace{0.075\textwidth}
    \includegraphics[width=0.45\textwidth]{Figures/L16_H25/attn_maps_l16h25_github_small.pdf}
    \caption{\small\textbf{Visualizations of attention weights for Llama 2 7B L16H25 on both Wikipedia and GitHub data.} On four random samples from each domain, we truncate each sample to 64 tokens and visualize the (post-softmax) attention weights from this head. We observe that for Wikipedia the head has one or two attention sinks, while for GitHub the head has no attention sink, corresponding to our hypothesis that the head is ``dormant'' on Wikipedia and ``active'' on GitHub. Further samples are plotted in \Cref{fig:attn_l16_h25_improved}, maintaining this trend.}
    \label{fig:attn_l16_h25_small}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/L16_H25/attn_logits_l16h25_wiki_small.pdf}
    \hspace{0.075\textwidth}
    \includegraphics[width=0.45\textwidth]{Figures/L16_H25/attn_logits_l16h25_github_small.pdf}
    \caption{\small\textbf{Visualizations of pre-softmax attention logits for Llama 2 7B L16H25 on both Wikipedia and GitHub data.} \DP{@TG: please fill in the description here and in main body.} Further samples are plotted in \Cref{fig:attn_logits_l16_h25_improved}, maintaining this trend. \tianyu{how about deleting this figure? It's hard to tell that the logits are around the same. Instead, how about make annotations on previous figure, showing the attention logits on bos?}}
    \label{fig:attn_logits_l16_h25_small}
\end{figure}



==> Sections/deprecated_sections/compression_results.tex <==
\DP{write intro for this}

Causal compression algorithm: at sequence index \(t\) with final index \(T\), threshold out all but \(\approx \frac{1}{2}t\) or \(\frac{1}{10}t\) tokens. Non-causal compression algorithm: threshold out all but \(\approx \frac{1}{2}T\) or \(\frac{1}{10}T\) tokens. When \(T \gg t\) (i.e., infinite-streaming contexts), the former is more restrictive than the latter, and also may scale much better.

For all tasks we report the raw zero-shot accuracy as computed by EleutherAI's evaluation harness \citep{eval-harness}, at this \href{https://github.com/EleutherAI/lm-evaluation-harness/tree/cffc1bd3fd69453eaa75da891256682123226f0f}{permalink}.

\begin{table}[H]
    \centering
    \resizebox{0.99\textwidth}{!}{
        \begin{tabular}{@{}llllllllll@{}}
        \toprule
        Model     & Compression Scheme                          & Compression Ratio & ARC-C & ARC-E & HellaSwag & LAMBADA & OpenBookQA & PIQA  & Winogrande \\ \midrule
        Llama2-7B & No Compression                              & N/A               & 0.434 & 0.763 & 0.571     & 0.683   & 0.314      & 0.781 & 0.691      \\
                  & Adaptive Per-Layer Compression              & 50\%              & 0.435 & 0.763 & 0.571     & 0.683   & 0.314      & 0.781 & 0.691      \\
                  &                                             & 90\%              & 0.431 & 0.746 & 0.572     & 0.679   & 0.272      & 0.772 & 0.698      \\
                  & Adaptive Per-Head Compression               & 50\%              & 0.434 & 0.763 & 0.571     & 0.683   & 0.314      & 0.781 & 0.691      \\
                  &                                             & 90\%              & 0.416 & 0.734 & 0.567     & 0.681   & 0.28       & 0.766 & 0.706      \\
                  & Adaptive Per-Query-Token Causal Compression & 50\%              & 0.437 & 0.761 & 0.571     & 0.681   & 0.312      & 0.780 & 0.691      \\
                  &                                             & 90\%              & 0.404 & 0.720 & 0.546     & 0.643   & 0.268      & 0.763 & 0.658      \\ \bottomrule
        \end{tabular}
    }
    \caption{\textbf{Comparison of our attention head compression methods on zero-shot accuracy on standard benchmarks.} We observe that all compression methods preserve the performance of the base Llama2 model. The Per-Query-Token Causal Compression method performs the worst with 90\% of tokens compressed, but still preserves most of the performance and scales the best.}
    \label{tab:comparing_our_different_compression_methods}
\end{table}


\begin{table}[H]
    \centering
    \resizebox{0.99\textwidth}{!}{
        \begin{tabular}{@{}llllllllll@{}}
            \toprule
            Model     & Compression Scheme                          & Compression Ratio & ARC-C & ARC-E & HellaSwag & LAMBADA & OpenBookQA & PIQA  & Winogrande \\ \midrule \midrule
            Llama2-7B & No Compression                              & N/A               & 0.434 & 0.763 & 0.571     & 0.683   & 0.314      & 0.781 & 0.691      \\
                      & StreamingLLM Compression                    & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\
                      & StreamingLLM Causal Compression             & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\
                      & Adaptive Per-Query-Token Causal Compression & 50\%              & 0.437 & 0.761 & 0.571     & 0.681   & 0.312      & 0.780 & 0.691      \\
                      &                                             & 90\%              & 0.404 & 0.720 & 0.546     & 0.643   & 0.268      & 0.763 & 0.658      \\ \midrule
            Mistral-7B& No Compression                              & N/A               &       &       &           &         &            &       &            \\
                      & StreamingLLM Compression                    & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\
                      & StreamingLLM Causal Compression             & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\
                      & Adaptive Per-Query-Token Causal Compression & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\ \midrule
            Gemma-7B  & No Compression                              & N/A               &       &       &           &         &            &       &            \\
                      & StreamingLLM Compression                    & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\
                      & StreamingLLM Causal Compression             & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\
                      & Adaptive Per-Query-Token Causal Compression & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\ \midrule
            Pythia-7B & No Compression                              & N/A               &       &       &           &         &            &       &            \\
                      & StreamingLLM Compression                    & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\
                      & StreamingLLM Causal Compression             & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\
                      & Adaptive Per-Query-Token Causal Compression & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\ \bottomrule
        \end{tabular}
    }
    \caption{\textbf{Comparison of our adaptive causal attention compression algorithm against the previous one posed by StreamingLLM \citep{xiao2023efficient} on zero-shot accuracy on standard benchmarks.} We observe that our method succeeds most of the time in retaining performance, at least on these benchmarks, much better than StreamingLLM. This holds even if we do not force their mechanism to be causal.}
    \label{tab:compare_ours_streamingllm_zeroshot}
\end{table}



We also evaluate their perplexity on LAMBADA and the first row of the PG19 dataset (an extremely long document), chunked into \DP{INSERT HERE} subsets of \DP{INSERT HERE} contiguous tokens over which the perplexity is averaged.

\begin{table}[H]
    \centering
    \resizebox{0.99\textwidth}{!}{
        \begin{tabular}{@{}lllll@{}}
            \toprule
            Model     & Compression Scheme                          & Compression Ratio & LAMBADA Perplexity & PG19 Document 1 Perplexity \\ \midrule
            Llama2-7B & No Compression                              & N/A               & 4.13               &                            \\
                      & StreamingLLM Compression                    & 50\%              &                    &                            \\
                      &                                             & 90\%              &                    &                            \\
                      & StreamingLLM Causal Compression             & 50\%              &                    &                            \\
                      &                                             & 90\%              &                    &                            \\
                      & Adaptive Per-Layer Compression              & 50\%              & 4.12               &                            \\
                      &                                             & 90\%              & 4.16               &                            \\
                      & Adaptive Per-Head Compression               & 50\%              & 4.13               &                            \\
                      &                                             & 90\%              & 4.19               &                            \\
                      & Adaptive Per-Query-Token Causal Compression & 50\%              & 4.14               &                            \\
                      &                                             & 90\%              & 5.06               &                            \\ \bottomrule
        \end{tabular}
    }
    \caption{\textbf{Comparison of our attention-head compression algorithms against the previous one posed by StreamingLLM \citep{xiao2023efficient} on average perplexity on the LAMBADA task and the first document of the PG19 dataset.} We observe that our adaptive methods generally maintain significantly better perplexity than the previous StreamingLLM-derived methods on both short and long contexts.}
    \label{tab:compare_ourrs_streamingllm_ppl}
\end{table}

==> Sections/deprecated_sections/dormant_heads.tex <==
\section{Dormant Attention Heads}\label{sec:dormant_heads}
 
 In this section, we will more carefully define dormant heads and show that they are ubiquitous on both pre-trained LLMs and small transformers trained via next-token-prediction.

\subsection{Dormant Head Conjecture} \label{sub:dormant_head_conjecture}

As in \Cref{sub:case_study_l25_h16}, we define a \textit{dormant attention head} as follows.
\begin{quote}
    \textit{An attention head is \underline{dormant} on a particular input if its output consists of only one (or a small number of) vector(s), repeated across every token index.}
\end{quote}
 The output of a dormant head does not respect the semantic content of the input, and essentially outputs a bias. Heads which are attention sinks are dormant attention heads, and indeed almost all (but not necessarily all) dormant attention heads are attention sinks. Our \textit{dormant heads conjecture} states that dormant heads are ubiquitous in LLMs. In particular, we say that a head which is not dormant is \textit{active}. Then, we conjecture the following:
 \begin{quote}
     \textit{\underline{Dormant heads conjecture:} for autoregressive transformer-based language models, a large fraction of heads are dormant on some inputs and active on some others.}
 \end{quote}
 In this section, we will provide evidence for this conjecture through finding a circuit in Llama 2 7B which creates dormant heads (\Cref{sub:circuit_evidence}), developing an automated detection system for attention sinks and thus showing that many heads in Llama 2 7B are empirically dormant on some inputs and active on others (\Cref{sub:lots_of_dormant_heads}), and showing that the dormant head phenomenon persists in small autoregressive transformers trained on next-token-prediction (\Cref{sub:controlled_experiments}).

\DP{TODO: description}

\subsection{Evidence 1 For Conjecture: Circuit for Dormant Heads in Llama 2} \label{sub:circuit_evidence}

\DP{TODO: description}

\begin{figure}[t]
  \centering
  % \begin{minipage}{0.24\textwidth}
  %     \centering
  %     \subcaption{\small Attention weights}
  %     \label{fig:circuit-attn-weights}
  %     \vspace{-.2em}
  %     \includegraphics[width=\linewidth]{Figures/figures_circuit/attn_weights_dormant.pdf}
  % \end{minipage}
  % \hspace{-1em}
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Attention logits}
      \label{fig:circuit-attn-logits}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/logits.pdf}
  \end{minipage}~
  % \hspace{-1em}
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Output norm}
      \label{fig:circuit-massive-norm}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/massive.pdf}
  \end{minipage}
  \hspace{-1em}
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Value states norm}
      \label{fig:circuit-value-norm}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/values.pdf}
  \end{minipage}
  \vspace{-1em}
  \caption{\small \textit{Algebraic findings.} We sample ``\bos~Summer is hot. Winter is cold.'' $+$ ``random test token'''s for $1000$ times to obtain a distribution of hidden states in \llama. Figure \ref{fig:circuit-attn-logits} presents the attention logits computed by using the test tokens as queries and the previous tokens as keys. The logits on \bos~and the first \delim are effectively positive constants, with logits on other tokens vary among different test tokens, and being mostly negative. Figure \ref{fig:circuit-massive-norm} shows the norm of the outputs across all the layers, with the \bos~and the first \delim possessing significantly massive norms from layers 2 to 29. Figure \ref{fig:circuit-value-norm} shows the norm distribution of the value states across layers 2 to 29. The norms of the \bos~and the first \delim token are effectively small constants. 
  }
  \label{figure:algebra-findings}
  \vspace{-1em}
\end{figure}



We summarize the algebraic features of \bos~ and the first \delim tokens in the computation graph, all of which point to the dormant heads conjecture. Previous works discover parts of these features separately. As a demonstration, we randomly sample 1000 tokens from the vocabulary of \llama, prefix it with ``\bos~Summer is hot. Winter is cold.'' to form one test sequence, and implement the forward pass. By collecting  hidden states for each test sequence, it provides us with a distribution of hidden states.
\ref{figure:algebra-findings} summarizes the four algebraic features:
\begin{enumerate}
    \item \textit{Attention sink}: Figure XXX visualizes the attention weights. Before the first \delim, the attention weights from all tokens on \bos~are near 1. The \delim would split half of the attention weights on \bos.
    \item \textit{Stable attention logits}: Figure \ref{fig:circuit-attn-logits} presents the attention logits from the test token (query) on tokens in the prefix (key). The distribution comes from a fixed head, L16H25, with 1000 test tokens. The attention logits on \bos~and \delim are nearly constant across all test tokens, while vary a lot on other tokens. 
    \item \textit{Massive norms}: Figure \ref{fig:circuit-massive-norm} presents the norm of hidden states across layer 0 to 31, averaged among 1000 test sequences. The \bos~and \delim have norms around 500 to 1000 times of other tokens.
    \item \textit{Small value states}: Figure \ref{fig:circuit-value-norm} shows the norm distribution of norms of value states. The distribution comes from all heads from layer 2 to 29 and with 1000 test tokens. \bos~and the first \delim both possess negligible norm.
\end{enumerate}

\tianyu{I will postpone the circuit here}
The algebraic findings depict a potential circuit of the dormant mechanism. Figure XXX illustrates the entire procedure, which we summarize as follows:
\begin{enumerate}
    \item Preparatory phase (layer 0 and 1): The $\mlp$ of layer 1 adds an output with massive norm residual streams of \bos~and the first \delim tokens. Using causal ablations, we verify the function of each components in layer 0 and 1.
    \begin{enumerate}
        \item \tianyu{We need to discuss the names here} Both the $\MLP$ in layer 0 and 1 contribute to the formation of a XXX in layer 1.
        \item $\Attn$ in both layer 0 and 1 adjust the formation of XXX. For example, shown by zero-out intervention, L1H8 both assists the initial token to be XXX and suppresses the other tokens to be XXX.
        \item The \rope in $\Attn$ heads in layer 0 and 1 suppresses the formation of XXX starting from the second delimiter tokens.
    \end{enumerate}
    \item Dormant/active phase: At this stage, the residual streams of \bos~and the first \delim remain nearly untouched, since any outputs added on the residual stream have negligible norms. At the main time, the layer norm map them to a special direction XXX, which corresponds to a sink key state which has nearly constant attention logits fitted with any queries. The direction XXX also possesses minor value states,. As a result, a test token has two modes on the attention weights:
    \begin{itemize}
        \item dormant mode: when no other keys align with its queries. After the Softmax function, \bos~and the first \delim take up a great proportion of its attention weights
        \item active mode: when there's other key that aligns with its query, which renders a attention logits comparable or even greater than the attention logits on \bos. After the Softmax function, \bos~and the first \delim take up a small proportion of its attention weights.
    \end{itemize}
    Since the value states of \bos~and \delim are notably small,
    The different modes on attention weights lead to different     \begin{itemize}
        \item dormant mode: add a minor output on the residual stream
        \item active mode: add a large output on the residual stream
    \end{itemize}
\item Recover phase: On \bos~and \delim, the $\MLP$ in the last two layers add a massive norm on the residual, while on its negative direction. As a result, The norms of \bos~and \delim become normal. There's no dormant phenomenon in last two layers.
\end{enumerate}

After the preparatory work in layers $0$ and $1$, the


\subsection{Evidence 2 For Conjecture: Abundance of Dormant Heads in Llama 2} \label{sub:lots_of_dormant_heads}

\DP{TODO: description}

\subsection{Evidence 3 For Conjecture: Dormant Heads in Small Transformers} \label{sub:controlled_experiments}

We further demonstrate that attention heads learn to be dormant even under a toy task, which we call as the \textit{dormant copy} task. As illustrated in Figure \ref{fig:pretraining-dgp}, we generate the input sequence with three steps. First, we always start with a \bos~token. Second, on normal tokens, we use a pre-determined Markov transition probability $P_e$ to predict the next token. Third, on $k$ trigger tokens, instead of using the Markov transition $P_e$, we copy the previous token to the next position. Similar to \citet{bietti2024birth}, we choose the $P_e$ and the vocabulary from the estimated character-level bigram distribution on the tiny \textit{Shakespeare} dataset. We manually add the \bos~token to the character-level vocabulary of \textit{Shakesphere}, making it to contain $N_{voc}=66$ tokens in total. 
To avoid repeat occurrence of the \bos~token, We sample the second token from the estimated unigram distribution in the \textit{Shakespeare} dataset, but drop the sequence if it's a trigger token. We fix the trigger tokens as the $k=3$ most frequent tokens in the unigram distribution.

The optimal algorithm for the \textit{dormant copy} task is to predict the next token distribution with $P_e$ on normal tokens and with previous tokens on trigger tokens. The transformer structure allows it to replicate the optimal algorithm. With the dormant conjecture in mind, since normal tokens do not require any in-context mechanism, we expect the $\Attn$ layer is dormant with only the $\MLP$ layer takes effect. The trigger tokens require the copying from the previous token, on which we expect the $\Attn$ layer is active. 

To verify our dormant/active modes mechanism, we pre-train a transformer with $1$ layer and $1$ head on the \textit{dormant copy} task using ADAM for $10000$ rounds. The resulting transformer could match the optimal algorithm on the prediction loss. More importantly, we observe clear patterns of the $\Attn$ head being dormant or active. Figures \ref{fig:pretraining-attn-weights-dormant} and \ref{fig:pretraining-attn-weights-active} visualize the attention weights on different input sequences. Figure \ref{fig:pretraining-attn-weights-dormant} shows that the \Attn head is dormant, with all attention weights are on the \bos~token when there's no trigger token. As a result, the \Attn head only adds a constant to the residual stream of normal tokens. Figure \ref{fig:pretraining-attn-weights-active} shows that the \Attn head is active and attend on the previous tokens from trigger tokens, which adds information from the previous tokens on the residual stream of trigger tokens.

\begin{figure}[t]
  \centering
  \begin{minipage}{0.4\textwidth}
      \centering
      \subcaption{\small Data generating procedure}
      \label{fig:pretraining-dgp}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_copy.pdf}
  \end{minipage}
  \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Dormant}
      \label{fig:pretraining-attn-weights-dormant}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_copy/dormant_copy_attn_weights_seq0.pdf}
  \end{minipage}
  \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Active}
      \label{fig:pretraining-attn-weights-active}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_copy/dormant_copy_attn_weights_seq1.pdf}
  \end{minipage}
  % \vspace{-1em}
  \caption{\small \textbf{The dormant copy experiment.} Figure \ref{fig:pretraining-dgp} illustrates the data generating procedure of the dormant copy task. We fix `t', `e', and ` ' as three trigger tokens. Figure \ref{fig:pretraining-attn-weights-dormant} shows the attention weights on an input without triggers, with the $x$-axis representing the key tokens and the $y$-axis representing the query tokens. The \bos~token takes up nearly all the attention weights among all tokens. Figure \ref{fig:pretraining-attn-weights-active} shows the attention weights on an input with triggers. The \Attn head still puts all attention weights on normal tokens. However, it is active on trigger tokens and attend to the previous tokens.}
  \label{figure:pretraining-findings}
  \vspace{-1em}
\end{figure}

Moreover, on a pre-trained transformer with $3$ layers, we could recover all the algebraic features of the dormant mechanism in large language models. Figure \ref{fig:pretraining-massive-norm} presents the distribution of output norms of layer $1$ on different tokens, sampled from $512$ input sequences with each has $256$ tokens. The output norm of \bos~(around 100) is notably greater than most tokens. Surprisingly, the token $\backslash n$ has even greater norm. Figure \ref{fig:pretraining-small-value} presents the corresponding distribution of value states. Matching the massive norms of the output, \bos~and $\backslash n$ both possess remarkably small value states. It's unclear why the token $\backslash n$ also exhibits similar features with the \bos~token. We conjecture that similar to the first \delim token in \llama, the $\backslash n$ assists the dormant mechanism with the \bos~token. We delegate attention weights plots supporting this conjecture in the appendix.

\begin{figure}[t]
  \centering
  \begin{minipage}{0.4\textwidth}
      \centering
      \subcaption{\small Massive norms}
      \label{fig:pretraining-massive-norm}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_copy/dormant_copy_L3_massive.pdf}
  \end{minipage}
  \begin{minipage}{0.4\textwidth}
      \centering
      \subcaption{\small Small value states}
      \label{fig:pretraining-small-value}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_copy/dormant_copy_L3_minor.pdf}
  \end{minipage}
  \vspace{-1em}
  \caption{\small \textbf{The norms of hidden states in the dormant copy experiment} A summary of the norm distributions of the output of layer 1 (Figure \ref{fig:pretraining-massive-norm}) and the value states of layer 2 (Figure \ref{fig:pretraining-small-value}) in a 3-layer transformer trained on the \textit{dormant copy} task. The \bos~token is at the left most, with three trigger tokens ` ', `t', and `e' following it. We then randomly choose six tokens and separately summarize their norm distributions. We pull all other tokens together, forming the distribution of the norms of others at the right most. Only the \bos~and the $\backslash n$ token possess remarkably large output norms and small value states norms.}
  \label{figure:pretraining-findings-norms}
  \vspace{-1em}
\end{figure}

The inspection on the training dynamics enriches our understanding of the emergence of the dormant mechanism. Figure \ref{figure:pretraining-dynamics} summarises the change of multiple metrics along the training dynamics, including the ICL risk, the Markov prediction risk, the proportion of tokens that only attend to the \bos~token, the average attention weights on \bos, and the scaled norm of the output of layer 1 on \bos. Figure \ref{fig:pretraining-dynamics-long} presents their change along the entire training steps. The norm of the \bos~in layer 1 keeps increasing while other metrics remain unchanged. Figure \ref{figure:pretraining-dynamics} zooms in on the first 0 to 1000 steps along the training steps. The dynamics exhibit three phases: 1. Markov learning phase (0 to 140 steps): The prediction risk on normal tokens drops; the ICL risk firstly drops then stuck at a relatively high level; there is neither large attention weights nor massive output norms on the \bos~token. 2. ICL learning phase (140 to 240 steps): The prediction risk on normal tokens has negligible decrease; the ICL risk drops sharply; at the same time, the attention weights on the \bos~token increase and the output norms of \bos~slightly decreas. 3. Attention sink and massive norm formation phase (after 240 steps): the ICL risk decreases slowly and remains unchanged after 1000 training steps; the attention weights and the proportion of dormant tokens keep increasing; the output norm of \bos~keeps increasing along all training steps.

\begin{figure}[t]
\centering
    \begin{minipage}{0.4\textwidth}
      \centering
      \subcaption{\small From 0 to 10000 steps}
      \label{fig:pretraining-dynamics-long}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_copy/dormant_copy_dynamics_long.pdf}
  \end{minipage}
    \begin{minipage}{0.4\textwidth}
      \centering
      \subcaption{\small Zoom in on 0 to 1000 steps}
      \label{fig:pretraining-dynamics}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_copy/dormant_copy_dynamics.pdf}
  \end{minipage}
  \hspace{-1em}

  \vspace{-1em}
  \caption{\small \textbf{Training dynamics of the dormant copy experiment} The ICL risk computes the prediction risk on trigger tokens; the Markov risk computes the prediction risk on normal tokens; we count the number of tokens that have attention weights on the \bos~token greater than 0.9 and get the proportion of dormant tokens; we take the average attention weights on \bos~from normal tokens; for better visualization and since only the trend is important in our message, we scale down the output norm of \bos~by $20$. The training dynamics possess three phases, with the Markov risk drops first, then the ICL risk together with the attention sink, and finally the massive norm emerges.}
  \label{figure:pretraining-dynamics}
  \vspace{-1em}
\end{figure}


==> Sections/deprecated_sections/findings.tex <==
\section{Findings}

Attention sink phenomenon: For autoregressive LLMs such as Llama2, in intermediate layers (all but layers 0, 1, 2, and -1) and most heads, the $N\times N$ attention matrix is heavily concentrated on the initial token.

Consider a fixed (layer, head) in which ``attention sink'' happens. Let $(\bq_i, \bk_i, \bv_i)_{i\in[N]}$ denote the (query, key, value) vectors for this head. Let $(\bh_i)_{i\in[N]}$ denote the hidden state vector. Let $s_{ij}$ denote the attention score of query token $i$ with respect to KV token $j\in[i]$. Attention sink refers to the phenomenon that
\begin{align*}
    s_{i1} \approx 1, \quad s_{ij}\approx 0~~\textrm{for}~~2\le j\le i.
\end{align*}

\paragraph{Our findings}
\begin{enumerate}
    \item Value norms exhibit ``reverse sink'':
    \begin{align}
    \label{eqn:value}
        \ltwo{\bv_1} \ll \ltwo{\bv_j}~~\textrm{for}~~2\le j\le i,
    \end{align}
    and they balance out the attention sink in the sense that
    \begin{talign*}
        \ltwo{s_{i1}\bv_1} \approx \ltwo{\sum_{j=2}^i s_{ij}\bv_j},
    \end{talign*}
    where ``$\approx$'' denotes the same order of magnitude. This means that the head is still non-degenerate, and is not approximable by a fixed value vector. Also, the ``sparse attention'' interpretation~\citep{block2023llm} is wrong.

    % \yub{However, we can use this to by-pass the partition function in softmax and speed up the attention computation (even in FlashAttention?)}

    \item Hidden state norms exhibit a sink:
    \begin{align*}
        \ltwo{\bh_1} \gg \ltwo{\bh_j}~~\textrm{for}~~2\le j\le i.
    \end{align*}
    Combined with~\cref{eqn:value}, it must happen that the value matrix $\bV$ is nearly orthogonal to $\bh_1$, compared with to $(\bh_j)_{j\ge 2}$.
\end{enumerate}

Ablations:
\begin{enumerate}
\item Most LLMs exhibit this phenomenon (this is more exacerbated with RoPE embedding, but standard trainable positional encoding schemes like GPT-2 also exhibits this).

\item This phenomenon shows up very early in training, but not at init. 
\end{enumerate}

==> Sections/deprecated_sections/linear-algebra.tex <==


\section{Linear algebraic mechanisms behind sink tokens}

\tianyu{Massive tokens are not necessarily sink tokens in OOD?}

\yub{better title?}

\yub{In each subsection, we give a set of plots (in 1 - 2 lines), and give some explanation. If there is some further studies that naturall come after the initial set of plots, we give another set of plots.}

Throughout the rest of this section, we use LlaMa2-7B~\citep{touvron2023llama}.

\subsection{Birth of sink tokens}

\paragraph{How are sink tokens produced?}
% ~\yub{mostly done.}

\cref{fig:mlp1} shows that $\MLP_1$ produces the sink tokens, i.e. makes certain tokens have massive norms.


LlaMa's MLP layer is defined by three weight matrices $\sets{\Wgate, \Wdown, \Wup}$~\yub{dimensions} with the SwiGLU activation~\citep{shazeer2020glu}:
\begin{align}
    f_{\mlp}(\bh) = \Wdown \paren{ \silu\paren{ \Wgate\bh } \odot \paren{\Wup\bh} }.
\end{align}
Above, $\silu(t) \defeq t\cdot \sigmoid(t)$ denotes the SiLU (or Swish) activation~\citep{ramachandran2017searching}.

\begin{figure}[H]
\centering
\begin{minipage}{.32\textwidth}
\centering
    % \subcaption{{\footnotesize BLAH}}\label{fig:11}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/Summer/layer_1_attn_output.pdf}
\end{minipage}
% \hfill
\begin{minipage}{.32\textwidth}
    \centering
    % \subcaption{{\footnotesize BLAH}}\label{fig:12}
    %\vspace{-.7em}
    \includegraphics[width=.95\textwidth]{Figures/Summer/layer_1_attn_output_post_residual.pdf}
\end{minipage}
% \hfill
% \begin{minipage}{.24\textwidth}
%     \centering
%     \subcaption{{\footnotesize BLAH}}\label{fig:13}
%     %\vspace{-.7em}
%     \includegraphics[width=.95\textwidth]{Figures/Summer/layer_1_attn_output_post_ln.pdf}
% \end{minipage}
\begin{minipage}{.32\textwidth}
    \centering
    % \subcaption{{\footnotesize BLAH}}\label{fig:14}
    %\vspace{-.7em}
    \includegraphics[width=.95\textwidth]{Figures/Summer/layer_1_mlp_output.pdf}
\end{minipage}
\caption{
\small
Sink tokens (token 0 and token 3) are produced by $\MLP_1$. Sentence: ``Summer is warm. Winter is cold.''
\yub{maybe a better illustration is to track the evolution of all 8 tokens, one on each curve, x axis is the module name (along forward pass), y axis is norm.}
}
\label{fig:mlp1}
\vspace{-1em}
\end{figure}

% Group of plots for $\MLP_1$. Plot 0: Narrow it down to MLP1. Plot 1: Some flowchart. Plot 2 (maybe with one other plot that shows the shape of $W3[:, 7890]$): How massive tokens activate the $W_{\{1,2\}}[7890, :]$, and how $W3[:, 7890]$ produces massive entries at $1415, 2533$.


\begin{figure}[H]
\centering
\begin{minipage}{.32\textwidth}
\centering
    \subcaption{{\footnotesize Histogram of $\sets{\ltwos{\Wgate[i, :]}}_{i}$}}\label{fig:w1-norm}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/Summer/w1_norm_hist.pdf}
\end{minipage}
% \hfill
\begin{minipage}{.32\textwidth}
    \centering
    \subcaption{{\footnotesize $\<\bh_j, \Wgate[i, :]\>$}}\label{fig:corr-w1}
    %\vspace{-.7em}
    \includegraphics[width=.95\textwidth]{Figures/Summer/corr_with_w.pdf}
\end{minipage}
% \hfill
% \begin{minipage}{.24\textwidth}
%     \centering
%     \subcaption{{\footnotesize BLAH}}\label{fig:13}
%     %\vspace{-.7em}
%     \includegraphics[width=.95\textwidth]{Figures/Summer/layer_1_attn_output_post_ln.pdf}
% \end{minipage}
\begin{minipage}{.32\textwidth}
    \centering
    \subcaption{{\footnotesize $\Wdown[:, i]$}}\label{fig:w3}
    %\vspace{-.7em}
    \includegraphics[width=.95\textwidth]{Figures/Summer/w3.pdf}
\end{minipage}
\caption{
\small
Mechanisms of $\MLP_1$. (a) Neuron 7890 has the largest norm among all neurons in $\Wgate$. (b) $\Wgate[7890, :]$ has large positive inner products with sink tokens, and large negative inner products with non-sink tokens. (c) $\Wdown[:, 7890]$ has large entries at $[1415, 2533]$-th coordinate.
Sentence: ``Summer is warm. Winter is cold.''
}
\label{fig:special-neuron}
\vspace{-1em}
\end{figure}

\textbf{What does the special neuron tell us?} By computing the correlations of hidden states and $\Wgate[7890, :]$, we can detect important sub-layers that contribute to the massive tokens.

\begin{figure}[H]
\centering
\begin{minipage}{.24\textwidth}
\centering
    \subcaption{Layer 0 with ROPE}\label{fig:l0-rope-corr}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/tianyu_tentative/layer0wrope.png}
\end{minipage}
% \hfill
\begin{minipage}{.24\textwidth}
\centering
    \subcaption{Layer 1 with ROPE}\label{fig:l1-rope-corr}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/tianyu_tentative/layer1wrope.png}
\end{minipage}
\begin{minipage}{.24\textwidth}
\centering
    \subcaption{Layer 0 without ROPE}\label{fig:l0-norope-corr}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/tianyu_tentative/layer0norope.png}
\end{minipage}
\begin{minipage}{.24\textwidth}
\centering
    \subcaption{Layer 1 without ROPE}\label{fig:l0-rope-corr}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/tianyu_tentative/layer1norope.png}
\end{minipage}
\caption{
\small
Bar-plots of correlations between hidden states and $\Wgate[7890, :]$.
}
\label{fig:special-neuron}
\vspace{-1em}
\end{figure}


\paragraph{Why does the initial token always become a sink token?}
Our approach is to examine the forward pass of all 32K tokens in LlaMa tokenizer.

% Do all the 32000 tokens get to be attention sinks when placed at the initial position?~\yub{vast majority, but not all.}

\begin{figure}[H]
\centering
\begin{minipage}{.25\textwidth}
\centering
    \subcaption{{\footnotesize Norm after Layer 1}}\label{fig:initial-layer1-norm}
    %\vspace{-.7em}
    \includegraphics[width=\textwidth]{Figures/initial_token/token_0_layer_1_out_norms.pdf}
\end{minipage}
% \hfill
\begin{minipage}{.25\textwidth}
    \centering
    \subcaption{{\footnotesize Norm of embeddings}}\label{fig:initial-embed-norm}
    %\vspace{-.7em}
    \includegraphics[width=\textwidth]{Figures/initial_token/token_0_embed_norms.pdf}
\end{minipage}
% \hfill
% \begin{minipage}{.24\textwidth}
%     \centering
%     \subcaption{{\footnotesize BLAH}}\label{fig:13}
%     %\vspace{-.7em}
%     \includegraphics[width=.95\textwidth]{Figures/Summer/layer_1_attn_output_post_ln.pdf}
% \end{minipage}
\begin{minipage}{.48\textwidth}
    \centering
    \subcaption{Inner product with $\bw_\star$}\label{fig:ph}
    %\vspace{-.7em}
    \includegraphics[width=\textwidth]{Figures/initial_token/evolution_initial_token.pdf}
\end{minipage}
\caption{
\small
Evolution of token 0 along the forward pass. Here each sentence just consists of a single token.
}
\label{fig:special-neuron}
\vspace{-1em}
\end{figure}

% \yub{TODO(yub): Evolution of initial token to be aligned with $\bw_\star$. Choose one regular token, and one small token. Also work out a common plot scheme for evolution plots.}

% Plot 1. Out of the 32000 tokens, about 31800 of them gets to be massive when placed at the initial token (maybe use one plot). Plot 2: Evolution of initial token to be aligned with $\bw_\star$.

\yub{TODO(Tianyu): exhaust the list of delimiter tokens (among 32K tokens), defined as any token that becomes massive at non initial locations.}

\paragraph{Which head turns token 0 into sink token?}

\yub{Tianyu has some findings here (Attn1, Head8).}~\yub{Made a plot for Attn1 in~\cref{fig:attn1-heads-rope}.}

Head 8 in $\Attn_1$ is the main symmetry breaker here. See~\cref{fig:attn1-heads-rope}.

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{Figures/attn_0/attn_1_inner_prod_wstar.pdf}
    \caption{\small The inner product between $\Attn_1$'s \emph{OV output} in each head, and $\bw_\star$. We plot both across heads $m\in[M]$, and across tokens $\bh_i$ in the sequence. Sentence: ``Summer. Summer. Summer. Summer. Summer.'' We also consider a NoRoPE version where the RoPE in $\Attn_0$ is disabled. Observe that {\bf Head 8} produces a large output on the initial token.}
    \label{fig:attn1-heads-rope}
\end{figure}


\yub{Do we have an answer now for why initial token becomes massive? Based on Head 8}

\paragraph{Which head identifies delimiter tokens?}

When feeding LLM with a single token, the attention weights reduces to a point mass, and the attention output reduces to the summation of ``OV'' projections:
\begin{align}
    \Attn_0(\sets{\bh_0}) = \sum_{m=1}^M \bO_m\bV_m \bh_0, \quad \bO_m\in\R^{d\times (d/M)},~\bV_m\in\R^{(d/M)\times d}.
\end{align}

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{Figures/attn_0/attn_0_corr_wstar.pdf}
    \caption{\small The correlation of $\sets{\bO_m\bV_m\bh_0}_{m,\bh_0}\subset \R^d$ with $\bw_\star$ across both different heads $m\in[M]$, and across different tokens $\bh_0$ (corresponding to post-layernorm of the 32K token embeddings). Several heads identify the period token $29889$ (`.'). }
\end{figure}



\paragraph{Why the \emph{first} delimiter only?}
why does first delimiter become sink, and other layers not become sink?~\yub{TODO, some more symmetry breaking analysis with attention}

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{Figures/attn_0/attn_0_inner_prod_wstar.pdf}
    \caption{\small The inner product between $\Attn_0$'s \emph{OV output} in each head, and $\bw_\star$. We plot both across heads $m\in[M]$, and across tokens $\bh_i$ in the sequence. Sentence: ``Summer. Summer. Summer. Summer. Summer.'' We also consider a NoRoPE version where the RoPE in $\Attn_0$ is disabled. Observe that for {\bf Head 28}, the versions with and without RoPE differ significantly in their patterns.}
    \label{fig:attn0-heads-rope}
\end{figure}

% $w_\star^{(0)}=W_1^{(0)}[7374, :]$
Message: 1. We find, Head 28 in Attn 0 actually got impacted a lot by Rope. First, for period token, its OV state by head 28 produces a large negative correlation with $\bw_\star$ (see~\cref{fig:attn0-heads-rope}). Then, if there is rope in head 28 (as in regular LLM), then second period onward will attend significantly to prevoius period tokens. As a result, the attention output gives get large negative correlation. However, if there is no rope in head 28, then basiccally this negative correlation won't affect things, and period tokens would have positive correlation with $w_\star^{(0)}$. 

\begin{figure}[H]
\centering
\begin{minipage}{.32\textwidth}
\centering
    \subcaption{Attention weights of head 28 in layer 0}\label{fig:l0-h28-attn}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/tianyu_tentative/attn1 28.png}
\end{minipage}
% \hfill
\begin{minipage}{.32\textwidth}
\centering
    \subcaption{Cumulative correlations with $\bW_0[7374, :]$ across attention layer 0}\label{fig:attn-head-corr}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/tianyu_tentative/attn2 cum corr.png}
\end{minipage}
\begin{minipage}{.32\textwidth}
\centering
    \subcaption{Correlations between value states and $\bW_0[7374, :]$}\label{fig:value-corr}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/tianyu_tentative/values_w0star corr.png}
\end{minipage}
\caption{
\small
Mechanisms for the break of symmetry on the second delimiter.
}
\label{fig:special-neuron}
\vspace{-1em}
\end{figure}

\begin{figure}[H]
\centering
% \hfill
\begin{minipage}{.45\textwidth}
\centering
    \subcaption{Cumulative correlations with $\bW_1[7890, :]$ across attention layer 1}\label{fig:attn1-head-corr}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/tianyu_tentative/attn1 cum corr.png}
\end{minipage}
\begin{minipage}{.45\textwidth}
\centering
    \subcaption{Correlations between value states and $\bW_1[7890, :]$}\label{fig:value1-corr}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/tianyu_tentative/values w1star corrs.png}
\end{minipage}
\caption{
\small
Mechanisms for the break of symmetry on the second token.
}
\label{fig:special-neuron}
\vspace{-1em}
\end{figure}




The later mechanism in $\MLP_0$ and consequently $\MLP_1$ dictates that, a positive correaltion with $w_\star^{(0)}$ makes the token massive.


\subsection{Attention concentration}

\yub{Put initial plots + study in more depth.}

\subsection{Value anti-concentration}

\yub{Put initial plots + study in more depth.}

\subsection{Something else...?}

\yub{what happens for other architectures? Mainly mistral 7B.}

\yub{training dynamics? (can do this for either GPT2, or XGen-7B), for which we can obtain the model checkpoints.}

==> Sections/deprecated_sections/sink-tokens.tex <==
\section{Sink tokens in LLMs}

\subsection{Transformers}

\subsection{Sink tokens}

\yub{Formalize language: what we mean by ``initial token'', ``delimiter token'', etc, is the hidden states vectors in the middle.}

==> Sections/deprecated_sections/sparsify.tex <==
\section{Attention sparsification for accelerated inference}

\yub{Question: how does it reconcile with the value anti-concentration thing.}

\yub{Normalize could have played a role?}

==> Sections/deprecated_sections/theory.tex <==
\section{Theory}
Let \( N^{(\ell)} \) be the number of $(\ell)$ tokens in front of a Markov token, let \( \beta^{(\ell)} \be_{\ell} \) be the corresponding value state. 
state, and let \( p_{k} \) be the Markov transition probability, i.e., $P( k \mid \text{current term})$.

\[
\text{Loss} = \sum_k p_k \left[ \log \left( \sum_{\ell} p_\ell e^{\frac{\beta^{(\ell)}N^{(\ell)}}{e^y+N}}\right) - \frac{\beta^{(\ell)}N^{(\ell)}}{e^y+N} - \log p_k\right].
\]

(I later realized that we should use $e^x\approx 1+x+x^2/2$ and $\log(1+x)\approx x$ to approximate.

==> Sections/discussion.tex <==
\section{Discussion and Implications}\label{sec:discussion}



==> Sections/plans.tex <==
\section*{Outline}
\begin{itemize}
    \item \sm{Title: Birth of Attention Sink in Large Language Models}
    \item \tianyu{Title: Switching Attention Heads: Mechanistically Demystifying Outlier Phenomena in LLMs}
    \item \DP{Title: Outlier Phenomena in Large Language Models}
\end{itemize}
% \paragraph{Some concepts: }
% \begin{itemize}
%     \item Dormant attention head: given an input, a head that effectively outputs a bias, i.e., doesn't have cross token interactions
%     \item Active attention head: a head which is not dormant on the particular input
%     \item Relate dormant attention head to attention sink: the attention sink is nearly the only possible mechanism for a head to be dormant while remaining the ability to be active
%     \item Functional head: head which has some defined function(s) during forward pass
%     \item Indexing: from 0
%     \item Attention weights: The attention weight from token $i$ to the BOS is large.
%     \item Massive token \& Massive activation (need to clarify in the preliminaries)
%     \item Dormant head token score = attention score of BOS + all delimiter tokens
%     \item Dormant head detection metric = (maximum/mean) dormant head token score over all tokens in the sample
%     \item Dormant head detection thresholds = bound for dormant head detection metric, above (resp.~below) which the head is classified as dormant (resp.~active) on the given sample
%     \item \sm{Suggested name for "Dormant copy model": Bigram-Backcopy Model (BBM) or Markov Backcopy Model (MBM). }
%     \item  \sm{Message: The observed sink heads are not always dormant. Every head has a dormant phase and an active phase. In the active phase, the head transports information from previous tokens to the current one. In the dormant phase, the head behaves as if it is constantly biased. Plot the histogram of dormant metric for every head over different prompts. Use L16H25 Llama 2 as a concrete example. }
%     \item \sm{Title: Birth of Attention Sink in Large Language Models}
%     \item \tianyu{Title: Attention heads learn to have dormant phase: demystifying (attention sink; massive norm; value states) extreme values in LLMs}
% \end{itemize}

% \paragraph{Outline: }
% \begin{itemize}
%     \item Section 1: Intro and related work
%     \begin{itemize}
%         \item Introduction (TODO: DP)
%         \item Related work (TODO: SM? + DP)
%     \end{itemize}
%     \item Section 2: Case study as motivation for conjecture
%     \begin{itemize}
%         \item Notations (TODO: DP)
%         \item Preliminaries (what is a transformer, what is attention, etc) (TODO: DP)
%         \item Preliminaries part 2 (what are massive activations, what are massive tokens, what are attention sinks) --- point out the figure for Layer 16 Head 25, point out it's massive activation, massive token, attention sink properties (TODO: DP)
%         \item Llama2 Layer 16 Head 25: what do we observe about its behavior on Wiki vs coding? Use the best precision we can give in the time remaining  (TODO: DP)
%         \begin{itemize}
%             \item Two side-by-side figures of attention weights on this head on Wikipedia and Github
%             inputs (TODO: DP)
%             \item Same for logits (TODO for figure generation: DP, for detailed analysis: TG)
%         \end{itemize}
%     \end{itemize}
%     \item Section 3: Conjecture and evidence 
%     \begin{itemize}
%         \item Describe dormant head conjecture in as precise language as possible (TODO: DP + TG?)
%         %\item Theoretical evidence: linear algebraic mechanism + empirical evidence: attention sinks + massive activation (TODO: DP + TG)
%         \begin{itemize}
%             \item Attention sink is nearly the only possible mechanism to keep head dormant on some inputs and active on others
%         \end{itemize}
%         \item Evidence 1: circuit in Llama2 which causes dormant head (TODO: TG)
%         \begin{itemize}
%             \item a flowchart (TG + DP)
%             \item some supporting findings: norm bar-plot of tokens? table of (mean, var) of attention logits on bos tokens and other tokens (some randomly selected tokens) 
%         \end{itemize}
        
%         \item Evidence 2: intervention study on Llama 2. Goals: show that our automated dormant head detection system is very effective with strong quantitative behavior connecting to qualitative observations, and then show that it finds many heads (TODO: DP)
%         \begin{itemize}
%             \item Graph all heads. x axis = max metric among 32 samples of Wikipedia + 32 samples of Github, y axis = min metric, top right = always dormant, bottom left = always active, etc. Red color for L16H25. (TODO: DP)
%             \item Display \# of heads detected on Wikipedia, Github, and Wikipedia+Github (TODO: DP; also include common crawl?)
%         \end{itemize}
%         \item Evidence 3: pretraining on simple tasks? (TODO: TG)
%         \begin{itemize}
%             \item Attention weights heatmap for the ``dormant copy'' experiment;
%             \item Training Dynamics of the ``dormant copy'' experiment;
%         \end{itemize}
%     \end{itemize}
%     \item Section 4: Discussions, implications on interpretability? (TODO: DP? + TG)
%     \begin{itemize}
%         \item Conjecture on the emergence of dormant heads during pretraing: task variety -> value states monosemanticity -> dormant mechanism (the supporting experiment is in appendix)
%         \item Conjecture on massive tokens and massive activations
%         \item Some parts of Circuit are not fully understood.
%         \item Contradicting observations of dormant conjecture: Relationship of dormant head to head irrelevant for task (i.e., zeroing out doesn't change PPL)?
%         \begin{itemize}
%             \item Table documenting the perplexity before and after zeroing out L16H25 on Wikipedia and Github
%             \item Table relating attention sink score to PPL difference when zeroing out; shows weak trend (\DP{TODO: need to do it for new metrics})
%         \end{itemize}
%     \end{itemize}
%     \item Section 5: Conclusion (TODO: DP)

%     \item Appendix:
%     \begin{itemize}
%         \item Supporting results for Evidence 1:
%         \begin{itemize}
%             \item An illustration figure to explain the method to find the circuit
%         \end{itemize}
%         \item Supporting results for Evidence 2:
%         \begin{itemize}
%             \item Include plots for 32 samples on Wiki/Github for the given special head L16H25
%             \item Ablation on the different dormant head token score mechanism + dormant head detection metric --- lots of figures, pretty convincing that these choices are fairly robust
%         \end{itemize}
%         \item Supporting results for Evidence 3:
%         \begin{itemize}
%             \item Ablations: Biette's setting;
%             \item Ablations part2: another one;
%             \item Interpolating between dormant copy and dormant markov
%             \item Massive tokens
%         \end{itemize}
%     \end{itemize}
%     \item REMEMBER LLAMA3 EXPS
% \end{itemize}

% \paragraph{New outline: }
% \begin{itemize}
%     \item Section 1: Intro and related work
%     \begin{itemize}
%         \item Introduction (TODO: DP)
%         \item Related work (TODO: SM + DP)
%     \end{itemize}
%     \item Section 2: Case study as motivation for investigation
%     \begin{itemize}
%         \item Notations (TODO: DP)
%         \item Preliminaries (what is a transformer, what is attention, etc) (TODO: DP)
%         \item Preliminaries part 2 (what are massive activations, what are massive tokens, what are attention sinks (TODO: DP)
%         \item  \sm{Our preliminary findings: The observed sink heads are not always dormant. Every head has a dormant phase and an active phase. In the active phase, the head transports information from previous tokens to the current one. In the dormant phase, the head behaves as if it is constantly biased. Plot the histogram of dormant metric for every head over different prompts. }
%         \item An example of the above point: Llama2 Layer 16 Head 25: what do we observe about its behavior on Wiki vs coding? Use the best precision we can give in the time remaining  (TODO: DP)
%         \begin{itemize}
%             \item Two side-by-side figures of attention weights on this head on Wikipedia and Github
%             inputs (TODO: DP)
%             \item Same for logits (TODO for figure generation: DP, for detailed analysis: TG)
%         \end{itemize}
%     \end{itemize}
%     \item Section 3: Static mechanism of attention sink, small value state, and massive norm. 
%     \begin{itemize}
%     \item Mechanism in Llama 2. 
%     \item Mechanism in Llama 3.1. 
%     \item Pretraining of Bigram-Backcopy task. One-layer TF demonstrates the attention sink and small value state phenomena. Three-layer TF demonstrates the massive norm phenomenon. 
%     \end{itemize}
%     \item Section 4: Dynamical mechanism of attention sink, small value state, and massive norm. 
%     \begin{itemize}
%     \item Statement of the mechanism: For any attention head with a certain prompt, if the value vector of any seen token is not useful in predicting the next token, the gradient dynamics, together with the softmax mechanism, will push the attention weights to the token with a small value vector. For tokens that are non-useful in predicting the next token in all prompts, since their attention weights are large, gradient dynamics will push down their value vector norm. So, large attention weights and small value vector norms reinforce each other, making such tokens sink tokens. Gradient dynamics favors pushing early tokens to be sink tokens. \sm{How to state the mechanism of the massive norm? }
%     \item Experimental evidence in BBM. (ReLU attention does not exhibit the behavior. ) 
%     \item Theoretical explanation in BBM. 
%     \item Experimental evidence in the pre-training checkpoint of Pythia. 
%     \end{itemize}
%     \item Section 5: Conclusion (TODO: DP)
% \end{itemize}

% \paragraph{New outline-copy: }
% \begin{itemize}
%     \item Section 1: Intro and related work
%     \begin{itemize}
%         \item Introduction (TODO: DP)
%         \item Related work (TODO: SM + DP)
%         \item Notations (TODO: DP)
%         \item Preliminaries (what is a transformer, what is attention, etc) (TODO: DP)
%         \item Preliminaries part 2 (what are massive activations, what are massive tokens, what are attention sinks (TODO: DP
%     \end{itemize}
%     \item Section 2: State our ``conjecture'' and show all experiments on LLMs.
    
% )
% \begin{itemize}
%         \item  \sm{Our preliminary findings: The observed sink heads are not always dormant. Every head has a dormant phase and an active phase. In the active phase, the head transports information from previous tokens to the current one. In the dormant phase, the head behaves as if it is constantly biased. Plot the histogram of dormant metric for every head over different prompts. }
%         \item An example of the above point: Llama2 Layer 16 Head 25: what do we observe about its behavior on Wiki vs coding? Use the best precision we can give in the time remaining  (TODO: DP)
%         \begin{itemize}
%             \item Two side-by-side figures of attention weights on this head on Wikipedia and Github
%             inputs (TODO: DP)
%             \item Same for logits (TODO for figure generation: DP, for detailed analysis: TG)
%         \end{itemize}
%     \item Mechanism in Llama 2. 
%     \item Mechanism in Llama 3.1. 
%     \item Experimental evidence in the pre-training checkpoint of Pythia. 
%     \end{itemize}
%     \item Section 3: Controlled experiments. 
%     \begin{itemize}
%     \item Pretraining of Bigram-Backcopy task. One-layer TF demonstrates the attention sink and small value state phenomena. Three-layer TF demonstrates the massive norm phenomenon. 
%     \item dynamics
%     \item (the importance of value states meaning)
%     \end{itemize}
%     \item Section 4: Dynamical mechanism of attention sink, small value state, and massive norm. 
%     \begin{itemize}
%     \item Theoretical explanation in BBM. (motivated by the results in Section 3)
%     \item (Statement of the mechanism): For any attention head with a certain prompt, if the value vector of any seen token is not useful in predicting the next token ({\color{red} the value vectors for seen tokens are useful for a different task}), the gradient dynamics, together with the softmax mechanism, will push the attention weights to the token with a small value vector. For tokens that are non-useful in predicting the next token in all prompts, since their attention weights are large, gradient dynamics will push down their value vector norm. So, large attention weights and small value vector norms reinforce each other, making such tokens sink tokens. Gradient dynamics favors pushing early tokens to be sink tokens. \sm{How to state the mechanism of the massive norm? }
%     \item massive norm: (1. related to attention sink; 2. the influence function is constant; 3. the Adam update is constant.)
%     \item (with our theory, we predict some experimental results): Show more experimental evidence in BBM. (ReLU attention does not exhibit the behavior; Simplified model shows similar dynamics (+value state, +massive norm); SGD eliminates the massive norms. )
    
    
%     \end{itemize}
%     \item Section 5: Conclusion (TODO: DP)
% \end{itemize}

Some token is a $\{$attention sink, value-state drain, residual-state peak$\}$. 

Some token has $\{$dominant attention score, small value state, massive residual state$\}$. 

"Outlier phenomena" vs "Extreme-value phenomena" vs "Extreme-token phenomena" vs "Sink Phenomena". 

"Active phase and dormant phase", "Active phase and idle phase". 

Mechanism: "active-dormant mechanism", "active-idle mechanism", "switching mechanism". 

Dynamical mechanism: "Cyclic-Reinforcement Mechanism", "Mutual Reinforcement Mechanism"


\paragraph{NEW New outline-copy (based on Tianyu's Slack proposal): }
\begin{itemize}
    \item Section 1: Intro and related work
    \begin{itemize}
        \item Introduction (TODO: DP)
        \item Related work (TODO: SM + DP)
        \item Notations (TODO: DP)
        \item Preliminaries (what is a transformer, what is attention, etc) (TODO: DP)
        \item Preliminaries part 2 (what are massive activations, what are massive tokens, what are attention sinks (TODO: DP
    \end{itemize}

    \item Section 2: Bigram-Backcopy task to isolate attention sink phenomenon. Statics and Dynamics.
    \begin{itemize}
    \item Motivate Bigram-Backcopy task. The optimal implementation should result in a ``controlled'' attention sink.
    \item Theoretical results of training dynamics in bigram-backcopy task.
    \item Empirical results of pretraining in BB task.
    \begin{itemize}
        \item Statics. One-layer TF demonstrates the attention sink and small value state phenomena. Three-layer TF demonstrates the massive norm phenomenon. 
        \item Circuit analysis and dynamics. Statement of the mechanism of attention sink in BB task: For any attention head with a certain prompt, if the value vector of any seen token is not useful in predicting the next token ({\color{red} the value vectors for seen tokens are useful for a different task}), the gradient dynamics, together with the softmax mechanism, will push the attention weights to the token with a small value vector. For tokens that are non-useful in predicting the next token in all prompts, since their attention weights are large, gradient dynamics will push down their value vector norm. So, large attention weights and small value vector norms reinforce each other, making such tokens sink tokens. Gradient dynamics favors pushing early tokens to be sink tokens. \sm{How to state the mechanism of the massive norm? } 
        \item massive norm: (1. related to attention sink; 2. the influence function is constant; 3. the Adam update is constant.) When there are multiple layers (>=3), the output of the first layer (both attn and mlp) facilitates the formation of attention sink in the upper layers (denote this output as $\boldsymbol{m}$)-> the scale of the $\nabla_{\text{Params in layer 0}} \ltwo{\boldsymbol{m}}$ remains constant -> due to the layer norm in upper layers, the norm of the projection of $\nabla_{\text{Params in layer 0}} \text{Loss} $ onto the direction of $\nabla_{\text{Params in layer 0}} \ltwo{\boldsymbol{m}}$ shrinks quickly. -> due to Adam, the small gradients lead to constant update. \DP{Check this in OLMO...}
        
        \item Additional predictions from this theoretical understanding. Show more experimental evidence in BBM. (ReLU attention does not exhibit the behavior; Simplified model shows similar dynamics (+value state, +massive norm); SGD eliminates the massive norms. )
        \item \DP{Major point: the predictions made in this section NEED to transfer to LLMs.}
    \end{itemize}
    \end{itemize}

    \item Section 3: Show that predictions from BB task translate to LLMs.
    \begin{itemize}
        \item  \sm{Our preliminary findings: The observed sink heads are not always dormant. Every head has a dormant phase and an active phase. In the active phase, the head transports information from previous tokens to the current one. In the dormant phase, the head behaves as if it is constantly biased. Plot the histogram of dormant metric for every head over different prompts. }
        \item An example of the above point: Llama2 Layer 16 Head 25: what do we observe about its behavior on Wiki vs coding? Use the best precision we can give in the time remaining  (TODO: DP) \DP{Characterize dormant vs active phase in Llama 2 L16H25}
        \begin{itemize}
            \item Two side-by-side figures of attention weights on this head on Wikipedia and Github
            inputs (TODO: DP)
            \item Same for logits (TODO for figure generation: DP, for detailed analysis: TG)
        \end{itemize}
    \item Mechanism in Llama 2. 
    \item Mechanism in Llama 3.1. \DP{this is substantially easier; the main point is to note that the mechanism presents differently with multiple layers, but the idea carries through.}
    \item Experimental evidence in the pre-training checkpoint of OLMo. \DP{all dynamics results: value state norms, attention weights, and norms of tokens.}
    \end{itemize}
    \item Section 4: Conclusion (TODO: DP)
\end{itemize}


% \begin{itemize}
% \item Prelim, report existing findings.
% \item Linear algebraic mechanism
% \begin{itemize}
% \item Attention concentration (correlation, not massive norm), value anti-concentration.
% \item Birth of sink tokens: mechanism of MLP1, effect of Rope, ...
% \end{itemize}
% \item Dormant head hypothesis
% \begin{itemize}
% \item Dormant head in LlaMa2: L16H25.~\yub{Need a bunch of control experiments.}~\yub{Ideally, find other dormant heads, say still use RedPajama dataset to identify.}
% \item \yub{something else?} (Find more signals for dormant head in LlaMa2.)
% \item \yub{For \emph{every} attention sink head (can use some heuristic method to define what an attention sink head is), can we find sentence to activate it and sentence to deactivate it?}
% \item \yub{Theory? e.g. approximation results for specific kinds of heads with/without attention sink (or BOS token). }
% \item \yub{Any attention head can be modified to a dormant head, which is the same head on some input sequence, and deactivated on some other input sequence (with some separation from the original inputs).}
% \end{itemize}
% \item Pretraining with small transformers and synthetic data
% \begin{itemize}
% \item Dormant head phenomenon in Bietti's experiment
% \begin{itemize}
% \item Attention concentration -> massive norm -> massive activation.~\yub{Any experiments that show this quantitatively?}
% % ~\yub{GPT2 does not use RoPE, so do not expect massive activation. But massive activation paper they report massive activation for GPT2??? LayerNorm also makes standard coordinates special.}
% \end{itemize}
% \item 50-50 mixture of pure Markov transition prediction and pure induction head phenomenon.~\yub{Intuition: In RepICL where every sequence requires the same task (Rep + ridge regression), there is no attention sink. }
% \item \yub{TODO: Try full sequence copying after some special trigger token.}
% \item 50-50 mixture of any two tasks. Can get you more deactivated heads / attention sink.
% \item \yub{Try ReLU transformer on Bietti's experiment.}
% \end{itemize}
% \item Qualitative difference between LlaMa2 and LlaMa3?
% \end{itemize}

% \section*{TODOs}

% \begin{itemize}
%     % \item Conjecture: Where attention sink appears $\approx$ that layer is not very important, does some simple functional. Can we characterize that functional in function space?
%     \item Attention sink $\equiv$ bias (added after QKV)?
%     \begin{align*}
%         \bh_i' = \bh_i + \sum_{j=1}^i \softmax\paren{ (\<\bq_i, \bk_j\>)_{j=1}^i }_j \bv_j \approx \bh_i + \sum_{j=2}^i \softmax\paren{ (\<\bq_i, \bk_j\>)_{j=1}^i }_j \bv_j + \bbb
%     \end{align*}
%     Conjecture: Training an architecture with bias, can alleviate all the unbalancedness, and get rid of the streaming LLM problem.

%     \item Training dynamics of GPT2?
%     \begin{itemize}
%         \item Plot the gradient.
%     \end{itemize}
% \end{itemize}

==> Sections_arxiv/BBM.tex <==
\section{The Bigram-Backcopy Task}\label{sec:bb_task}
The Bigram-Backcopy task consists of two sub-tasks: \textit{Bigram-transition} and \textit{Backcopy}. Each input sequence begins with a \bos~token, followed by tokens sampled according to a pre-determined bigram transition probability $\transit$. When some special trigger tokens are encountered, instead of sampling, the preceding token is copied to the next position. Following \citet{bietti2024birth}, we select the transition $\transit$ and the vocabulary $\vocab$ with $| \vocab | = V = 64$ based on the estimated character-level bigram distribution from the tiny \textit{Shakespeare} dataset. In all experiments, the set of trigger tokens $\cT$ is fixed and consists of the $\abs{\cT}=3$ most frequent tokens in the unigram distribution. Thus, the non-trigger token set, $\vocab\setminus \cT$, comprises $61$ tokens.

\subsection{One-layer transformer shows \attnsink s and \valuedrain s.}

On the \bb~task, we pre-train a standard one-layer transformer with only one softmax \attn~head and one \mlp~layer. Unless otherwise specified, the model is trained with Adam for $10,000$ steps.  We relegate the training details in Appendix \ref{sec:ablations}. Figure \ref{fig:bbm-attn} shows that the trained transformer also exhibits the \attnsink~phenomenon, where the \bos~token captures a significant proportion of the attention weights. More importantly, the attention weights reveal interpretable patterns: all non-trigger tokens exhibit \attnsink s, while the attention for trigger tokens is concentrated on their preceding positions. Furthermore, Figure \ref{fig:bbm-value} reveals a value state drain phenomenon similar to LLMs, indicating that on non-trigger tokens, the \attn~head adds a minimal value to the residual stream. 

\begin{figure}[t]
  \centering
  \begin{minipage}{0.38\textwidth}
      \centering
      \subcaption{\small The Bigram-Backcopy task}
      \label{fig:bbm-dgp}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM/BBM.pdf}
  \end{minipage}
  % \hspace{-1em}
  \begin{minipage}{0.26\textwidth}
      \centering
      \subcaption{\small Attention pattern}
      \label{fig:bbm-attn}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM/attn_fig1.pdf}
  \end{minipage}
  % \hspace{-1em}
  \begin{minipage}{0.27\textwidth}
      \centering
      \subcaption{\small Small value states}
      \vspace{0pt}
      \label{fig:bbm-value}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM/value_states_white.pdf}
  \end{minipage}
  % \vspace{-1em}
  \caption{\small \textbf{Experiments on the Bigram-Backcopy task.} 
  %\sm{Consistently use left (a) instead of reference to self} 
  \textit{Left (a):} We illustrate the data generation procedure for the Bigram-Backcopy task, where we fix 't', 'e', and the space character (' ') as trigger tokens. The BB task samples bigram transitions for non-trigger tokens and backcopies for trigger tokens. \textit{Middle (b):} We present the attention weight heat map of a given prompt, with trigger tokens marked in red. Non-trigger tokens act as attention sinks.  \textit{Right (c):} We plot the value state norms for the prompt, where the \bos~token has a tiny norm.}
  \label{figure:pretraining-findings}
  \vspace{-1em}
\end{figure}

% \begin{figure}[t]
%   \centering
%   \begin{minipage}{0.4\textwidth}
%       \centering
%       \subcaption{\small }
%       \label{fig:pretraining-massive-norm}
%       \vspace{-.2em}
%       \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_copy/dormant_copy_L3_massive.pdf}
%   \end{minipage}
%   \begin{minipage}{0.4\textwidth}
%       \centering
%       \subcaption{\small Small value states norm}
%       \label{fig:pretraining-small-value}
%       \vspace{-.2em}
%       \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_copy/dormant_copy_L3_minor.pdf}
%   \end{minipage}
%   \vspace{-1em}
%   \caption{\small \textbf{The norms of residual states and value states in the Bigram-Backcopy task.} A summary of the norm distributions of the output of layer 1 (Figure \ref{fig:pretraining-massive-norm}) and the value states of layer 2 (Figure \ref{fig:pretraining-small-value}) in a 3-layer transformer trained on the \textit{dormant copy} task. The \bos~token is at the left most, with three trigger tokens ` ', `t', and `e' following it. We then randomly choose six tokens and separately summarize their norm distributions. We pull all other tokens together, forming the distribution of the norms of others at the right most. Only the \bos~and the $\backslash n$ token possess remarkably large output norms and small value states norms.}
%   \label{figure:pretraining-findings-norms}
%   \vspace{-1em}
% \end{figure}

\paragraph{The \activedormant~of the attention head:} Inspired by the observed interpretable attention weight patterns, we propose the \textit{\activedormant}. For any given token, an attention head is considered \textit{active} if it contributes significantly to the residual state, and \textit{dormant} if its contribution is minimal. As illustrated in Figure \ref{fig:bbm-attn}, trained on the BB task, the attention head is active on trigger tokens and dormant on non-trigger tokens. 

Figure \ref{fig:interventions} demonstrates that the \mlp~layer is responsible for the Bigram task whereas the \attn~head takes care of the Backcopy task. When the \mlp~layer is zeroed out, the backcopy loss remains significantly better than a random guess, but the bigram loss degrades to near-random levels. Conversely, when the \attn~layer is zeroed out, the backcopy loss becomes worse than a random guess, while the bigram loss remains unaffected. This suggests that on trigger tokens, the \attn~head is active and handles the backcopy task, whereas on non-trigger tokens, the \attn~head is dormant, allowing the \mlp~layer to handle the Bigram task. We summarize the \activedormant~of the \attn~head in Claim \ref{claim:active-dormant}.

\begin{claim}
\label{claim:active-dormant}
In the BB task, the \attn~head demonstrates \activedormant, alternating between two phases:
\begin{itemize}[leftmargin=2em]
\setlength\itemsep{0pt}
\item \textbf{Dormant phase}: On non-trigger tokens, the \attn~head puts dominant weights to the \bos~token, adding minimal value to the residual stream, having little impact on the model’s output.
\item \textbf{Active phase}: On trigger tokens, the \attn~head puts dominant weights to the relevant context tokens, adding substantial value states to the residual stream, resulting in a significant impact on the model’s output. 
\end{itemize}
\end{claim}

\paragraph{The growth of attention logits on the \bos~token and the decrease in the norm of its value state.} Figure \ref{fig:dynamics} displays the training dynamics of excess risks, attention weights, attention logits, and value state norms for the \bos~token. All values are rescaled to highlight the trends. The backcopy excess risk and the bigram excess risk both drop to zero within the first 1000 steps. As the backcopy risk decreases, the attention weights on the \bos~token increase, suggesting a relationship between the formation of attention sinks and the functional development of the attention heads. For each token $\tok_n$ at position $n$ in the prompt, we compute $\text{logit}_{\bos} = \mathtt{mean}_{n}[\langle \query_{\tok_n}, \key_\bos \rangle - \mathtt{mean}_{i}(\langle \query_{\tok_n}, \key_{\tok_\toki}) \rangle]$, which serves as a progress measure for attention sinks. Even after the attention weights on the \bos~token is nearly $1$, $\text{logit}_{\bos}$ continues to increase. Simultaneously, the norm of the value state of the \bos~token continues to decrease to a small value.

\begin{figure}
  \centering
  \begin{minipage}{0.37\textwidth}
      \centering
      \subcaption{\small Excess risk after interventions}
      \label{fig:interventions}
      % \vspace{-0.5cm}
      \includegraphics[width=\textwidth]{Figures/BBM/interventions.pdf}
  \end{minipage}
  % \hspace{1em}
  \begin{minipage}{0.6\textwidth}
      \centering
      \subcaption{\small Training dynamics }
      \label{fig:dynamics}
    \includegraphics[width=\textwidth]{Figures/BBM/dynamics_combine.pdf}
  \end{minipage}
  \hspace{-1em}
    \caption{\small \textbf{Interventions and dynamics of one-layer transformer on the Bigram-Backcopy task.}  \textit{Left (a)}: We display the excess risks for a one-layer model trained on the Bigram-Backcopy (BB) task under various interventions. \textit{Right (b):} We plot the excess risks, attention weights, attention logits, and value state norms for the \bos~token along the training dynamics. Each curve is rescaled to fall within a 0 to 1 range, though the trends remain consistent without rescaling. On the right side of \textit{(b)}, the horizontal axis is logarithmically scaled. The $\text{logit}_{\bos}$ curve denotes the mean of attention logits from all given non-trigger query tokens $\tok$ on the \bos~token, normalized by the mean of attention logits on other tokens. The shaded area gives the 90\% confidence interval on the distribution over all non-trigger tokens.}
    \label{figure:verify-assumptions}
\end{figure}

\subsection{Analysis of a minimally-sufficient transformer architecture}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/BBM/SimpleModel.pdf}
    \caption{\small \textbf{The simplified transformer architecture with one \mlp-layer and one \attn~head in parallel.} The predicted probability is the softmax of the output. Assume that the trainable variables are $(\vecsink,\vecvalue) \in \R^V \times \R^V$, which stands for the attention logits and value states of the $\bos$ tokens.}
    \label{figure:simple-model}
\end{figure}

In this section, we analyze the training dynamics on the BB task by simplifying the architecture while preserving the attention sinks and value state drains phenomena. Let $\vocab$ denote the set of all tokens except the $\bos$ token, and $\cT$ denote the set of all trigger tokens. Given any $\tok \in \vocab$, we denote $\transition_{\tok\tokk}=\transit(\tokk|\tok)$ to be the next token Markov transition probability, and $\bp_v = [p_{v1}, \ldots, p_{vV}]$ be the row vector in the simplex. We assume that the tokens are embedded into $V$-dimensional space using one-hot encoding, and for notation simplicity, we abuse $v$ to stand for its one-hot encoding vector $\bm{e}_v \in \R^V$ which is a row vector. The predicted probability of the $n+1$ token is given by $\softmax(\TF([\bos; v_{1:n-1}; v])_n)$, where transformer architecture is given by $\TF(\cdot) = \attn(\cdot ) + \mlp(\cdot )$. Here $\attn(\cdot ) = \softmax(\mask(\query(\cdot ) \key(\cdot )^\top )) \vall(\cdot )$ and $(\query, \key, \vall)$ are linear maps from $\R^V \to \R^V$. Since the \mlp~layer could handle the Bigram task, we assume that $\mlp$ outputs the Markov transition probabilities $\bp_v$ on non-trigger tokens $v$ and zero on trigger tokens. For the \attn~head, we assume that the attention logits on the $\bos$ key-token are $(\sink_{v_1}; \ldots; \sink_{v_n})$, the attention logits on any trigger query-token are $(0, \ldots, \lambda, 0)$ where the second last coordinate is $\lambda$, and assume other logits are zero. Assume that the value state of $\bos$ is $\vecvalue \in \R^V$, and the value state of each non-trigger token $\tok$ is a one-hot encoding vector $\bm{e}_\tok$ multiplied by $\xi_\tok \geq 0$. Figure \ref{figure:simple-model} illustrates this simplified transformer architecture. These assumptions are summarized in the following equations. 
\begin{equation}\label{eqn:simplification_TF}
\begin{aligned}
&~ \mlp(\tok) = \log \bp_v \cdot 1\{ \tok \not\in \cT  \} ~~~ \text{for } \tok \in \vocab,\\
&~\langle \query(\tok), \key(\bos) \rangle =\sink_\tok \cdot 1 \{ v \not\in \cT \}~~~\text{for } \tok\in\vocab, \\
&~\langle \query(\tok), \key(\tok') \rangle = \lambda \cdot 1\{ \tok \in \cT, \tok' \text{ is the former token of } \tok \} ~~~\text{for } \tok, \tok' \in \cV, \\
&~ \vall(\tok) = \xi_\tok \bm{e}_\tok  ~~~\text{with $\xi_\tok=0$ for $\tok\in\cT$, and $\xi_\tok\geq 0$ for $\tok\in\vocab\setminus\cT$.}
\end{aligned}
\end{equation}

Theorem \ref{thm:construction} demonstrates the existence of a transformer structure that is equivalent to the simplified version. We relegate the proof in Section \ref{sec:proof}.

\begin{theorem}\label{thm:construction}
For any parameters $(\vecsink \in \R^{V}, \vecvalue \in \R^V, \bm{\xi} \in \R^V, \lambda \in \R)$, there is a one-layer transformer $(\mlp, \query, \key, \vall)$ such that Eq. (\ref{eqn:simplification_TF}) holds. The transformer gives ground truth transition of the BB model if $\min_{v \in \vocab} \sink_v \to\infty$, $\min_{v \in \vocab} \xi_v \to\infty$, $\lambda\to \infty$, and $\vecvalue=0$.
\end{theorem}

% \sm{I am here.} We make further simplifications on the loss function. Given a non-trigger token at position $n$, assume $W=\sum_{i=1}^n \exp \query_n^\top \key_i $. Assume that $W=\sum_{\tokk=1}^\vocabsize W_\tokk$, with each $W_\tokk$ corresponds to the summations from . We assume that they are fixed values and do not depend on the position $n$. %In reality $W\approx N/2$, which is half of the total sequence length. Since token $\tokk$ takes a proportion $\stable_\tokk$ in the stable distribution, $W_\tokk \approx \stable_\tokk W$ on average. 
Throughout we adopt Eq.~(\ref{eqn:simplification_TF}) as our assumption. We further define $W_{\tokk} = \sum_{i = 1}^n 1\{ \tok_i = \tokk \}$, $\bm{W} = (W_1, \ldots, W_V)$, and $W = \sum_{\tokk \in \vocab} W_{\tokk} = n$. Then for a non-trigger token $v$, the output of attention layer with input sequence $[\bos; v_{1:n-1}; v]$ gives (denoting $\xi_{\tokk} = 0$ for $\tokk \in \cT$)
\[
\TF([\bos; v_{1:n-1}; v])_n = \log \bp_v + \frac{e^{\sink_\tok}}{e^{\sink_\tok} + W} \vecvalue + \sum_{\tokk=1}^{\vocabsize} \frac{W_\tokk \xi_\tokk}{e^{\sink_\tok} + W} \cdot \bm{e}_\tokk.
\]
% Combining the above simplifications, we get that
% \[
% \TF([v_{1:n-1}; v])=\Big[\log \transition_{\tok1} + \frac{e^{\sink_\tok}\ivalue_1+W_1\xi_1}{e^{\sink_\tok}+W};\ldots;\log \transition_{\tok\vocabsize} + \frac{e^{\sink_\tok} \ivalue_\vocabsize+W_\vocabsize\xi_\vocabsize}{e^{\sink_\tok}+W}\Big].
% \]
Therefore, on the non-trigger token $\tok$, the cross-entropy loss between the true Markov transition $\bp_\tok$ and predicted transition $\softmax(\TF([\tok_{1:n-1}; \tok])_n)$ is given by
\[
\loss_\tok(\sink_\tok, \vecvalue) = \sum_{\tokk=1}^\vocabsize \transition_{\tok\tokk}\Big\{ \log \Big[ \sum_{\toki=1}^\vocabsize \transition_{\tok\toki} \exp\Big(\frac{e^{\sink_\tok}\ivalue_\toki+W_\toki\xi_\toki}{e^{\sink_\tok}+W}\Big) \Big] - \frac{e^{\sink_\tok}\ivalue_\tokk+W_\tokk\xi_\tokk}{e^{\sink_\tok}+W} - \log \transition_{\tok\tokk} \Big\}.
\]
For simplicity, we neglect the loss on trigger tokens and assume that $(\{ W_i \}_{i \in [V]}, W)$ are fixed across different positions in the input sequences\footnote{We note that \cite{reddy2023mechanistic} makes similar simplification in analyzing induction heads.}, and consider the total loss to be the losses on each non-trigger token averaged with its proportion in the stable distribution $\{\pi_v\}_{v \in \vocab}$, given by
\[
\loss(\vecsink,\vecvalue) = \sum_{\tok \in \vocab \setminus \cT} \stable_\tok \loss_\tok(\sink_\tok, \vecvalue).
\]
% \tianyu{change the summation notation in the proof.}
\begin{theorem}\label{thm:main}
Consider the gradient flow of the loss function $\loss(\vecsink, \vecvalue)$. Assume $\xi_\tok \ge 0$ for any $\tok$, and $\{ W_i \cdot \xi_i \}_{i \in \vocab}$ are not all equal. 
\begin{itemize}[leftmargin=2em]
\setlength\itemsep{0pt}
    \item (Attention logits grow logarithmically reinforced by small value states) Fix $\vecvalue= \beta \cdot \bm{1}$ for a constant $\beta$, and consider the gradient flow over $\vecsink$. With any initial value $\vecsink(0)$, there exists $\bm{r}(t)$ with norm uniformly bounded in time such that 
    \[\vecsink(t) = \frac{1}{2} \log t \cdot \bm{1} + \bm{r}(t).\]
    \item (Value state shrinks to a small constant vector reinforced by large attention logits) Fix $\vecsink = \sink \cdot \bm{1}$ for a constant $\sink$, and define $\bar{\ivalue}(0) = V^\inv[\sum_{\tok} \ivalue_\tok(0)]$. Consider the gradient flow over $\vecvalue$. As $t \to \infty$, we have
    \[\vecvalue(t) \to \vecvalue^\star = \bar\ivalue(0) \cdot \bm{1} - e^{-\sink} \cdot \bm{W}\circ \bm{\xi}.\]
    \item (Stable phase: identical attention logits) Consider the gradient flow over variables $(\vecsink, \vecvalue)$. Any vector of the following form
    \[\vecsink = \sink \cdot \bm{1}, \quad \vecvalue = c \cdot \bm{1} - e^{-\sink} \cdot \bm{W} \circ \bm{\xi},  ~~~ \sink, c\in\R \]
     is a stationary point. These are all global minimizers of $\loss(\vecsink,\vecvalue)$.
\end{itemize}
\end{theorem}
The proof of Theorem~\ref{thm:main} is provided in Appendix~\ref{app:proof-main}. We give three key remarks: (1) As $\sink_\tok\to\infty$, a Taylor expansion of the gradient $\partial \loss/\partial \sink_\tok$ suggests that $\mathrm{d}\sink_\tok/\mathrm{d}t \propto \exp(-2 \sink_\tok)$, which leads to the logarithmic growth of $\sink_\tok$. Similar logarithmic growth exists in the literature under different setups \citep{tian2023scan,han2023lm}. (2) For a fixed $\vecsink=\sink\bm{1}$, under additional assumptions on the initial value $\vecvalue(0)$, we can prove a linear convergence for $\vecvalue$. (3) The stable phase described in Theorem \ref{thm:main} seems to imply that the system could be stable without attention sinks, as it does not require $\sink$ to be large. However, in practice, models trained on the BB task tend to converge to a stable phase where $\sink$ is relatively large. 
% \tianyu{We expect LLMs to converge to the stable phase outlined in Theorem \ref{thm:main} as well.}
% Revisiting Figure \ref{fig:attention_logits_random}, which shows attention logits in Llama 2-7B, the attention logits on the \bos~token appear identical. 
% Thus, we expect LLMs to converge to the stable phase outlined in Theorem \ref{thm:main} as well.

\paragraph{The Formation of Attention Sinks and Value State Drains.} When $\vecvalue = \bm{0}$, the attention logits on the \bos~token increase monotonically. This demonstrates that the presence of a small value state of the \bos~token reinforces the formation of attention sinks. When $\vecsink = \sink \cdot \bm{1}$, with $\sink$ sufficiently large, $\vecvalue(t) \to \bar{\ivalue}(0) \bm{1}$. Given the random Gaussian initialization, $\|\bar{\ivalue}(0) \bm{1}\|_2 \approx \|\vecvalue(0)\|_2 / \sqrt{d}$, where $d$ is the hidden dimension. This demonstrates that the presence of attention sinks reinforces the formation of value states drains.

% \paragraph{combine to the previous paragraph} Although all the $\vecsink=\sink \bm{1}$, $\vecvalue=c\bm{1}-e^{-\sink} \bm{W}\circ \bm{\xi}$ are stable phases. Only the phase with $\vecsink\to \infty$ and $\vecvalue\to c \bm{1}$ can match the oracle algorithm with any out of distribution input. When the value $\sink$ is finite, $\vecvalue$ depends on the value $\bm{W}\approx \bm{\stable} W$, which strongly depends on the stable distribution $\bm{\stable}$. Therefore, if tested with OOD input that has different stable distribution, it cannot match the oracle algorithm.

\paragraph{Experimental verification.} Revisiting Figure \ref{fig:dynamics}, which shows the dynamics of a full transformer model trained with Adam, we observe that both $\text{logit}_{\bos}$ and $\|\vall_{\bos}\|_2$ exhibit growth rates consistent with Theorem \ref{thm:main}. The $\text{logit}_{\bos}$ is equivalent to $\sink$ in this context, as all other attention logits are assumed to be zero under the setup of Theorem \ref{thm:main}. When plotted on a logarithmic scale, the $\text{logit}_{\bos}$ curve grows approximately linearly between 1,000 and 10,000 steps, then accelerates before stabilizing around 100,000 steps.  Meanwhile, the norm of the value state decreases monotonically. The simultaneous increase in attention weights and decrease in value-state norms suggest that these phases occur together during the training process. To further validate Theorem \ref{thm:main}, we construct a simplified model that aligns with Equ. \eqref{eqn:simplification_TF}, and train the parameters $(\vecsink \in \R^{V}, \vecvalue \in \R^V, \bm{\xi} \in \R^V, \lambda \in \R)$ with Adam. The resulting training curves are similar to those of a one-layer transformer, also exhibiting the mutual reinforcement mechanism.

Combining theoretical insights and experimental evidence, we summarize the formation of attention sinks and value state drains as a mutual reinforcement mechanism.

% P = f(X, V_1, V_2) (ground truth). When P is independent of V_1, V_2, f(X, V_1, V_2) = f(X); Assume p = f(x, 0, 0). Now we fit it with p = f(x, a_1 v_1, a_2 v_2). When v_1, v_2 \neq 0, we need to have a_1, a_2 = 0 to make accurate prediction. 

\begin{claim}[Mutual reinforcement mechanism]
For any attention head given a specific prompt, if the model can accurately predict the next token without the attention head, but adding any value state from previous tokens worsens the prediction, the attention head becomes dormant, forming an attention sink, leading to the mutual reinforcement of attention sinks and value state drains: 
\begin{enumerate}[leftmargin=2em]
\setlength\itemsep{0pt}
    \item The SoftMax mechanism pushes the attention weights to the value state drains, reinforcing attention sinks.
    \item The attention sinks on the value state drains further pushes down the value state, reinforcing value state drains.
    % \item The value state drains attract more attention weights, reinforcing the attention sinks.
\end{enumerate} 
The mutual reinforcement stabilizes at the phase when all tokens have identical large attention logits on the value state drains. 
%\sm{This sentence appears here seems weird} \tianyu{I added mutual reinforcement mech}
Finally, due to the causal mask, the training dynamics favor the \bos~token to become an extreme token.
\end{claim}

We expect that the formation of extreme tokens in LLMs follows a similar mutual reinforcement mechanism. Indeed, although Theorem \ref{thm:main} focuses on a specific BB task with a simplified architecture and loss function, the same principles can be applied to more general scenarios. Specifically, for an attention head $\attn$, we assume that $(\text{LLM}\setminus \attn)(\tok) = \log \bm{\transition}_\tok$, meaning that the LLM, even if we zeroed out  $\attn$, can still output an accurate next token prediction. Furthermore, we assume $\val(\tok) = \xi_\tok \bm{e}_\tok$, indicating that adding the value state from any previous tokens performs a specific function. Under these assumptions, we expect the same theoretical results to apply to LLMs. In Section \ref{sec:llm}, we will explore the formation of attention sinks and value state drains along the training dynamics of LLMs, where we find empirical evidence that aligns with the theory. 

\begin{figure}
  \centering
    \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small ReLU attention}
      \label{fig:relu-attn}
      \includegraphics[width=\textwidth]{Figures/BBM/relu_dynamics.pdf}
  \end{minipage}
    \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Interventions on a 3-layer TF}
      \label{fig:massive-interventions}
      \includegraphics[width=\textwidth]{Figures/BBM/massive_interventions.pdf}
  \end{minipage}
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Eliminating
      residual state peaks}
      \label{fig:sgd}
      \includegraphics[width=\textwidth]{Figures/BBM/adam_vs_sgd.pdf}
  \end{minipage}
    \caption{\small \textbf{Experiments on massive norms with multi-layer transformers trained on the Bigram-Backcopy task.} 
    \textit{Left (a):} We present the training dynamics of the ReLU attention for the first 1,000 steps.
    \textit{Middle (b):} We plot the intervention results on the \attn+\mlp+\attn+\mlp+\mlp~structure.
    % Figure \ref{fig:minimal-massive} \sm{no self reference in caption} shows the  $\|\Output(\bos)\|_2$ at layer 0 across different model architectures. 
    \textit{Right (c):} We plot the evolution of massive norms in a three-layer transformer trained with Adam, SGD, and using a ReLU attention structure. Notably, only the three-layer model with softmax attention trained using Adam results in the emergence of residual state peaks. \sm{Figure (c) y label $Res_{<s>}$}\tianyu{looks fine to me?}}
\end{figure}

\paragraph{Replacing SoftMax by ReLU attention removes extreme-token phenomena.} As an implication of our theory, we predict that training with ReLU attention instead of SoftMax attention will eliminate the extreme-token phenomena. Without the SoftMax, the dynamics no longer push the attention weights on the \bos~token, which remains zero along the training dynamics. Without attention sink, the dynamics no longer push down the value state norm, and the mutual reinforcement mechanism breaks. Figure~\ref{fig:relu-attn} illustrates the training experiment on the BB task replacing SoftMax with ReLU, showing that both the Bigram and Backcopy risk match the Bayes risk after 200 training steps, but the attention logits of \bos~do not grow, and the value state does not shrink, confirming the prediction. 

\subsection{The emergence of residual state peaks}
\paragraph{The residual state peaks require a three-layer structure.}  No residual state peaks appear in a one-layer transformer trained on the BB task. We train various models on the BB task and track the \bos~token’s residual state norms after layer $0$. We relegate the experimental results to Appendix \ref{sec:ablations}. We find that a three-layer transformer is enough to produce residual state peaks. 
% In Figure \ref{fig:minimal-massive},  
If we allow to skip some \mlp~or \attn~layers, the ``\attn+\mlp+\attn+\mlp+\mlp'' combination becomes the simplest model that produces residual state peaks (Figure \ref{appfigure:massive_minimal}). Circuit analysis also reveals that LLMs typically add a large vector in the first layer and cancel it in the last layer. We propose that the add-then-cancel mechanism is essential for residual state peaks and requires at least three layers.

\paragraph{Residual state peak reinforces attention sinks and value state drains in trained models.} Figure \ref{fig:massive-interventions} presents the intervention results on the ```\attn+\mlp+\attn+\mlp+\mlp'' model. We recenter the $\|\res_{\bos}\|_2$ by subtracting the average norm of other tokens from the \bos~token norm. The $\text{logit}_{\bos}$ and $\|\val_{\bos}\|$ are computed in layer $1$ following the same ways as in Figure \ref{fig:dynamics}. When layer 0 is zeroed out, the residual norm returns to normal, attention logits decrease, and the value state norm rises. It verifies that the residual state peak contributes to the attention sink and value state drain phenomenon in the trained transformer.

% \paragraph{I plan to put the theory for residual state peaks part in the appendix} To include the 
% To model the dynamics of massive norms, we assume that $\cos(\query_i, \key_0)=1$ for any $i$. The output of the lower layer adds $m \key_0/\ltwo{\key_0}$ on the residual stream of the \bos~token and get $\bh_0+m\key_0$. Assume that $\ltwo{\bh}=1$ and $\cos(\bh, \key_0) = c$. As a result,  

% \paragraph{Conjecture: The \activedormant~and the use of Adam reinforce the linear growth of residual state peaks in dynamics.} Since residual state peaks drive attention sinks and value state drains in trained transformers, we hypothesize that the \activedormant~strengthens their formation. Specifically, when the training dynamics push the attention logits on the \bos~token, it also pushes up the norm of $\attn_0(\bos)$ and $\mlp_0(\bos)$ in layer 0. Due to the layer norm, their gradients shrink quickly, but Adam makes small gradients to be constant updates. Further experiments support the conjecture. Figure \ref{fig:sgd} shows the \bos's residual state norms after layer $0$ of three-layer transformers with different configurations. Adam leads to a linear increase in residual norms. In contrast, with SGD, attention sinks persist, but residual state peaks vanish. The ReLU attention, which lacks the \activedormant, shows no residual peaks. 

\tianyu{I want to keep parts of the original explanations.}
\paragraph{Replacing Adam by SGD removes the linear growth of residual state norm.} Figure \ref{fig:sgd} shows the \bos's residual state norms at the output of layer $0$ of three-layer transformers with different configurations. Adam leads to a linear increase in residual norms. In contrast, with SGD, attention sinks persist, but residual state peaks vanish. The ReLU attention, which lacks the \activedormant, shows no residual state peaks. 
% Therefore, we hypothesize that the \activedormant~strengthens their formation. Specifically, when the training dynamics push the attention logits on the \bos~token, it also pushes up the norm of $\vall_{\bos}$ and $\mlp_{\bos}$ in layer 0. Due to the layer norm, their gradients shrink quickly, but Adam makes small gradients constant updates, leading to a linear increase in residual norms.


% \begin{itemize}
%     \item The attention sinks and value state drains are external manifestations of the active-dormant mechanism in LLMs.
%     \item The attention heads go through the attention-increasing and value-state-shrinking phases. They converge to the stable phase with identical attention logits on the \bos~token.
%     \item The residual state peaks reinforce attention sinks and value state drains. Both the lower layer attentions and MLPs contribute to the residual state peaks.
%     \item The residual states go through linear increasing phase in the pre-training.
% \end{itemize}


% \subsection{Verify the predictions from the theory}





==> Sections_arxiv/abstract.tex <==
\begin{abstract}
We investigate the mechanisms behind three puzzling phenomena observed in transformer-based large language models (LLMs): \textit{attention sinks}, \textit{value-state drains}, and \textit{residual-state peaks}, collectively referred to the \textit{extreme-token phenomena}. \sm{Briefly describe what are these phenomenon, and what is the consequence.} First, we demonstrate that these phenomena also arise in simpler architectures—transformers with one to three layers—trained on a toy model, the Bigram-Backcopy (BB) task. In this setting, we identify an \textit{active-dormant mechanism} that causes attention heads to become attention sinks for certain domain-specific inputs while remaining non-sinks for others. We further develop a precise theoretical characterization of the training dynamics that lead to these phenomena, revealing that they are driven by a \textit{mutual reinforcement mechanism}. By small interventions, we demonstrate ways to avoid extreme-token phenomena during pre-training. Next, we extend our analysis to pre-trained LLMs, including Llama and OLMo, revealing that many attention heads are governed by a similar active-dormant mechanism as in the BB task. We further show that the same mutual reinforcement mechanism drives the emergence of extreme-token phenomena during LLM pre-training. Our results study the mechanisms behind extreme-token phenomena in both synthetic and real settings and offer potential mitigation strategies. % Finally, we offer predictions on removing extreme-token phenomena by adjusting the model architecture and training dynamics, which we validate in the BB task. \tianyu{change it to emphases the interpretability}
\end{abstract}

% \tianyu{old version:}
% Both the training and inference phases in large language models (LLMs) exhibit mysterious phenomena which may affect the model's capability or stability. In this paper, we examine the root cause of three such phenomena which have been empirically shown to occur in trained transformers including LLMs: \textit{attention sinks}, \textit{small value states}, and \textit{massive norms}, which we refer to as \textit{outlier phenomena}. Specifically, we first investigate these phenomena in a toy setting, which we call the Bigram-Backcopy (BB) task, using small one- to three-layer transformers. We develop a precise theoretical characterization, verified through careful experiments, of when and how outlier phenomena occur, and the training dynamics which lead to them in this setting. We then show that our characterization of these phenomena extends to LLMs. We unveil a circuit and training dynamics, both essentially predicted by the BB task, showing how the outlier phenomena occurs in LLMs. In the process, we uncover a so-called \textit{switching mechanism} which ensures that attention heads are attention sinks when the input is text drawn from certain domains, while not being attention sinks for other inputs. Our results reveal the mechanisms behind the ubiquitous outlier phenomena in LLMs.

% We investigate the mechanisms behind three puzzling phenomena observed in transformer-based large language models (LLMs): \textit{attention sinks}, \textit{value-state sinks}, and \textit{residual-state peaks}, collectively referred to the \textit{extreme-token phenomena}. First, we demonstrate that these phenomena also arise in simpler architectures—transformers with one to three layers—trained on a toy model, the Bigram-Backcopy (BB) task. In this setting, we identify an \textit{active-dormant mechanism} that causes attention heads to become attention sinks for certain domain-specific inputs while remaining non-sinks for others. We further develop a precise theoretical characterization of the training dynamics that lead to these phenomena, revealing that they are driven by a \textit{cyclic-reinforcement mechanism}. 

% Next, we extend our analysis to pre-trained LLMs, including Llama and OLMo, revealing that many attention heads are governed by similar active-dormant mechanism as in the BB task. We further show that the same cyclic-reinforcement mechanism drives the emergence of extreme-token phenomena during LLM pre-training. Finally, we offer predictions on how to mitigate extreme-token phenomena by adjusting the model architecture and training dynamics, which we validate in the BB task. 

==> Sections_arxiv/appendices/ablations.tex <==
\section{Ablations}
\label{sec:ablations}

\paragraph{Experimental details.} We train transformers with positional embedding, pre-layer norm, $\softmax$ activation in \attn, and ReLU activation in \mlp. 
We use Adam with constant learning rate $0.0003$, $\beta_1=0.9$, $\beta_2=0.99$, $\eps=10^{-8}$, and a weight decay of $0.01$. We choose a learning rate of $0.03$ for the SGD. In each training step, we resample from the BB task with a batch size of $B=512$ and sequence length $N=256$. Unless otherwise specified, the model is trained for $10,000$ steps. Results are consistent across different random seeds.

\paragraph{More attention plots}: Figure \ref{appfigure:more-attn} presents more attention-weight heat maps of the one-layer transformer model trained on the BB task. All attention maps show the attention sink phenomenon. Interestingly, the trigger tokens serve as attention sinks in some inputs.
\begin{figure}[t]
  \centering
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Sequence 0}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/app_attn_fig1.pdf}
  \end{minipage}
  % \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Sequence 1}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/app_attn_fig2.pdf}
  \end{minipage}
  % \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Sequence 2}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/app_attn_fig3.pdf}
  \end{minipage}
  % \vspace{-1em}
  \caption{\small Attention plots of the one-layer transformer trained on the Bigram-Backcopy task.}
  \label{appfigure:more-attn}
  \vspace{-1em}
\end{figure}

\subsection{Ablations of different model structures trained on the Bigram-Backcopy task.}

\paragraph{Exploring the minimal structure for massive norms.} Figure \ref{appfigure:massive_minimal} presents the difference of residual norms between the \bos~token and others ($\|\res_{\bos}\|-\E_{\tok\neq\bos}[\|\res_{\tok}\|]$), with different combinations of model structures. The $3\times \TF$ and $2\times \TF+\mlp$ are two outliers, showing clear evidence of residual state peaks.

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{Figures/BBM_appendix/massive_norm_minimal.pdf}
    \caption{\small Minimal structures to elicit residual state peaks. We use $A+B+C$ to indicate the model with structure $A$, $B$, $C$ in layers 0, 1, and 2, respectively.}
    \label{appfigure:massive_minimal}
\end{figure}

\paragraph{Attention plots, value state norms, and residual norms for a three-layer transformer trained on BB task.} Figures \ref{appfigure:massive-attn}, \ref{appfigure:massive-value-norm}, and \ref{appfigure:massive-norm} show the extreme token phenomena in a three-layer transformer. The residual state peaks show different phenomena from those in LLMs, with the last layer output increasing the residual norms of non-\bos~tokens. Figure \ref{figure:extreme-token}
 demonstrates that the residual state norms of \bos~drop match the magnitudes of other tokens at the last layer. 
\begin{figure}[t]
  \centering
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Layer 0}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/massive_attn_fig0.pdf}
  \end{minipage}
  % \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Layer 1}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/massive_attn_fig1.pdf}
  \end{minipage}
  % \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Layer 2}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/massive_attn_fig2.pdf}
  \end{minipage}
  % \vspace{-1em}
  \caption{\small Value state norms of three-layer transformer trained on the BB task}
  \label{appfigure:massive-attn}
  \vspace{-1em}
\end{figure}

\begin{figure}[t]
  \centering
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Layer 0}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/value_states_layer_0.pdf}
  \end{minipage}
  % \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Layer 1}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/value_states_layer_1.pdf}
  \end{minipage}
  % \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Layer 2}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/value_states_layer_2.pdf}
  \end{minipage}
  % \vspace{-1em}
  \caption{\small Value state norms of three-layer transformer trained on the BB task}
  \label{appfigure:massive-value-norm}
  \vspace{-1em}
\end{figure}


\begin{figure}[t]
  \centering
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Layer 0}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/norms_layer_0.pdf}
  \end{minipage}
  % \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Layer 1}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/norms_layer_1.pdf}
  \end{minipage}
  % \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Layer 2}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/norms_layer_2.pdf}
  \end{minipage}
  % \vspace{-1em}
  \caption{\small Residual state norms of three-layer transformer trained on the BB task}
  \label{appfigure:massive-norm}
  \vspace{-1em}
\end{figure}

% \paragraph{Exploring the minimal structure for massive norms.} Figure \ref{appfigure:massive_minimal} presents the difference of residual norms between the \bos~token and others ($\|\res_{\bos}\|-\E_{\tok\neq\bos}[\|\res_{\tok}\|]$), with different combinations of model structures. The $3\times \TF$ and $2\times \TF+\mlp$ are two outliers, showing clear evidence of residual state peaks.
\paragraph{Statics and dynamics of the simplified model in Theorem \ref{thm:main}.} With the simplified model structure in Figure \ref{figure:simple-model}, we pre-train the model using Adam with learning rate $0.03$. Figure \ref{appfigure:simple-static} and \ref{appfigure:simple-dynamic} show results that match both the theory and the observations of the one-layer transformer. 

\begin{figure}[t]
  \centering
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Attention weights}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/simple_attn_fig0.pdf}
  \end{minipage}
  % \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Value state norms}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/simple_value_states_layer_0.pdf}
  \end{minipage}
  \caption{\small The simplified model structure trained on the BB task.}
  \label{appfigure:simple-static}
  \vspace{-1em}
\end{figure}

\begin{figure}[t]
  \centering
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small First 1000 steps}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/simple_dynamics.pdf}
  \end{minipage}
  % \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small From 0 to 10000 steps}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/simple_dynamics_logit.pdf}
  \end{minipage}
  \caption{\small The dynamics of the simplified model structure trained on the BB task. \textit{Left (a):} The training curves match the one-layer transformer. \textit{Right (b):} The logit curve is close to the logarithmic growth predicted in Theorem \ref{thm:main}.}
  \label{appfigure:simple-dynamic}
  \vspace{-1em}
\end{figure}

\subsection{Variations of the Bigram-Backcopy task}

\paragraph{Bigram-Backcopy task without the \bos~token.} We train a one-layer transformer on the BB task without the \bos~token. Figure \ref{appfigure:no-bos-extreme} shows that the \bos~token is perhaps not the extreme token. Instead, trigger tokens and delimiter tokens seem to become extreme tokens. The results indicate that initial tokens may not be the only candidates for the extreme token, partially explaining why delimiter tokens could also be extreme tokens in LLMs.
\begin{figure}[t]
  \centering
  \begin{minipage}{0.35\textwidth}
      \centering
      \subcaption{\small Attention weights}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/no_bos_attn_fig0.pdf}
  \end{minipage}
  \begin{minipage}{0.35\textwidth}
      \centering
      \subcaption{\small Value state norms}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/no_bos_value_states_layer_0.pdf}
  \end{minipage}
  % \vspace{-1em}
\caption{\small Attention weights and value state norms of a one-layer transformer trained on the BB task without the \bos~token.}
  \label{appfigure:no-bos-extreme}
  \vspace{-1em}
\end{figure}


\paragraph{The Bigram-Skip-one (BS) task.} We make slight modifications to the Bigram-Backcopy task. On trigger tokens, instead of copying the preceding token, we sample from the bigram-probability of the preceding token $\texttt{P}(\cdot\mid \text{Second-to-last token})$. We train a one-layer transformer on it using the same configuration as the BB task. Figure \ref{appfigure:BS-findings} shows that extreme token phenomena are mitigated. The reason is that trained under BS, both the value states $\vall_\tok$ and the token embedding $\embd_\tok$ give the logit of the bigram transition probability. Therefore, other than having attention sink on the \bos~token, self-attention becomes a new possibility to achieve the active-dormant mechanism.

\begin{figure}[t]
  \centering
  \begin{minipage}{0.38\textwidth}
      \centering
      \subcaption{\small The Bigram-Skip-one task}
      % \label{fig:bbm-dgp}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/BS.pdf}
  \end{minipage}
  % \hspace{-1em}
  \begin{minipage}{0.26\textwidth}
      \centering
      \subcaption{\small Attention pattern}
      % \label{fig:bbm-attn}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/BS_attn.pdf}
  \end{minipage}
  % \hspace{-1em}
  \begin{minipage}{0.27\textwidth}
      \centering
      \subcaption{\small Small value states}
      \vspace{0pt}
      % \label{fig:bbm-value}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/BBM_appendix/BS_value.pdf}
  \end{minipage}
  % \vspace{-1em}
  \caption{\small \textbf{Experiments on the Bigram-Skip-one task.} 
  All phenomena are close to those in the BB task, but with diagonal attention sinks and relatively larger $\|\vall_\bos\|$ compared with Figure \ref{figure:pretraining-findings}.}
  \label{appfigure:BS-findings}
  \vspace{-1em}
\end{figure}




==> Sections_arxiv/appendices/caveats.tex <==
\section{Assorted Caveats}\label{sec:caveats}

\subsection{Multiple Attention Sinks vs. One Attention Sink}\label{sub:multiple_sinks_discussion}

As we have seen, attention heads in the BB task (\Cref{sec:bb_task}), Llama 2-7B-Base (\Cref{sub:active_dormant}), and OLMo (\Cref{sub:olmo_dynamics}) exhibit multiple attention sinks. That is, when heads in these models are dormant, they tend to have two attention sinks. For the LLMs in this group, at least on prose data, the \bos~token as well as the first delimiter token (e.g., representing \texttt{.} or \texttt{;}) are sink tokens. Meanwhile, Llama-3.1-8B-Base (\Cref{sec:llm}) only ever has one attention sink on prose data, and the \bos{} token is always the sink token. Here, we offer a possible explanation of this phenomenon. For the BB task, multiple sink tokens are necessary to solve the task. For LLMs, we believe this distinction may be explained by the relative proportion of coding data, in which delimiters have a greater semantic meaning than prose, within the training set. For instance, OLMo was trained on DOLMA \citep{soldaini2024dolma}, which has around 411B coding tokens. Meanwhile, Llama 2 used at most (2T \(\times\) 0.08 =) 0.16T coding tokens. Finally, Llama 3.1 used around (15.6T \(\times\) 0.17 =) 2.6T coding tokens \citep{dubey2024llama}. On top of the raw count being larger, coding tokens are a larger proportion of the whole pre-training dataset for Llama 3.1 compared to other model families. Thus, during training, the presence of delimiters would not be considered unhelpful towards next-token prediction, since such delimiters carry plenty of semantics in a wide variety of cases. Our earlier hypothesis in \Cref{sub:active_dormant} proposes that only tokens which lack semantics in almost all cases are made to be sink tokens. This could be a reason for the distinction.

\subsection{The Role of a Fixed \bos~ Token in the Active-Dormant Mechanism}\label{sub:fixed_bos}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Figures/bos_study/attn_heads_shuffled.png}
    \caption{\small \textbf{Attention sinks with shuffled input in Layer 24 of OLMo.} In order to understand the impact of positional encodings when there is no \bos{} token, we shuffle the input of the test string ``Summer is warm. Winter is cold.'' in OLMo. We observe that there is still an attention sink on token \(0\), despite it being a random token that does not usually start sentences or phrases (since it is uncapitalized). This shows that the positional embedding, say via RoPE, has a large impact on the formation of attention sinks --- when the semantics of each token have switched positions, the attention sink still forms on the zeroth token.}
    \label{fig:bos_shuffle}
\end{figure}

Some models, such as OLMo, are not trained with a \bos{} token. Despite this, the first token of the input still frequently develops into a sink token. We can study the effect of positional encoding of the tokens on the attention sink phenomenon by shuffling the tokens before inputting them into the transformer, and observing how and why attention sinks form. If we do this with the phrase ``Summer is warm. Winter is cold.'' with OLMo, we observe that at Layer 24, there are many attention sink heads where the first token and first delimiter token share attention mass, even if the sentence is jumbled up and makes no grammatical sense. This points towards the observation that without a \bos{} token, the attention sink formation uses both positional data and, to a greater degree, the semantic data of each token. We leave studying this effect in greater detail to future work.


% \DP{Add ablation experiments with RoPE. It should work since that is the only place which has positional information.}


% \subsection{The attention logits on non-bos tokens decrease through the training dynamics}





==> Sections_arxiv/appendices/circuit.tex <==
\section{Fine-Grained Static Mechanisms for Extreme-Token Phenomena} \label{sec:circuit}

In this section, we will identify more fine-grained static mechanisms for extreme-token phenomena in Llama 3.1-8B-Base. To do this, we identify circuits for the origin of attention sinks and small value states. Then, using ablation studies, we study the origin of massive norms. Again, we use the generic test phrase ``\bos{} Summer is warm. Winter is cold.''

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{Figures/llama_31_circuit/llama_31_attn_l0.png}
    \caption{\small \textbf{A visualization of attention heads at Layer 0 of Llama 3.1-8B-Base.} Notice that many heads have the attention sink property, even at Layer 0 without any cross-token interaction. As usual, the test phrase is ``Summer is warm. Winter is cold.'' The most clear attention sink is Head 31.}
    \label{fig:llama_31_attn_layer0}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
    \caption{Alignment of query states and key states (L0H31).}
        \includegraphics[width=\textwidth]{Figures/llama_31_circuit/llama_31_qk_l0.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\textwidth}
        \caption{Alignment of key states and key states (L0H31).}
        \includegraphics[width=\textwidth]{Figures/llama_31_circuit/llama_31_kk_l0.png}
    \end{subfigure}
    \caption{\small \textbf{Alignment between query states and key states at Layer 0 Head 31 of Llama 3.1-8B-Base.} We observe that the key state of \bos{} is orthogonal to all other key states, and heavily aligned with all query states. Meanwhile, all semantically meaningful (i.e., not delimiter) tokens have aligned key states.}
    \label{fig:llama_31_qk_kk}
\end{figure}

\paragraph{Attention sinks and global contextual semantics.} There are many attention sinks at layer \(0\), and the \bos{} token is always the sink token (see \Cref{fig:llama_31_attn_layer0}). From now on until the end of this section, we \textit{restrict our attention to Head 31 of Layer 0, which is an attention sink.} These attention sinks are caused by two linear-algebraic factors, demonstrated in \Cref{fig:llama_31_qk_kk}.
\begin{enumerate}
    \item The key state of the \bos{} token has small dot product with all other tokens. 
    \item The query states of all tokens are nearly orthogonal to the key states of all tokens except the \bos{} token.
\end{enumerate}
 These two facts combine to ensure that the key state of the \bos{} token is picked out by each query state, causing the attention sink. Since these query and key states are produced without any cross-token interaction, the alignment of different states is caused purely by the token's global importance or meaning imparted via pretraining. The \bos{} token has no semantic meaning in the context of prose tokens, so its key state is not aligned with key states of meaningful prose tokens. Also, delimiter tokens, oft considered secondary attention sinks (c.f.~\Cref{sub:fixed_bos}), have the most aligned key states to the key state of the \bos{} token, and are also the tokens with the least semantic meaning in the prose context. Thus, we identify that, at least in this restricted example, query state and key state alignment depends heavily on the contextual semantics of the token.

 \begin{figure}[h]
     \centering
     \includegraphics[width=0.4\linewidth]{Figures/llama_31_circuit/llama_31_value_states.png}
     \caption{\small \textbf{Value state drains at Layer 0 Head 31 of Llama 3.1-8B-Base.} We observe that the value state associated with \bos{} is already much smaller than every other semantically meaningful token, and still smaller than the delimiter tokens in the same sentence.}
     \label{fig:llama_31_value_states}
 \end{figure}

\paragraph{Value state drains.} The value states of the \bos{} token at Layer \(0\) Head 31 are already near zero, as demonstrated in \Cref{fig:llama_31_value_states}. While the delimiter tokens, which are less semantically meaningful in the prose context, have smaller value states than the rest, they are not as small as the value state of the \bos{} token which is guaranteed to not have any semantics.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{Figures/llama_31_circuit/llama_31_massive_norms.png}
    \caption{\small\textbf{Ablation study on the cause of the residual state peak in Llama 3.1-8B-Base.} We perform a series of ablations to understand which components of the network promote the residual state peaks. We find that ablating either the zeroth or first layer's MLP is sufficient to remove the residual state peak phenomenon, while no other layer-level ablation can do it.}
    \label{fig:enter-label}
\end{figure}

\paragraph{Residual state peaks.} Residual state peaks are caused by the first two layers' MLPs. In particular, we perform several ablations, comparing between the residual state norms in a later layer (\(24\)) of an un-edited forward pass versus forward passes where we force the output of either multiple layers, a single layer, an attention block, or an MLP to be zero (and hence remove its contribution from the residual stream). This intervention showed that ablating \textit{either} Layer 0's or Layer 1's MLP is sufficient to remove the residual state peak. In particular, the second-largest token at Layer 24 in \textit{each} ablation (including the original setup) has norm between \(29\) and \(38\), so the interventions ensure that all tokens have similar size.

% \begin{figure}
%     \centering
%     \begin{subfigure}[t]{0.24\textwidth}
%         \centering 
%         \caption{\small Attention sinks (L0).}
%         \includegraphics[width=\textwidth]{Figures/llama_31_circuit/llama_31_attn_l0.png}
%         \label{fig:llama_31_attn_sink_l0}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.32\textwidth}
%         \centering 
%         \caption{\small Value norms (L0H31).}
%         \includegraphics[width=\textwidth]{Figures/llama_31_circuit/llama_31_value_l0.png}
%         \label{fig:llama_31_v_l0}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.49\textwidth}
%         \centering 
%         \caption{\small Correlations between query/key states (L0H31).}
%         \includegraphics[width=0.49\textwidth]{Figures/llama_31_circuit/llama_31_qk_l0.png}
%         \includegraphics[width=0.49\textwidth]{Figures/llama_31_circuit/llama_31_kk_l0.png}
%         \label{fig:llama_31_qk_kk_l0}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.24\textwidth}
%         \centering 
%         \caption{\small Res.~stream ablations.}
%         \includegraphics[width=\textwidth]{Figures/llama_31_circuit/llama_31_massive_norm.png}
%         \label{fig:llama_31_resid_l0}
%     \end{subfigure}
    
%     %\includegraphics[width=0.5\linewidth]{}
%     \caption{\small \textbf{A circuit for extreme-token phenomena in Llama 3.1-8B-Base.} \textit{Top:} Attention sinks present in Layer 0. \textit{Left:} Value states of tokens which are semantically irrelevant for prose are small, and the \bos{} token (which is always semantically irrelevant) is the smallest. Since these value states are in the zeroth layer, they have not been computed via any cross-token interaction, so this is a result about how tokens align with the value weight matrix as per their usefulness. \textit{Middle:} In the first layer, attention sinks form because key states of semantically irrelevant tokens are correlated with all query states, while other key states are nearly orthogonal to all query states. Meanwhile, all semantically relevant key states are nearly orthogonal to semantically irrelevant key states, and are very aligned with each other. Again, the query and key states were computed in the zeroth layer and so without any previous cross-token interaction, so this shows how the zeroth-layer query and key weight matrices align to tokens depending on their semantic meaning as inferred by pre-training. \textit{Right:} Residual state peaks are present due to the MLPs in the first two layers: ablating either of them by manually removing their contribution to the residual stream is sufficient to remove the residual-state peaks, but ablating any other components will preserve the residual state peak phenomenon. % Evidence of a circuit for massive norm, attention sink, value states in Llama 3.1
%     %\DP{TODO: left figure is show a few attention heatmaps, like 4 or 8; middle figure is show Q dot K, K dot K, and value norms; right figure is residual norm}
%     }
%     \label{fig:llama_31_circuits}
% \end{figure}


==> Sections_arxiv/appendices/extra_heads.tex <==
\section{More Attention Heads in Dormant and Active Phase}\label{sec:more_heads}

In this section, we present two more dormant- and active- phase heads in Llama 2-7B-Base, in \Cref{fig:llama_l16h20,fig:llama_l16h28}, which are more difficult to interpret than Layer 16 Head 25, but go dormant on some inputs and active on others. 

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{0.475\textwidth}
        \centering 
        \caption{}
        \includegraphics[width=\linewidth]{Figures/L16H20/github.png}
        \includegraphics[width=\linewidth]{Figures/L16H20/wikipedia.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.475\textwidth}
        \centering 
        \caption{}
        \includegraphics[width=\linewidth]{Figures/L16H20/intervention.pdf}
    \end{subfigure}
    \caption{\small \textbf{Layer 16 Head 20 of Llama 2-7B-Base.}}
    \label{fig:llama_l16h20}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.475\textwidth}
        \centering
        \caption{}
        \includegraphics[width=\linewidth]{Figures/L16H28/github.png}
        \includegraphics[width=\linewidth]{Figures/L16H28/wikipedia.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.475\textwidth}
        \centering
        \caption{}
        \includegraphics[width=\linewidth]{Figures/L16H28/intervention.pdf}
    \end{subfigure}
    \caption{\small \textbf{Layer 16 Head 28 of Llama 2-7B-Base.}}
    \label{fig:llama_l16h28}
\end{figure}




==> Sections_arxiv/appendices/proof.tex <==
\section{Proofs}
\label{sec:proof}
% \subsection{More Detailed Notation}\label{sub:app_notation}

% As our investigation will become more detailed and in-depth, we introduce a more detailed notation system than that which was provided in \Cref{sub:prelim}.

% \paragraph{Basic notation.} For a finite set \(\gX\), we denote the set of probability distributions on \(\gX\) as \(\Delta(\gX)\). For two matrices \(\bX, \bY\) of the same size, we denote their element-wise product by \(\bX \odot \bY\).

% \paragraph{Notation for our setup.} We consider a transformer-based autoregressive language model as a function \(\mathrm{LM} \colon \gV^{N} \to \Delta(\gV)\), where \(\gV\) is the vocabulary and \(N\) is the sequence length. Here \(\Delta(\gV)\) denotes the estimated probability distribution of token \(N\) given tokens \(0\) through \(N - 1\). An autoregressive language model is composed of a \textit{tokenizer} \(\mathrm{Tok} \colon \gV^{N} \to \R^{D \times N}\), where \(D\) is the token dimension, a \textit{transformer} neural network \(\TF \colon \R^{D \times N} \to \R^{D \times N}\), and a \textit{classification head} \(\mathrm{Cls} \colon \R^{D \times N} \to \Delta(\gV)\), such that 
% \begin{equation}
%     \mathrm{LM} = \mathrm{Cls} \circ \TF \circ \mathrm{Tok}.
% \end{equation}
% In this paper, we focus mainly on the transformer component of the language model. As a deep neural network, we can write the transformer as a composition of \(L\) layers, i.e., 
% \begin{equation}
%     \TF = \mathrm{Layer}^{L - 1} \circ \cdots \circ  \mathrm{Layer}^{0}.
% \end{equation}
% Each layer (\(\mathrm{Layer}^{\ell} \colon \R^{D \times N} \to \R^{D \times N}\)) can be further decomposed into a \textit{self-attention block} (\(\Attn^{\ell} \colon \R^{D \times N} \to \R^{D \times N}\)) and
% a \textit{multi-layer perceptron} (\(\MLP^{\ell} \colon \R^{D \times N} \to \R^{D \times N}\)), defined as follows. Let \(D_{\sf attn} \doteq D / K\), and let \(\phi \colon \R^{N \times N} \to \R^{N \times N}\) be the column-wise softmax, i.e., 
% \begin{equation}
%     \phi(\mat{C})_{ij} = \frac{e^{C_{ij}}}{\sum_{i^{\prime} = 0}^{N - 1}e^{C_{i^{\prime}j}}}, \qquad \forall \mat{C} \in \R^{N \times N}.
% \end{equation}
% Let \(\mathrm{RoPE}^{\ell} \colon \R^{D_{\sf attn} \times N} \to \R^{D_{\sf attn} \times N}\) be the rotary positional embedding \citep{su2024roformer} at layer \(\ell\). Then we have
% \begin{align}\label{eq:attn_def}
%     \Attn^{\ell}(\bH) 
%     &\doteq \bH + \sum_{k = 0}^{K - 1}\bO_{k}^{\ell}(\bV_{k}^{\ell}\bH)\bA_{k}^{\ell}(\bH), \qquad \forall \bH \in \R^{D \times N} \\ 
%     \text{where} \quad  \bA_{k}^{\ell}(\bH) 
%     &\doteq \phi\left(\frac{\mathrm{RoPE}^{\ell}(\bK_{k}^{\ell}\bH)^{\top}\mathrm{RoPE}^{\ell}(\bQ_{k}^{\ell}\bH)}{\sqrt{D_{\sf attn}}}\right), \qquad \forall \bH \in \R^{D \times N},
% \end{align}
% where \(\bQ_{k}^{\ell}, \bK_{k}^{\ell}, \bV_{k}^{\ell} \in \R^{D_{\sf attn} \times D}, \bO_{k}^{\ell} \in \R^{D \times D_{\sf attn}}, \theta^{\ell} \in \R\) are parameters of the network for each \(k \in [K], \ell \in [L]\).

% Now, let \(\silu \colon \R^{D_{\sf mlp} \times N} \to \R^{D_{\sf mlp} \times N}\) be the element-wise SiLU function \citep{ramachandran2017searching}. Then we have
% \begin{align}\label{eq:mlp_def}
%     \MLP^{\ell}(\bH) 
%     &\doteq \bH + \Wdown^{\ell} (\silu(\Wgate^{\ell}\bH + \bgate^{\ell}\mathbf{1}^{\top}) \odot (\Wup^{\ell}\bH + \bup^{\ell}\mathbf{1}^{\top})) \\ 
%     &\qquad\ + \bdown^{\ell}\mathbf{1}^{\top},\qquad \forall \bH \in \R^{D \times N}.
% \end{align}
% Here, \(\Wup^{\ell}, \Wgate^{\ell} \in \R^{D_{\sf mlp} \times D}, \bup^{\ell}, \bgate^{\ell} \in \R^{D_{\sf mlp}}, \Wdown^{\ell} \in \R^{D \times D_{\sf mlp}}, \bdown^{\ell} \in \R^{D}\) are network parameters for each \(\ell \in [L]\). Each layer then just writes 
% \begin{equation}
%     \mathrm{Layer}^{\ell} = \MLP^{\ell} \circ \Attn^{\ell}
% \end{equation}
% Let the \textit{input} to layer \(\ell\) be \(\bH^{\ell} = [\bh_{1}^{\ell}, \dots, \bh_{N}^{\ell}] \in \R^{D \times N}\), and the \textit{input} to the MLP block in layer \(\ell\) be \(\bH_{+}^{\ell} = [\bh_{+1}^{\ell}, \dots, \bh_{+N}^{\ell}] \in \R^{D \times N}\), so that layer \(\ell\) maps \(\bH^{\ell}\) to \(\bH^{\ell + 1}\), like so:
% \begin{equation}
%     \mathrm{Layer}^{\ell} \colon \bH^{\ell} \xrightarrow{\hspace{1em}\Attn^{\ell}\hspace{1em}} \bH_{+}^{\ell} \xrightarrow{\hspace{1em}\MLP^{\ell}\hspace{1em}} \bH^{\ell + 1}.
% \end{equation}
% In this notation, observations in previous works can be written succintly as follows.
% \begin{itemize}
%     \item The ``massive activation'' phenomenon in \citet{sun2024massive} is that some hidden states \(H_{ij}^{\ell}\) have very large magnitudes, i.e., \(\abs{H_{ij}^{\ell}} \gg 1\), for layers \(\ell \geq 2\).
%     \item The ``attention sink'' phenomenon in \citet{xiao2023efficient} is that \(\sum_{i = 0}^{N - 1}A_{k}^{\ell}(\bH^{\ell})_{i 0} \approx 1\), for some \((k, \ell) \in [K] \times [L]\).
% \end{itemize}
Since we drop the trigger tokens in the loss function, we neglect $\cT$ throughout the proof for notational convenience, assuming that $\vocab$ consists of only non-trigger tokens.
We provide new notations which are frequently used in the proofs. Define the full bigram transition probability. 
\begin{equation}\label{appeqn:P-matrix}
\Transition = \left(\begin{matrix}
\transition_{11} & \ldots & \transition_{1\vocabsize}\\
\vdots & \ddots & \vdots \\
\transition_{\vocabsize 1} & \ldots & \transition_{\vocabsize\vocabsize}\\
\end{matrix}\right) = \left(\begin{matrix}
\bm{\transition}_1^\top\\
\vdots \\
\bm{\transition}_\vocabsize^\top\\
\end{matrix}\right).
\end{equation}
Given token $\tok$, define the predicted probability, which is the logit output passed through the softmax activation 
\begin{equation}\label{appeqn:pred-prob}
\bm{\ppred}_{\tok} = \softmax(\TF([\bos; v_{1:n-1}; v])_n).
\end{equation}
Similarly, define the full output probability matrix.
\begin{equation}\label{appeqn:Q-matrix}
\Ppred = \left(\begin{matrix}
\ppred_{11} & \ldots & \ppred_{1\vocabsize}\\
\vdots & \ddots & \vdots \\
\ppred_{\vocabsize 1} & \ldots & \ppred_{\vocabsize\vocabsize}\\
\end{matrix}\right) = \left(\begin{matrix}
\bm{\ppred}_1^\top\\
\vdots \\
\bm{\ppred}_\vocabsize^\top\\
\end{matrix}\right).
\end{equation}
Given any vector $\bm{u}=[u_1;\ldots;u_d]$, define the corresponding diagonal matrix as
\[
\diag(\bm{u}) = \left(\begin{matrix}
u_{1} & 0 & \ldots & 0\\
\vdots & \ddots &  & \vdots \\
\vdots & & \ddots & \vdots \\
0 & \ldots & 0 & u_d \\
\end{matrix}\right).
\]
Define 
\[
\gppred_\tok^{\Ppred} = \diag(\bm{\ppred}_\tok) - \bm{\ppred}_\tok \bm{\ppred}_\tok^\top \quad \gppred_\tok^{\Ppred} = \diag(\bm{\transition}_\tok) - \bm{\transition}_\tok \bm{\transition}_\tok^\top.
\]
Denote $\bm{z} = W \cdot \vecvalue - \bm{W} \circ \bm{\xi}$. We present a technical lemma.
\begin{lemma}\label{appthm:positive-definite}
The matrices $\gppred^\Transition_\tok$ and $\gppred^\Ppred_\tok$ are positive semi-definite for any $\tok$.
\end{lemma}
\begin{proof}
Since we have that $\sum_{\tokk=1}^\vocabsize \transition_{\tok\tokk} = 1$ and $\sum_{\tokk=1}^\vocabsize \ppred_{\tok\tokk} = 1$ for any $\tok$,
\begin{align*}
(\gppred^\Transition_\tok)_{\toki\toki}=\transition_\toki - \transition_{\toki}^2 & = \transition_\toki(\sum_{\tokk\neq\toki} \transition_\tokk) \geq \sum_{\tokk\neq\toki} |(\gppred^\Transition_\tok)_{\toki\tokk}| \\
(\gppred^\Ppred_\tok)_{\toki\toki}=\ppred_\toki - \ppred_{\toki}^2 & = \ppred_\toki(\sum_{\tokk\neq\toki} \ppred_\tokk) \geq \sum_{\tokk\neq\toki} |(\gppred^\Ppred_\tok)_{\toki\tokk}|.
\end{align*}
This shows that both $\gppred^\Transition_\tok$ and $\gppred^\Ppred_\tok$ are diagonally dominant matrices. By Corollary 6.2.27 in \citet{horn2012matrix}, they are positive semi-definite.
\end{proof}

\subsection{Proof of Theorem \ref{thm:construction}}\label{app:proof-construction}
We denote the hidden dimension as $d$ and the sequence length as $N$. We begin with the assumption regarding the transformer's positional embedding:
\begin{assumption}\label{ass:linear_indp}
For any token $\tok$ and position $\toki$, assume that the encoding combined with the positional embedding ensures that $\set{\embd(\tok_\toki)}$ is linearly independent.
\end{assumption}
Assumption \ref{ass:linear_indp} requires that $d\geq \vocabsize N$. Given the fact that there are  $O(\exp(d))$ approximately linearly independent vectors for large $d$ \citep{vershynin2018high}, it is possible to apply approximation theory to avoid Assumption \ref{ass:linear_indp}. However, since Assumption \ref{ass:linear_indp} pertains only to the construction of $\lambda$ for trigger tokens and is unrelated to Theorem \ref{thm:main}, we adopt it to simplify the proof of Theorem \ref{thm:construction}.

\begin{proof}
%  We concatenate the one-hot encoding $\bm{e}_\tok$ with $d-\vocabsize$ zeros, augmenting it to $\bm{e}_\tok\in\R^d$. Define the positional embeddings as $\Pos_\toki = [\bm{0}_{\vocabsize+1}; \br_\toki]$ for $\toki=0,\ldots,N$, with $\br_\toki \in \R^{d-\vocabsize-1}$ The input of the attention layer becomes 
% \[
% \embd(\tok_\toki) = \bm{e}_{\tok_\toki} + \Pos_\toki.
% \] 
% We define a matrix $\bA\in \R^{d\times d}$ such that $\bA\Pos_{\toki} = \Pos_{\toki-1}$ for $\toki\in[N]$ and $A \bm{e}_\tok=0$ for any $\tok\in\vocab$. Since $\{\bm{e}_\tok,\Pos_{\toki}\}_{\tok\in\vocab,\toki\leq N}$ is linear independent, the existence is guaranteed. Similarly, we define a matrix $\bB \in \R^{d\times d}$ such that $\bB \embd(\tok_{\toki}) = \bm{0}$ for any $\tok_\toki\in\cT$, $\bB \bm{e}_\tok = 0$ for any $\tok\in\vocab\setminus \cT$, and $(\lambda-1) \Pos_{\tokj}^\top \bB \Pos_{\toki} + \sink \Pos_{\tokj}^\top \bB \bm{e}_{\bos}=0$. \tianyu{check}
% Define the value, key, and query matrices as 
% \[
% V = \sum_{\tok\in\vocab\setminus\cT}
% \]

% Then, we have that 
% We augment the one-hot encoding $\bm{e}_\tok$ to $\R^d$, concatenating it with $d-\vocabsize$ zeros. 
Consider vectors $\bu_{i}\in\R^d$, $i\in[N]$ such that $\bu_i^\top\bu_j=0$, $i\neq j$, and $\bu_i^\top\embd(\tok_j)$ for any $\tok\in\vocab$ and $i$, $j\in[N]$.
Adopting Assumption \ref{ass:linear_indp}, there exists a matrix $\query$ such that
\begin{equation}\label{appeqn:mlp-construct}
\begin{aligned}
&~\query(\embd(\tok_i)) = \lambda\bu_{i-1}~~~\text{for }\tok_i\in\cT,~~i>1,\\
&~\query(\embd(\tok_i)) = \sink_{\tok_i} \bu_{0}~~~\text{for }\tok_i\in\vocab\setminus\cT,~~i>0.\\
\end{aligned}
\end{equation}
Define the corresponding key matrix.
\begin{equation}
\begin{aligned}
&~\key(\embd(\tok_i)) =  \bu_{i}~~~\text{for }\tok_i\in\vocab,~~i> 0,\\
&~\key(\embd(\bos)) = \bu_{0}.
\end{aligned}
\end{equation}
There exists a value matrix $\val{}$ such that
\begin{equation}
\begin{aligned}
&~\val(\embd(\tok_i)) = 0~~~\text{for }\tok_i\in\cT,~~i> 1,\\
&~\val(\embd(\tok_i)) = \xi_{\tok_i}\bu_{i}~~~\text{for }\tok_i\in\vocab\setminus\cT,~~i> 0,\\
&~\val(\embd(\bos)) = \vecvalue.\\
\end{aligned}
\end{equation}
Further define the matrix $\bM$ that satisfies
\begin{equation}
\begin{aligned}
&~ \bM (\embd(\tok_i)) = \log \bp_{\tok_i} \cdot 1\{ \tok_i \not\in \cT  \}  ~~~ \text{for } \tok_i \in \vocab,~~i\in[N],\\
&~ \bM  (\bu_i) = \bm{e}_i ~~~ \text{for }i\in[N].
\end{aligned}
\end{equation}
Setting $\mlp(\cdot)=\text{ReLU}(\bM (\cdot))$, we can then verify that the residual connection gives that $\TF([\bos; v_{1:n-1}; v_n])=\mlp(\embd(\tok_n)+\attn(\embd(\tok_n)))$, which is equivalent to the simplified model. 

When $\min_{v \in \vocab} \sink_v \to\infty$, $\min_{v \in \vocab} \xi_v \to\infty$, $\lambda\to \infty$, and $\vecvalue=0$, if $v_n\in\cT$, $\softmax[\TF([\bos; v_{1:n-1}; v_n])] = \delta_{\tok_{n-1}}$. If $\tok_{n}\in\vocab\setminus\cT$, $\softmax[\TF([\bos; v_{1:n-1}; v_n])] = \bm{\transition}_{\tok_n}$. All next-token probabilities match those in the data-generating procedure, aligning with the oracle algorithm.
\end{proof}

\subsection{The stable phase in  Theorem \ref{thm:main}}\label{app:proof-main}

Lemma \ref{appthm:g-ppred} computes the gradient of $\Ppred$.
\begin{lemma}\label{appthm:g-ppred} 
We have
\begin{align*}
\frac{\partial \ppred_{\toki\tokk}}{\partial \sink_\tok} = &~ \frac{\bm{1}\{\toki=\tok\} \ppred_{\toki\tokk}e^{\sink_\toki}}{(e^{\sink_\toki}+W)^2} \Big[W\ivalue_\tokk-W_\tokk \xi_\tokk - \sum_{\tokj=1}^\vocabsize \ppred_{\toki\tokj} (W\ivalue_\tokj - W_\tokj\xi_\tokj)\Big],\\
\frac{\partial \ppred_{\toki\tokk}}{\partial \ivalue_\tok} = &~ \frac{e^{\sink_\toki}}{e^{\sink_\toki}+W}[\ppred_{\toki\tokk}\bm{1}\{\tokk=\tok\} - \ppred_{\toki\tokk}\ppred_{\toki\tok}].\\
\end{align*}
Furthermore,
\[
\sum_{\tokk=1}^\vocabsize \frac{\partial \ppred_{\toki\tokk}}{\partial \sink_\tok} = 0, \quad \sum_{\tok=1}^\vocabsize \frac{\partial \ppred_{\toki\tokk}}{\partial \ivalue_\tok} = 0.
\]
\end{lemma}
\begin{proof}
We repeatedly use the following two facts:
\begin{align*}
\frac{\partial\Big\{\exp\Big[\frac{W_\tokk\xi_\tokk+e^{\sink_\toki}\ivalue_\tokk}{e^{\sink_\toki}+W}\Big]\Big\}}{\partial \sink_\tok} = &~ \frac{\bm{1}\{\toki=\tok\}e^{\sink_\toki}(W\ivalue_\tokk-W_\tokk\xi_\tokk)}{(e^{\sink_\toki}+W)^2} \exp\Big[\frac{W_\tokk\xi_\tokk+e^{\sink_\toki}\ivalue_\tokk}{e^{\sink_\toki}+W}\Big],
\nonumber\\
\frac{\partial\Big\{\exp\Big[\frac{W_\tokk\xi_\tokk+e^{\sink_\toki}\ivalue_\tokk}{e^{\sink_\toki}+W}\Big]\Big\}}{\partial \ivalue_\tok} = &~ \frac{\bm{1}\{\tokk=\tok\}e^{\sink_\toki}}{e^{\sink_\toki}+W} \exp\Big[\frac{W_\tokk\xi_\tokk+e^{\sink_\toki}\ivalue_\tokk}{e^{\sink_\toki}+W}\Big].
\nonumber
\end{align*}

When $\toki\neq \tok$, $\ppred_{\toki\tokk}$ does not include $\sink_\tok$, making the gradients as zero. When $\toki=\tok$, we have
\begin{align*}
\frac{\partial \ppred_{\tok\tokk}}{\partial \sink_\tok} = &~ \ppred_{\tok\tokk} e^{\sink_\tok} \Big[\frac{W\ivalue_\tokk-W_\tokk\xi_\tokk}{(e^{\sink_\tok}+W)^2}\Big] - \frac{\ppred_{\tok\tokk}\sum_{\toki=1}^\vocabsize \transition_{\tok\toki} e^{\sink_\tok} \Big[\frac{W\ivalue_\toki-W_\toki\xi_\toki}{(e^{\sink_\tok}+W)^2}\Big]\exp\Big[\frac{W_\toki\xi_\toki+e^{\sink_\tok}\ivalue_\toki}{e^{\sink_\tok}+W}\Big]}{\sum_{\toki=1}^\vocabsize \transition_{\tok\toki}\exp\Big[\frac{W_\toki\xi_\toki+e^{\sink_\tok}\ivalue_\toki}{e^{\sink_\tok}+W}\Big]}\\
= &~ \frac{e^{\sink_\tok}}{(e^{\sink_\tok}+W)^2} \Big\{ \ppred_{\tok\tokk} [W\ivalue_\tokk-W_\tokk \xi_\tokk] - \ppred_{\tok\tokk}\sum_{\tokj=1}^\vocabsize \ppred_{\tok\tokj} (W\ivalue_\tokj - W_\tokj\xi_\tokj)\Big\},
\end{align*}
and
\begin{align*}
\frac{\partial \ppred_{\toki\tokk}}{\partial \ivalue_\tok} = &~ \Big[\frac{e^{\sink_\toki}}{e^{\sink_\toki}+W}\Big]\ppred_{\toki\tokk} \bm{1}\{\tokk=\tok\} - \frac{\Big[\frac{e^{\sink_\toki}}{e^{\sink_\toki}+W}\Big]\transition_{\toki\tok}\exp\Big[\frac{W_\tok\xi_\tok+e^{\sink_\toki}\ivalue_\tok}{e^{\sink_\toki}+W}\Big]\transition_{\toki\tokk}\exp\Big[\frac{W_\tokk\xi_\tokk+e^{\sink_\toki}\ivalue_\tokk}{e^{\sink_\toki}+W}\Big]}{\Big(\sum_{j=1}^\vocabsize \transition_{\toki\tokj}\exp\Big[\frac{W_\tokj\xi_\tokj+e^{\sink_\toki}\ivalue_\tokj}{e^{\sink_\toki}+W}\Big]\Big)^2}\\
= &~ \Big[\frac{e^{\sink_\toki}}{e^{\sink_\toki}+W}\Big] [ \ppred_{\toki\tokk} \bm{1}\{\tokk=\tok\} - \ppred_{\toki\tokk} \ppred_{\toki\tok} ].
\end{align*}
We can verify that 
\begin{align*}
\sum_{\tokk=1}^\vocabsize \frac{\partial \ppred_{\toki\tokk}}{\partial \sink_\tok} = &~  \frac{e^{\sink_\tok}}{(e^{\sink_\tok}+W)^2} \sum_{\tokk=1}^\vocabsize \Big\{ \ppred_{\tok\tokk} [W\ivalue_\tokk-W_\tokk \xi_\tokk] - \ppred_{\tok\tokk}\sum_{\tokj=1}^\vocabsize \ppred_{\tok\tokj}^\top (W\sink_\tokj - W_\tokj\xi_\tokj)\Big\}\\
= &~ \frac{e^{\sink_\tok}}{(e^{\sink_\tok}+W)^2}  \Big\{\sum_{\tokk=1}^\vocabsize \ppred_{\tok\tokk} [W\ivalue_\tokk-W_\tokk \xi_\tokk] - \sum_{\tokj=1}^\vocabsize \ppred_{\tok\tokj}^\top (W\sink_\tokj - W_\tokj\xi_\tokj)\Big\}\\
= &~ 0,
\end{align*}
and
\begin{align*}
\sum_{\tok=1}^\vocabsize \frac{\partial \ppred_{\toki\tokk}}{\partial \ivalue_\tok} = &~   \Big[\frac{e^{\sink_\toki}}{e^{\sink_\toki}+W}\Big] \sum_{\tok=1}^\vocabsize [\ppred_{\toki\tokk} \bm{1}\{\tokk=\tok\} - \ppred_{\toki\tokk} \ppred_{\toki\tok} ]\\
= &~ \Big[\frac{e^{\sink_\toki}}{e^{\sink_\toki}+W}\Big] [\ppred_{\toki\tokk} - \ppred_{\toki\tokk} ]\\
= &~ 0.
\end{align*}
This finishes the proof of Lemma \ref{appthm:g-ppred}.
\end{proof}

Proposition \ref{appthm:gradients} computes the gradient of $\loss$ with respect to $\vecsink$ and $\vecvalue$, giving the gradient flow.
\begin{proposition}\label{appthm:gradients}
The gradient flow of optimizing $\loss(\vecsink, \vecvalue)$ is given by
\begin{align*}
\dot{\sink}_\tok(t) & = \frac{\stable_\tok e^{\sink_\tok}}{(e^{\sink_\tok}+W)^2} 
\sum_{\toki=1}^\vocabsize({\transition}_{\tok\toki}-{\ppred}_{\tok\toki})(W\ivalue_\toki-W_\toki\xi_\toki),\\
\dot{\ivalue}_\tok(t) & = \sum_{\tokk=1}^\vocabsize \Big\{\frac{\stable_\tokk e^{\sink_\tokk} [\transition_{\tokk\tok} - \ppred_{\tokk\tok}]}{e^{\sink_\tokk}+W}\Big\}.
\end{align*}
\end{proposition}
\begin{proof}
The gradient flow gives that
\[
\dot{\sink}_\tok(t) = - \frac{\partial \loss(\vecsink,\vecvalue)}{\partial \sink_\tok}, \quad \text{and}\quad \dot{\ivalue}_\tok(t)=-\frac{\partial\loss(\vecsink, \vecvalue)}{\partial \ivalue_\tok}.
\]
Taking the derivative of $\loss(\vecsink,\vecvalue)$ gives that
\begin{align*}
\frac{\partial \loss(\vecsink,\vecvalue)}{\partial \sink_\tok}
= ~& \stable_\tok \sum_{\tokk=1}^\vocabsize \transition_{\tok\tokk} \cdot \frac{-1}{\ppred_{\tok\toki}}\cdot \frac{\partial \ppred_{\tok\toki}}{\partial \sink_\tok}\\
= ~& \frac{\stable_\tok e^{\sink_\tok}}{(e^{\sink_\tok}+W)^2} \Big\{  \sum_{\toki=1}^\vocabsize \ppred_{\tok\toki} [W\ivalue_\toki - W_\toki \xi_\toki] - \sum_{\tokk=1}^\vocabsize \transition_{\tok\tokk} [W\ivalue_\tokk-W_\tokk\xi_\tokk]\Big\}\\
= ~& \frac{\stable_\tok e^{\sink_\tok}}{(e^{\sink_\tok}+W)^2} \sum_{\tokk=1}^\vocabsize \Big\{  [\ppred_{\tok\tokk}-\transition_{\tok\tokk}] [W\ivalue_\tokk-W_\tokk\xi_\tokk]\Big\}.
\end{align*}
Similarly, we have that
\begin{align*}
\frac{\partial \loss(\vecsink,\vecvalue)}{\partial \ivalue_\tok} 
= ~& \sum_{j=1}^\vocabsize \stable_\tokj \sum_{\tokk=1}^\vocabsize \transition_{\tokj\tokk} \Big\{ \frac{e^{\sink_\tokj} \ppred_{\tokj\tok}}{e^{\sink_\tokj}+W} - \frac{e^{\sink_\tokj} \bm{1}\{\tokk=\tok\}}{e^{\sink_\tokj}+W} \Big\}\\
= ~& \sum_{j=1}^\vocabsize \Big\{\frac{\stable_{\tokj}e^{\sink_\tokj}[\ppred_{\tokj\tok}-\transition_{\tokj\tok}]}{e^{\sink_\tokj}+W}\Big\}.
\end{align*}
This proves Proposition \ref{appthm:gradients}.
\end{proof}
% \begin{theorem}[Restatement of Theorem \ref{thm:main}]\label{appthm:main}
% Consider the gradient flow of optimizing $\loss(\vecsink, \vecvalue)$. We have that 
% \begin{enumerate}
%     \item (identical attention logits) The gradient flow has equilibria 
%     \[\vecsink = \sink \bm{1}, \quad \vecvalue = c \cdot \bm{1} - e^{-\sink} \cdot \bm{W}\circ \bm{\xi}.\]
%     \item (\textit{attention sink}) Fixing $\vecvalue= c \cdot \bm{1}$, with any initial value $\vecsink(0)$, there exists $\bm{r}(t)$ with bounded norm such that
%     \[\vecsink(t) = \frac{1}{2} \log t \cdot \bm{1} + \bm{r}(t).\]
%     \item (\textit{small value states}) Fixing $\vecsink = \sink \cdot \bm{1}$, with any initial value $\vecvalue(0)$, we have for any $\toki$,
%     \[\abs{\ivalue_\toki(t) - \bar\ivalue(0) - e^{-\sink} W_\toki \xi_\toki} \leq \delta e^{-\mu t},\]
%     where $\bar{\ivalue}(0) = V^\inv[\sum_{\tok} \ivalue_\tok(0)]$, $\delta>0$, and $\mu>0$.
% \end{enumerate}
% \end{theorem}
\begin{theorem}[Restatement the stable phase part in Theorem \ref{thm:main}]\label{appthm:main-1}
Consider the gradient flow of optimizing $\loss(\vecsink, \vecvalue)$. The gradient flow has sink stationary points 
\[\vecsink^\star = \sink \bm{1}, \quad \vecvalue^\star = c \cdot \bm{1} - e^{-\sink} \cdot \bm{W}\circ \bm{\xi}.\]
\end{theorem}
\begin{proof}
When $\vecsink=\vecsink^\star$ and $\vecvalue=\vecvalue^\star$, 
\begin{align*}
\ppred_{\tok\toki} = &~ \frac{\transition_{\tok\toki} \exp\Big[\frac{W_\toki\xi_\toki+e^{\sink}\ivalue_\toki}{e^{\sink}+W}\Big]}{\sum_{\tokk=1}^\vocabsize \transition_{\tok\tokk}\exp\Big[\frac{W_\tokk\xi_\tokk+e^{\sink}\ivalue_\tokk}{e^{\sink}+W}\Big]} \\
 = &~ \frac{\transition_{\tok\toki} \exp\Big[\frac{c}{e^{\sink}+W}\Big]}{\sum_{\tokk=1}^\vocabsize \transition_{\tok\tokk}\exp\Big[\frac{c}{e^{\sink}+W}\Big]} \\
 = &~ \transition_{\tok\toki}.
\end{align*}
Take $\ppred_{\tok\toki}$'s into $\partial \loss(\vecsink,\vecvalue)/\partial \vecsink$ and $\partial \loss(\vecsink,\vecvalue)/\partial \vecvalue$.
\begin{align*}
\frac{\partial \loss(\vecsink,\vecvalue)}{\partial \sink_\tok}\Big |_{\vecsink^\star,\vecvalue^\star} & = \frac{\stable_\tok e^{\sink_\tok}}{(e^{\sink_\tok}+W)^2} 
\sum_{\tokk=1}^\vocabsize \Big\{(\ppred_{\tok\tokk}-\transition_{\tok\tokk}) [W \ivalue_\tokk - W_\tokk \xi_\tokk]
\Big\} = 0,\\
\frac{\partial \loss(\vecsink,\vecvalue)}{\partial \ivalue_\tok}\Big |_{\vecsink^\star,\vecvalue^\star} & = \sum_{\tokk=1}^\vocabsize \Big\{\frac{\stable_\tokk e^{\sink_\tokk} [\ppred_{\tokk\tok}-\transition_{\tokk\tok} ]}{e^{\sink_\tokk}+W}\Big\} = 0.
\end{align*}
This shows that the given points are stationary points. We further compute the second-order derivative using Lemma \ref{appthm:g-ppred}. Define $\bz=[z_1;\ldots;z_\vocabsize]$ so that $z_\tokk = W \ivalue_\tokk - W_\tokk \xi_\tokk$.
\begin{align*}
\frac{\partial^2 \loss(\vecsink, \vecvalue)}{\partial \sink_\toki \partial \sink_\tok} \Big |_{\vecsink^\star,\vecvalue^\star} =  ~& \bm{1}\{\tok=\toki\}\cdot \frac{\stable_\tok e^{\sink}}{(e^{\sink}+W)^2} 
\sum_{\tokk=1}^\vocabsize \Big\{\frac{\partial \ppred_{\toki\tokk}}{\partial \sink_\tok} z_\tokk
\Big\}\\
=  ~& \bm{1}\{\tok=\toki\}\cdot \frac{\stable_\tok e^{2\sink}}{(e^{\sink}+W)^4} 
\Big\{ \sum_{\tokk=1}^\vocabsize \ppred_{\toki\tokk} z_\tokk^2 - \Big[\sum_{\tokk=1}^\vocabsize \ppred_{\toki\tokk}z_\tokk \Big]^2
\Big\},\\
=  ~& \bm{1}\{\tok=\toki\}\cdot \frac{\stable_\tok e^{2\sink}}{(e^{\sink}+W)^4} 
\Big\{ \sum_{\tokk=1}^\vocabsize \transition_{\toki\tokk} z_\tokk^2 - \Big[\sum_{\tokk=1}^\vocabsize \transition_{\toki\tokk}z_\tokk \Big]^2
\Big\}.
\end{align*}
where in the last line, we take $\Ppred=\Transition$. Similarly, we compute the gradients with respect to $\sink_\toki$ and $\ivalue_\tok$.
\begin{align*}
\frac{\partial^2 \loss(\vecsink, \vecvalue)}{\partial \sink_\toki \partial \ivalue_\tok} \Big |_{\vecsink^\star,\vecvalue^\star} =  ~& \frac{\stable_\toki e^{\sink}}{(e^{\sink}+W)^2} 
\sum_{\tokk=1}^\vocabsize \Big\{\frac{\partial \ppred_{\toki\tokk}}{\partial \ivalue_\tok} z_\tokk
\Big\}\\
=  ~& \frac{\stable_\toki e^{2\sink}}{(e^{\sink}+W)^3} 
\Big\{ \transition_{\toki\tok} z_\tokk - \transition_{\toki\tok} \sum_{\tokk=1}^\vocabsize  \transition_{\toki\tokk}z_\tokk
\Big\}.
\end{align*}
With the same manner, we compute the gradients with respect to $\ivalue_\toki$ and $\ivalue_\tok$.
\begin{align*}
\frac{\partial^2 \loss(\vecsink, \vecvalue)}{\partial \ivalue_\toki \partial \ivalue_\tok} \Big |_{\vecsink^\star,\vecvalue^\star} =  ~& \sum_{\tokk=1}^\vocabsize \Big\{\frac{\partial \ppred_{\tokk\toki}}{\partial \ivalue_\tok}\frac{\stable_\tokk e^{\sink}}{e^{\sink}+W}\Big\}\\
= ~& \frac{e^{2\sink}}{(e^\sink+W)^2}\sum_{\tokk=1}^\vocabsize \{ \stable_\tokk [\bm{1}\{\tok=\toki\} \transition_{\tokk\tok} - \transition_{\tokk\toki}\transition_{\tokk\tok}] \}.
\end{align*}
Combining the above computations gives that
\begin{align*}
\text{Hessian}(\loss(\vecsink^\star, \vecvalue^\star)) = \left(\begin{matrix}
\nabla^2_{\vecsink} \loss(\vecsink,\vecvalue) & \nabla_{\vecsink} \nabla_{\vecvalue}  \loss(\vecsink,\vecvalue)\\
\nabla_{\vecvalue} \nabla_{\vecsink} \loss(\vecsink,\vecvalue) & \nabla^2_{\vecsink} \loss(\vecsink,\vecvalue)\\
\end{matrix}\right),
\end{align*}
with
\begin{align*}
\nabla^2_{\vecsink} \loss(\vecsink,\vecvalue) = &~ \frac{e^{2\sink}}{(e^\sink+W)^4}\diag\Big\{ \stable \circ [\bz^\top \gppred^\Transition_1\bz;\ldots;\gppred^\Transition_\vocabsize \bz] \Big\},\\
\nabla_{\vecsink} \nabla_{\vecvalue} \loss(\vecsink,\vecvalue) = &~ \frac{e^{2\sink}}{(e^\sink+W)^3}\diag\Big\{ \stable \Big\} [ \bz^\top\gppred^\Transition_1;\ldots; \bz^\top\gppred^\Transition_\vocabsize] ,\\
\nabla^2_{\vecvalue} \loss(\vecsink,\vecvalue) = &~ \frac{ e^{2\sink}}{(e^{\sink}+W)^2} \sum_{\tokk=1}^\vocabsize  \stable_\tokk \gppred^\Transition_\tokk.\\
\end{align*}
At last, we diagonalize the Hessian matrix and get that
\[
\text{Diag-Hessian}(\loss(\vecsink^\star, \vecvalue^\star)) = \left(\begin{matrix}
\nabla^2_{\vecsink} \loss(\vecsink,\vecvalue) & 0\\
0 & \frac{ e^{2\sink}}{(e^{\sink}+W)^2} \bH\\
\end{matrix}\right),
\]
where the $\bH$ is given by
\begin{align*}
\bH = \sum_{\tokk=1}^\vocabsize  \stable_\tokk \Big(\gppred^\Transition_\tokk - (\bm{z}^\top \gppred_\tokk^\Transition \bm{z})^{-1}\gppred^\Transition_\tokk\bm{z}\bm{z}^\top\gppred^\Transition_\tokk\Big).
\end{align*}
To prove that $\bH$ is positive semi-definite, consider any vector $\bm{\eta}$ with $\|\bm{\eta}\|_2=1$.
\begin{align*}
\bm{\eta}^\top \bH \bm{\eta} = &~ \sum_{\tokk=1}^\vocabsize  \stable_\tokk \Big(\bm{\eta}^\top\gppred^\Transition_\tokk\bm{\eta} - \frac{\bm{\eta}^\top\gppred^\Transition_\tokk\bm{z}\bm{z}^\top\gppred^\Transition_\tokk\bm{\eta}}{\bm{z}^\top \gppred_\tokk^\Transition \bm{z}}\Big).
\end{align*}
Since $\gppred^\Transition_\tokk$'s are positive semi-definite, the Cauchy inequality gives that
\[
\bm{z}^\top\gppred^\Transition_\tokk\bm{\eta} \leq \sqrt{\bm{z}^\top \gppred_\tokk^\Transition \bm{z} \bm{\eta}^\top \gppred_\tokk^\Transition \bm{\eta}}.
\]
As a result, we have that
\begin{align*}
\bm{\eta}^\top \bH \bm{\eta} \geq &~ \sum_{\tokk=1}^\vocabsize  \stable_\tokk \Big(\bm{\eta}^\top\gppred^\Transition_\tokk\bm{\eta} - \frac{\bm{z}^\top \gppred_\tokk^\Transition \bm{z} \bm{\eta}^\top \gppred_\tokk^\Transition \bm{\eta}}{\bm{z}^\top \gppred_\tokk^\Transition \bm{z}}\Big) = 0.
\end{align*}
This shows that $\bH$ is positive semi-definte. Therefore, $\text{Hessian}(\loss(\vecsink^\star, \vecvalue^\star))$ is positive semi-definte. This proves Theorem \ref{appthm:main-1}.
\end{proof}
We prove Theorem \ref{appthm:main-1} through direct computation. Due to the non-linearity, it's unclear whether other stationary points exist. However, we observe that all of our simulations converge to the given stationary points. 
\subsection{Attention sinks in Theorem \ref{thm:main}}
\begin{theorem}[Restatement of the attention sink part in Theorem \ref{thm:main}]\label{appthm:main-2}
Fixing $\vecvalue= c \cdot \bm{1}$, with any initial value, there exists $\bm{r}(t)$ with bounded norm such that
\[\vecsink(t) = \frac{1}{2} \log t \cdot \bm{1} + \bm{r}(t).\]
\end{theorem}
\begin{proof}
We separately analyze each entry of $\vecsink$. Focusing on $\sink_\tok$, to simplify the notation, we introduce a random variable $\varphi$ such that $\P(\varphi=W_\tokk\xi_\tokk)=\transition_{\tok\tokk}$.
Define 
\[
u = e^{\sink_\tok}.
\]
Therefore, using Lemma \ref{appthm:gradients}, we get that
\begin{align*}
\frac{\mathrm{d} u}{\mathrm{d} t} = \frac{\stable_\tok e^{2\sink_\tok}}{(e^{\sink_\tok}+W)^2} 
\sum_{\toki=1}^\vocabsize({\ppred}_{\tok\toki}-{\transition}_{\tok\toki})(W\ivalue_\toki-W_\toki\xi_\toki).
\end{align*}
We take in $\ivalue = c$ and expand the expression of $\mathrm{d}u/\mathrm{d}t$. This gives us
\begin{align*}
\frac{\mathrm{d} u}{\mathrm{d} t} = &~ \frac{\stable_\tok u^2}{(u+W)^2} \frac{\sum_{\tokk=1}^\vocabsize \transition_{\tok\tokk} e^{W_\tokk\xi_\tokk/(u+W)}W_\tokk\xi_\tokk - \sum_{\tokk=1}^\vocabsize \transition_{\tok\tokk} e^{W_\tokk\xi_\tokk/(u+W)}\sum_{\tokk=1}^\vocabsize W_\tokk\xi_\tokk}{\sum_{\tokk=1}^\vocabsize \transition_{\tok\tokk} e^{W_\tokk\xi_\tokk/(u+W)}}\\
= &~ \frac{\stable_\tok u^2}{(u+W)^2} \frac{\Cov(e^{\frac{\varphi}{u+W}},\varphi)}{\E e^{\frac{\varphi}{u+W}}}.
\end{align*}
Since both $e^{x/(u+W)}$ and $x$ are monotonically increasing with respect to $x$, $u$ is monotonically increasing. This means that
\[
\frac{u(t)^2}{[u(t)+W]^2} \geq \frac{u(0)^2}{[u(0)+W]^2},\quad \E e^{\frac{\varphi}{u(t)+W}} \leq \E e^{\frac{\varphi}{u(0)+W}}.
\]
Meanwhile, if we consider the first and second order approximation of $e^{\varphi/(u+W)}$, 
\[
e^{\frac{\varphi}{u+W}} = 1 + \frac{\theta_1(\varphi) \varphi}{u+W},\quad e^{\frac{\varphi}{u+W}} = 1 + \frac{\varphi}{u+W} + \theta_2(\varphi) \Big[\frac{\varphi}{u+W}\Big]^2.
\]
Both $\theta_1(\varphi)$ and $\theta_2(\varphi)\varphi^2$ are  monotonically increasing functions of $\varphi$. We also have the bound
\[
\theta(\varphi) \leq \frac{e^{\frac{\max \varphi}{u(0)+W}}-1}{\frac{\max \varphi}{u(0)+W}-1} = C_\theta.
\]
Therefore, we get two more inequalities
\[
\Cov(\theta_1(\varphi)\varphi,\varphi)\leq C_\theta \Var(\varphi),\quad \Cov(\theta_2(\varphi)\varphi^2,\varphi)\geq 0.
\]
With all the preparatory works down, we give upper and lower bounds for $\mathrm{d}u/\mathrm{d}t$.
We first upper-bound $\mathrm{d}u/\mathrm{d}t$. 
\begin{align*}
\frac{\mathrm{d}u}{\mathrm{d}t} \leq &~ \stable_\tok \Cov(e^{\frac{\varphi}{u+W}}, \varphi)\\
= &~ \stable_\tok\Cov(1 + \frac{\theta_1(\varphi)\varphi}{u+W}, \varphi)\\
\leq &~ \frac{\stable_\tok C_\theta \Var(\varphi)}{u}.
\end{align*}
By solving the corresponding ODE, we get that
\begin{align*}
\frac{1}{2} u^2 \leq \sqrt{C_\theta \Var(\varphi) t} + C.
\end{align*}
To give a lower bound, we have that
\begin{align*}
\frac{\mathrm{d}u}{\mathrm{d}t} \geq &~ \frac{u(0)^2}{[u(0)+W]^2}\frac{\stable_\tok \Cov(e^{\frac{\varphi}{u+W}},\varphi)}{\E e^{\frac{\varphi}{u(0)+W}}} \\
\geq &~ \frac{u(0)^2}{[u(0)+W]^2}\frac{\stable_\tok}{\E e^{\frac{\varphi}{u(0)+W}}} \Cov(1+\frac{\varphi}{u+W}+\theta_2(\varphi) \Big[\frac{\varphi}{u+W}\Big]^2,\varphi)\\
\geq &~ \frac{u(0)^2}{[u(0)+W]^2}\frac{\stable_\tok}{\E e^{\frac{\varphi}{u(0)+W}}} \frac{\Var(\varphi)}{u+W}\\
\geq &~ \frac{u(0)^2}{[u(0)+W]^2}\frac{\stable_\tok}{\E e^{\frac{\varphi}{u(0)+W}}} \cdot \frac{u(0)}{u(0)+W} \cdot \frac{\Var(\varphi)}{u}\\
= &~ \Tilde{C}_\theta \frac{1}{u}.
\end{align*}
Therefore, $u \geq \sqrt{\Tilde{C}_\theta t + \Tilde{C}}$. In conclusion, 
\[
y_{\tok} = \log u = \frac{1}{2}\log t + r_{\tok},
\]
with $r_{\tok}$ bounded.
\end{proof}
\subsection{Value state drains in Theorem \ref{thm:main}}
\begin{theorem}[Restatement of Theorem \ref{thm:main}]\label{appthm:main-3}
Fixing $\vecsink=y\bm{1}$, $\vecvalue=c\bm{1}-e^{-\sink} \bm{W}\circ \bm{\xi}$ with $c\in\R$. Define $\bar{\ivalue}(t)=\vocabsize^{-1}\sum_{\toki=1}^\vocabsize \ivalue_\toki(t)$. Then the gradient flow of $\vecvalue(t)$ converges:
\[
\vecvalue(t) \to \vecvalue^\star=\bar{\ivalue}(0)\bm{1}-e^{-\sink} \bm{W}\circ \bm{\xi}.
\]
\end{theorem}
\begin{proof}
Theorem \ref{appthm:main-1} has already verified that $\vecvalue=c\bm{1}-e^{-\sink} \bm{W}\circ \bm{\xi}$ are stationary points of $\loss$.
In the proof of Theorem \ref{appthm:main-1}, we have derived $\nabla^2_{\vecvalue} \loss(\vecsink,\vecvalue)$.
\begin{align*}
\nabla^2_{\vecvalue} \loss(\vecsink,\vecvalue) = \sum_{\tokk=1}^\vocabsize \stable_\tokk \gppred^\Ppred_\tokk.
\end{align*}
Lemma \ref{appthm:positive-definite} indicates that it is positive semi-definite. Therefore, all stationary points attain the minimum of $\loss(\vecsink,\vecvalue)$. Suppose $\vecvalue^\star$ is a stationary point, we therefore get that $\ppred_{\tok\tokk}=\transition_{\tok\tokk}$ for any $\tok,$ $\tokk$. This implies that $e^y \ivalue^\star_\tokk + W_\tokk \xi_\tokk$ are constants across $\tokk$. We can solve $\ivalue^\star$ and get that
$\vecvalue^\star=c\bm{1}-e^{-\sink} \bm{W}\circ \bm{\xi}$. The convexity of the $\loss(\vecsink,\vecvalue)$ guarantees that $\vecvalue$ always converges to a stationary point $\vecvalue^\star$.

To find the value of $c$ in $\vecvalue^\star$, note that  $\sum_{\tok=1}^\vocabsize \dot{\ivalue}_\tok(t)=0$. We get that $\bar{\ivalue}^\star=\bar{\ivalue}(0)$. Therefore, $\vecvalue^\star=\vecvalue^\star=\bar{\ivalue}(0)\bm{1}-e^{-\sink} \bm{W}\circ \bm{\xi}$.
\end{proof}
\begin{remark}
If we assume that $\transition_{\tok\tokk}>0$ for any $\tok$, $\tokk$ and suppose that the initial value $\vecvalue(0)$ is close enough to $\vecvalue^\star$, it is possible to prove the fast convergence of $\vecvalue(t)$ to $\vecvalue^\star$.
\begin{equation*}
\|\vecvalue(t) - \vecvalue^\star\|^2_2 \leq \delta e^{-\mu t}.
\end{equation*}
\end{remark}




==> Sections_arxiv/appendices/related.tex <==
\section{Related works}
Several studies independently identified the ``attention sink'' phenomenon in language models and vision transformers,  where attention weights were found to be concentrated on a few tokens \citep{xiao2023efficient, darcet2023vision, han2023lm, zhai2023stabilizing, elhage2023privileged, dettmers2022gpt3}. Recent research has provided more detailed characterizations of this attention pattern and the attention sink phenomenon \citep{fu2024attentionpattern, sun2024massive}. \citet{sun2024massive} attributed the attention sink to the massive activation of the hidden representations of the corresponding tokens. Both \citet{sun2024massive} and \citet{zhai2023stabilizing} discussed methods for mitigating the attention sink by modifying the model and training recipes. Additionally, recent studies have leveraged the attention sink phenomenon to develop improved quantization and more efficient inference algorithms \citep{liu2024intactkv, chen2024image, yu2024unveiling, son2024prefixing}.

The dynamics of transformers are studied under various simplifications, including linear attention structures \citep{zhang2023trained,ahn2024transformers}, reparametrizations \citep{tian2023joma}, NTK \citep{deora2023optimization}, often in the setting of in-context linear regressions \citep{ahn2023linear,wu2023many,zhang2024context} and structured sequence  \citep{bietti2024birth,nichani2024transformers,tian2023scan}. Notably, \citet{zhang2023trained} proves that a one-layer linear attention head trained with gradient descent converges to a model that implements the in-context linear regression algorithm.
\cite{huang2023context,kim2024transformers} extend this to non-linear settings. \cite{bietti2024birth} shows the fast learning of bigram memorization and the slow development of in-context abilities. \cite{tian2023scan} shows the scan and snap dynamics in reparametrized one-layer transformers. \cite{reddy2023mechanistic} simplifies the structure of the induction head, showing the connection between the sharp transitions of in-context learning dynamics and the nested nonlinearities of multi-layer operations.

Mechanistic interpretability is a growing field focused on understanding the internal mechanisms of language models in solving specific tasks \citep{elhage2021mathematical, geva2023dissecting, meng2022locating, nanda2023progress, olsson2022context, bietti2024birth, wang2022interpretability, feng2023language, todd2023function}. This includes mechanisms like the induction head and function vector for in-context learning \citep{elhage2021mathematical, olsson2022context, todd2023function, bietti2024birth}, the binding ID mechanism for binding tasks \citep{feng2023language}, association-storage mechanisms for factual identification tasks \citep{meng2022locating}, and a complete circuit for indirect object identification tasks \citep{wang2022interpretability}. The task addressed in this paper is closely related to \cite{bietti2024birth}, which explored synthetic tasks where tokens are generated from either global or context-specific bigram distributions. Several other studies have also used synthetic tasks to investigate neural network mechanisms \citep{charton2022my, liu2022towards, nanda2023progress, allen2023physics, zhu2023physics, guo2023transformers, zhang2022unveiling}. 




We note that \citet{gurnee2024universal} proposed Attention Deactivation Neurons, a concept similar to Dormant Attention Heads. \citet{gurnee2024universal} hypothesized that when such a head attends to the first token, it indicates that the head is deactivated and has minimal effect. 







% For a positive integer \(n\) let \([n]\) be the set \(\{0, 1, \dots, n - 1\}\).\footnote{Throughout this paper, we will use zero-indexing, in order to keep consistency between code and math.} For a matrix \(\bX\), we denote its \(i^{\mathrm{th}}\) column by \(\bx_{i}\), its \((i, j)^{\mathrm{th}}\) entry by \(X_{ij}\), and its transpose by \(\bX^{\top}\).

% \begin{itemize}
% \item Methods: \cite{ramachandran2017searching}
% \end{itemize}




==> Sections_arxiv/appendices/supporting_results.tex <==
\section{Supporting Results}

% In this appendix, we provide more supporting evidence for our conjecture in \Cref{sec:dormant_heads}.


% \subsection{Supporting Results for \Cref{sub:circuit_evidence}} \label{sub:app_supporting_circuit}


\begin{figure}[t]
  \centering
  \begin{minipage}{0.24\textwidth}
      \centering
      \subcaption{\small lower layers on \bos}
      \label{fig:appendix-ablation-bos-lower}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/bos_lower.pdf}
  \end{minipage}~
  % \hspace{-1em}
  \begin{minipage}{0.24\textwidth}
      \centering
      \subcaption{\small upper layers on \bos}
      \label{fig:appendix-ablation-bos-upper}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/bos_upper.pdf}
  \end{minipage}~
  % \hspace{-1em}
  \begin{minipage}{0.24\textwidth}
      \centering
      \subcaption{\small lower layers on \delim}
      \label{fig:appendix-ablation-delim-lower}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/delim_lower.pdf}
  \end{minipage}~
  % \vspace{-1em}
    \begin{minipage}{0.24\textwidth}
      \centering
      \subcaption{\small upper layers on \delim}
      \label{fig:appendix-ablation-delim-lower}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/delim_upper.pdf}
  \end{minipage}~
  
  \caption{\small The effect of $\MLP$ and $\Attn$ of lower and upper two layers on the norm of \bos and \delim.}
  \label{figure:appendix-ablation-massive-sup-control}
  % \vspace{-1em}
\end{figure}


\begin{figure}[t]
  \centering
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Ablations on layer $0$}
      \label{fig:appendix-ablation-massive-sup-control-0}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/bos_control/bos_massive_sup_L0.pdf}
  \end{minipage}~
  % \hspace{-1em}
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Ablations on layer $1$}
      \label{fig:appendix-ablation-massive-sup-control-1}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/bos_control/bos_massive_sup_L1.pdf}
  \end{minipage}~
  % \hspace{-1em}
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Ablations on entire layer $0$}
      \label{fig:appendix-ablation-massive-sup-control-attn}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/bos_control/L0_intervention_attn_weights.pdf}
  \end{minipage}~
  % \vspace{-1em}
  
  \caption{\small Ablations using control sample
  }
  \label{figure:appendix-ablation-massive-sup-control}
  % \vspace{-1em}
\end{figure}

\begin{figure}[t]
  \centering
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Ablations on layer $0$}
      \label{fig:appendix-ablation-massive-sup-zero-0}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/bos_zero_out/bos_massive_L0.pdf}
  \end{minipage}~
  % \hspace{-1em}
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Ablations on layer $1$}
      \label{fig:appendix-ablation-massive-sup-zero-1}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/bos_zero_out/bos_massive_L1.pdf}
  \end{minipage}~
  % \hspace{-1em}
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Ablations on entire layer $0$}
      \label{fig:appendix-ablation-massive-sup-zero-attn}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/bos_zero_out/L0_zero_attn_weights.pdf}
  \end{minipage}~
  % \vspace{-1em}
  
  \caption{\small Ablations using zeroing-out
  }
  \label{figure:appendix-ablation-massive-zero}
  % \vspace{-1em}
\end{figure}

\begin{figure}[t]
  \centering
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Ablations on layer $0$}
      \label{fig:appendix-ablation-delim-0}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/delim_no_rope/delim_massive_suppression_L0.pdf}
  \end{minipage}~
  % \hspace{-1em}
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Ablations on layer $1$}
      \label{fig:appendix-ablation-delim-1}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/delim_no_rope/delim_massive_suppression_L1.pdf}
  \end{minipage}~
  % \hspace{-1em}
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Ablations on entire layer $0$}
      \label{fig:appendix-ablation-delim-attn}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/interventions/delim_no_rope/L0_no_rope_attn_weights.pdf}
  \end{minipage}~
  % \vspace{-1em}
  
  \caption{\small Ablations using no \rope
  }
  \label{figure:appendix-ablation-delim}
  % \vspace{-1em}
\end{figure}


\subsection{Supporting Results for \Cref{sub:lots_of_dormant_heads}} \label{sub:app_supporting_lots_of_heads}


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Figures/L16_H25/attn_maps_l16h25_wiki.pdf}
    \includegraphics[width=\textwidth]{Figures/L16_H25/attn_maps_l16h25_github.pdf}
    \caption{\small\textbf{Visualizations of attention weights for Llama 2 7B Layer 16 Head 25 on both Wikipedia and GitHub data.} A continuation of \Cref{fig:attn_l16_h25_small}.}
    \label{fig:attn_l16_h25_improved}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Figures/L16_H25/attn_logits_l16h25_wiki.pdf}
    \includegraphics[width=\textwidth]{Figures/L16_H25/attn_logits_l16h25_github.pdf}
    \caption{\small\textbf{Visualizations of pre-softmax attention logits for Llama 2 7B Layer 16 Head 25 on both Wikipedia and GitHub data.} A continuation of \Cref{fig:attn_logits_l16_h25_small}.}
    \label{fig:attn_logits_l16_h25_improved}
\end{figure}

\subsection{Supporting Results for \Cref{sub:controlled_experiments}} \label{sub:app_supporting_controlled}

\subsection{Task in \citet{bietti2024birth}}
\begin{figure}[t]
  \centering
  \begin{minipage}{0.4\textwidth}
      \centering
      \subcaption{\small Data generating procedure}
      \label{fig:appendix-pretraining-dgp}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/Biette.pdf}
  \end{minipage}
  \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Layer 0 on dormant sequence}
      \label{fig:appendix-biette-attn-weights-dormant-l0}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/Biette_attn_weights_seq0_layer0.pdf}
  \end{minipage}
  \hspace{-1em}
    \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Layer 1 on dormant sequence}
      \label{fig:appendix-biette-attn-weights-dormant-l1}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/Biette_attn_weights_seq0_layer1.pdf}
  \end{minipage}
  \vspace{-1em}
  \caption{\small Using the task in \citet{bietti2024birth}}
  \label{figure:appendix-pretraining-biette-findings}
  \vspace{-1em}
\end{figure}

\begin{figure}
\centering
  \begin{minipage}{0.45\textwidth}
      \centering
      \subcaption{\small Layer 0 on active sequence}
      \label{fig:appendix-biette-attn-weights-active-l0}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/Biette_attn_weights_seq1_layer0.pdf}
  \end{minipage}
  \hspace{-1em}
    \begin{minipage}{0.45\textwidth}
      \centering
      \subcaption{\small Layer 1 on active sequence}
      \label{fig:appendix-biette-attn-weights-active-l1}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/Biette_attn_weights_seq1_layer1.pdf}
  \end{minipage}
  \vspace{-1em}
  \caption{\small Using the task in \citet{bietti2024birth}}
  \label{figure:appendix-pretraining-biette-findings-1}
  \vspace{-1em}
\end{figure}

\begin{figure}
      \centering
  \begin{minipage}{0.45\textwidth}
      \centering
      \subcaption{\small Output norm on layer 1}
      \label{fig:appendix-biette-massive}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/Biette/Biette_L3_massive.pdf}
  \end{minipage}
  \hspace{-1em}
    \begin{minipage}{0.45\textwidth}
      \centering
      \subcaption{\small Value state norm on layer 2}
      \label{fig:appendix-biette-minor}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/Biette/Biette_L3_minor.pdf}
  \end{minipage}
  \vspace{-1em}
  \caption{\small Using the task in \citet{bietti2024birth}}
  \label{figure:appendix-pretraining-biette-findings-3}
  \vspace{-1em}
\end{figure}

\subsection{The ``dormant Markov task''}
\begin{figure}[t]
  \centering
  \begin{minipage}{0.4\textwidth}
      \centering
      \subcaption{\small Data generating procedure}
      \label{fig:appendix-pretraining-dgp-dormant-markov}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_markov.pdf}
  \end{minipage}
  \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Layer 0 on dormant sequence}
      \label{fig:appendix-dormant-markov-attn-weights-dormant}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_markov/dormant_markov_attn_weights_seq0.pdf}
  \end{minipage}
  \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Layer 0 on active sequence}
      \label{fig:appendix-dormant-markov-attn-weights-active}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_markov/dormant_markov_attn_weights_seq1.pdf}
  \end{minipage}
  \vspace{-1em}
  \caption{\small Dormant markov task}
  \label{figure:appendix-pretraining-dormant-markov-1}
  \vspace{-1em}
\end{figure}

\begin{figure}
      \centering
  \begin{minipage}{0.45\textwidth}
      \centering
      \subcaption{\small Output norm on layer 1}
      \label{fig:appendix-dormant-markov-massive}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_markov/dormant_markov_L3_massive.pdf}
  \end{minipage}
  \hspace{-1em}
    \begin{minipage}{0.45\textwidth}
      \centering
      \subcaption{\small Value state norm on layer 2}
      \label{fig:appendix-dormant-markov-minor}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_markov/dormant_markov_L3_minor.pdf}
  \end{minipage}
  \vspace{-1em}
  \caption{\small Dormant markov task}
  \label{figure:appendix-pretraining-dormant-markov-findings-2}
  \vspace{-1em}
\end{figure}

==> Sections_arxiv/appendices/tmp.tex <==
\frac{\partial \log\Big[\sum_{\toki=1}^\vocabsize \transition^\tokksup_\toki\exp\Big[\frac{W^\tokisup\beta^\tokisup+e^{\sink_j}\ivalue_\toki}{e^{\sink_j}+W}\Big]\Big]}{\partial \ivalue_\tok} = &~ \frac{e^{\sink_j}}{e^{\sink_j}+W} \cdot \frac{  \transition^\tokksup_\tok \exp\Big[\frac{W^\tokksup\beta^\tokksup+e^{\sink_j}\ivalue_\tok}{e^{\sink_j}+W}\Big]}{\sum_{\toki=1}^\vocabsize \transition^\toksup_\toki\exp\Big[\frac{W^\tokisup\beta^\tokisup+e^{\sink_j}\ivalue_\toki}{e^{\sink_j}+W}\Big]}\label{eqn:ds-part1} \\
\frac{\partial 

==> Sections_arxiv/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}

In this work, we investigated the \textit{extreme-token phenomena}, namely \textit{attention sinks}, \textit{value state drains}, and \textit{residual state peaks}. We analyzed a simple evocative model called the Bigram-Backcopy task, and theoretically and empirically showed that it exhibited the same extreme-token phenomena as in LLMs. Based on the Bigram-Backcopy task, we made several detailed predictions about the behavior of extreme-token phenomena in LLMs. In particular, we identified the \textit{active-dormant mechanism} for attention heads in both the BB model and LLMs, of which attention sinks and value state drains are indicators, and a \textit{mutual reinforcement mechanism} by which these phenomena are induced during pretraining. Using intuition about these mechanisms, we applied minor interventions to the model architecture and optimization procedure which disabled extreme-token phenomena within the BB model. Overall, our work uncovers the causes of extreme-token phenomena and points to possible pathways to eliminate them during LLM training.

We believe the most compelling direction for future work in this area is as follows. Specifically, one could build more performant and scalable interventions which would eliminate extreme-token phenomena and observe the effect on training dynamics and the finished model. This would make it easier to understand whether extreme token phenomena are necessary to build a powerful transformer-based LLM, whether they are merely helpful, or whether they are completely incidental to the particular architecture and optimization algorithms used by the community.

==> Sections_arxiv/deprecated_sections/applications.tex <==
\section{Applications}

% \begin{itemize}
%     % \item Speed up attention computation by by-passing softmax partition function?~\yub{first step: check whether decoding is still exactly correct on large corpus.}
% \end{itemize}

==> Sections_arxiv/deprecated_sections/case_study.tex <==
\section{Case Study and Motivation}\label{sec:case_study}

In this section, we will study a particular attention head in Llama 2, and use its behavior as a motivation for the more general analysis that follows.

\subsection{Preliminaries}\label{sub:prelim}

\DP{TODO @TG: Fill out a simplified notation block. Please ensure that the simplified notation is consistent with the notation in the appendix.}

\DP{TODO: mention that we pre-pend all inputs with \bos.}

A significantly more precise setup and notation is detailed in \Cref{sub:app_notation}.

\subsection{Understanding Layer 16 Attention Head 25 of Llama 2}\label{sub:case_study_l25_h16}

As motivation for our later reasoning, we will now examine the behavior of Layer 16 Attention Head 25 (abbreviated as L16H25) in Llama 2 7B, on both prose from the Wikipedia dataset \citep{wikidump} and code from the RedPajama Github dataset \citep{together2023redpajama}. This is the first attention head which we identify as a dormant head, and we want to understand its properties at a more fine-grained level. First, let us examine the difference in perplexity on samples of these two datasets obtained from the full forward pass versus a modified forward pass where the output of the attention head L16H25 is zeroed out. Specifically, we evaluate each forward pass on 32 samples of their respective datasets, where each sample is truncated to 64 tokens. We observe the results in \Cref{tab:ppl_wiki_github_l16h25}. Overall, the performance change is greater on the GitHub data than on the Wikipedia data, which signals that it may be the case that L16H25 is function-less on the Wikipedia data yet has a function on the GitHub data. To confirm our hypothesis, we plot the (post-softmax) attention weights on a few representative samples of GitHub and Wikipedia data in \Cref{fig:attn_l16_h25_small} (and \Cref{fig:attn_l16_h25_improved} in \Cref{sub:app_supporting_lots_of_heads}). We observe that L16H25 is an attention sink \citep{xiao2023efficient} on Wikipedia data. This means that for each sample, the attention head outputs roughly the same vector (or one of a few possible vectors) for each token position, acting like a bias which does not use correlations between tokens. On the other hand, on GitHub data L16H25 is not an attention sink. This discrepancy motivates the definition of a dormant head, expanded on in \Cref{sec:dormant_heads}, that a dormant head is one which does not use correlations between tokens to obtain an output (and thus is not impacted by the semantics of the input). To confirm this, we also plot the pre-softmax logits in \Cref{fig:attn_logits_l16_h25_small} (and \Cref{fig:attn_logits_l16_h25_improved} in \Cref{sub:app_supporting_lots_of_heads}). \DP{TODO: @TG could you give some reasoning here?}

\begin{table}
    \centering
    \caption{\small \textbf{Perplexity of Llama 2 7B when using an unmodified forward pass vs.~a forward pass which is modified to set the output of L16H25 to \(0\).} We observe that while the perplexity does not change substantially on Wikipedia data, it noticeably increases on Github data. This motivates the hypothesis that L16H25 is ``dormant'' for Wikipedia data and ``active'' for Wikipedia data.}
    \begin{tabular}{@{}lll@{}}
    \toprule
    \textbf{Perplexity}    & Wikipedia Dataset & Github Dataset \\ \midrule
    Unmodified forward pass                  &                   &                \\
    Modified forward pass  &                   &                \\ \bottomrule
    \end{tabular} 
    \label{tab:ppl_wiki_github_l16h25}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/L16_H25/attn_maps_l16h25_wiki_small.pdf}
    \hspace{0.075\textwidth}
    \includegraphics[width=0.45\textwidth]{Figures/L16_H25/attn_maps_l16h25_github_small.pdf}
    \caption{\small\textbf{Visualizations of attention weights for Llama 2 7B L16H25 on both Wikipedia and GitHub data.} On four random samples from each domain, we truncate each sample to 64 tokens and visualize the (post-softmax) attention weights from this head. We observe that for Wikipedia the head has one or two attention sinks, while for GitHub the head has no attention sink, corresponding to our hypothesis that the head is ``dormant'' on Wikipedia and ``active'' on GitHub. Further samples are plotted in \Cref{fig:attn_l16_h25_improved}, maintaining this trend.}
    \label{fig:attn_l16_h25_small}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/L16_H25/attn_logits_l16h25_wiki_small.pdf}
    \hspace{0.075\textwidth}
    \includegraphics[width=0.45\textwidth]{Figures/L16_H25/attn_logits_l16h25_github_small.pdf}
    \caption{\small\textbf{Visualizations of pre-softmax attention logits for Llama 2 7B L16H25 on both Wikipedia and GitHub data.} \DP{@TG: please fill in the description here and in main body.} Further samples are plotted in \Cref{fig:attn_logits_l16_h25_improved}, maintaining this trend. \tianyu{how about deleting this figure? It's hard to tell that the logits are around the same. Instead, how about make annotations on previous figure, showing the attention logits on bos?}}
    \label{fig:attn_logits_l16_h25_small}
\end{figure}



==> Sections_arxiv/deprecated_sections/compression_results.tex <==
\DP{write intro for this}

Causal compression algorithm: at sequence index \(t\) with final index \(T\), threshold out all but \(\approx \frac{1}{2}t\) or \(\frac{1}{10}t\) tokens. Non-causal compression algorithm: threshold out all but \(\approx \frac{1}{2}T\) or \(\frac{1}{10}T\) tokens. When \(T \gg t\) (i.e., infinite-streaming contexts), the former is more restrictive than the latter, and also may scale much better.

For all tasks we report the raw zero-shot accuracy as computed by EleutherAI's evaluation harness \citep{eval-harness}, at this \href{https://github.com/EleutherAI/lm-evaluation-harness/tree/cffc1bd3fd69453eaa75da891256682123226f0f}{permalink}.

\begin{table}[H]
    \centering
    \resizebox{0.99\textwidth}{!}{
        \begin{tabular}{@{}llllllllll@{}}
        \toprule
        Model     & Compression Scheme                          & Compression Ratio & ARC-C & ARC-E & HellaSwag & LAMBADA & OpenBookQA & PIQA  & Winogrande \\ \midrule
        Llama2-7B & No Compression                              & N/A               & 0.434 & 0.763 & 0.571     & 0.683   & 0.314      & 0.781 & 0.691      \\
                  & Adaptive Per-Layer Compression              & 50\%              & 0.435 & 0.763 & 0.571     & 0.683   & 0.314      & 0.781 & 0.691      \\
                  &                                             & 90\%              & 0.431 & 0.746 & 0.572     & 0.679   & 0.272      & 0.772 & 0.698      \\
                  & Adaptive Per-Head Compression               & 50\%              & 0.434 & 0.763 & 0.571     & 0.683   & 0.314      & 0.781 & 0.691      \\
                  &                                             & 90\%              & 0.416 & 0.734 & 0.567     & 0.681   & 0.28       & 0.766 & 0.706      \\
                  & Adaptive Per-Query-Token Causal Compression & 50\%              & 0.437 & 0.761 & 0.571     & 0.681   & 0.312      & 0.780 & 0.691      \\
                  &                                             & 90\%              & 0.404 & 0.720 & 0.546     & 0.643   & 0.268      & 0.763 & 0.658      \\ \bottomrule
        \end{tabular}
    }
    \caption{\textbf{Comparison of our attention head compression methods on zero-shot accuracy on standard benchmarks.} We observe that all compression methods preserve the performance of the base Llama2 model. The Per-Query-Token Causal Compression method performs the worst with 90\% of tokens compressed, but still preserves most of the performance and scales the best.}
    \label{tab:comparing_our_different_compression_methods}
\end{table}


\begin{table}[H]
    \centering
    \resizebox{0.99\textwidth}{!}{
        \begin{tabular}{@{}llllllllll@{}}
            \toprule
            Model     & Compression Scheme                          & Compression Ratio & ARC-C & ARC-E & HellaSwag & LAMBADA & OpenBookQA & PIQA  & Winogrande \\ \midrule \midrule
            Llama2-7B & No Compression                              & N/A               & 0.434 & 0.763 & 0.571     & 0.683   & 0.314      & 0.781 & 0.691      \\
                      & StreamingLLM Compression                    & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\
                      & StreamingLLM Causal Compression             & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\
                      & Adaptive Per-Query-Token Causal Compression & 50\%              & 0.437 & 0.761 & 0.571     & 0.681   & 0.312      & 0.780 & 0.691      \\
                      &                                             & 90\%              & 0.404 & 0.720 & 0.546     & 0.643   & 0.268      & 0.763 & 0.658      \\ \midrule
            Mistral-7B& No Compression                              & N/A               &       &       &           &         &            &       &            \\
                      & StreamingLLM Compression                    & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\
                      & StreamingLLM Causal Compression             & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\
                      & Adaptive Per-Query-Token Causal Compression & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\ \midrule
            Gemma-7B  & No Compression                              & N/A               &       &       &           &         &            &       &            \\
                      & StreamingLLM Compression                    & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\
                      & StreamingLLM Causal Compression             & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\
                      & Adaptive Per-Query-Token Causal Compression & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\ \midrule
            Pythia-7B & No Compression                              & N/A               &       &       &           &         &            &       &            \\
                      & StreamingLLM Compression                    & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\
                      & StreamingLLM Causal Compression             & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\
                      & Adaptive Per-Query-Token Causal Compression & 50\%              &       &       &           &         &            &       &            \\
                      &                                             & 90\%              &       &       &           &         &            &       &            \\ \bottomrule
        \end{tabular}
    }
    \caption{\textbf{Comparison of our adaptive causal attention compression algorithm against the previous one posed by StreamingLLM \citep{xiao2023efficient} on zero-shot accuracy on standard benchmarks.} We observe that our method succeeds most of the time in retaining performance, at least on these benchmarks, much better than StreamingLLM. This holds even if we do not force their mechanism to be causal.}
    \label{tab:compare_ours_streamingllm_zeroshot}
\end{table}



We also evaluate their perplexity on LAMBADA and the first row of the PG19 dataset (an extremely long document), chunked into \DP{INSERT HERE} subsets of \DP{INSERT HERE} contiguous tokens over which the perplexity is averaged.

\begin{table}[H]
    \centering
    \resizebox{0.99\textwidth}{!}{
        \begin{tabular}{@{}lllll@{}}
            \toprule
            Model     & Compression Scheme                          & Compression Ratio & LAMBADA Perplexity & PG19 Document 1 Perplexity \\ \midrule
            Llama2-7B & No Compression                              & N/A               & 4.13               &                            \\
                      & StreamingLLM Compression                    & 50\%              &                    &                            \\
                      &                                             & 90\%              &                    &                            \\
                      & StreamingLLM Causal Compression             & 50\%              &                    &                            \\
                      &                                             & 90\%              &                    &                            \\
                      & Adaptive Per-Layer Compression              & 50\%              & 4.12               &                            \\
                      &                                             & 90\%              & 4.16               &                            \\
                      & Adaptive Per-Head Compression               & 50\%              & 4.13               &                            \\
                      &                                             & 90\%              & 4.19               &                            \\
                      & Adaptive Per-Query-Token Causal Compression & 50\%              & 4.14               &                            \\
                      &                                             & 90\%              & 5.06               &                            \\ \bottomrule
        \end{tabular}
    }
    \caption{\textbf{Comparison of our attention-head compression algorithms against the previous one posed by StreamingLLM \citep{xiao2023efficient} on average perplexity on the LAMBADA task and the first document of the PG19 dataset.} We observe that our adaptive methods generally maintain significantly better perplexity than the previous StreamingLLM-derived methods on both short and long contexts.}
    \label{tab:compare_ourrs_streamingllm_ppl}
\end{table}

==> Sections_arxiv/deprecated_sections/dormant_heads.tex <==
\section{Dormant Attention Heads}\label{sec:dormant_heads}
 
 In this section, we will more carefully define dormant heads and show that they are ubiquitous on both pre-trained LLMs and small transformers trained via next-token-prediction.

\subsection{Dormant Head Conjecture} \label{sub:dormant_head_conjecture}

As in \Cref{sub:case_study_l25_h16}, we define a \textit{dormant attention head} as follows.
\begin{quote}
    \textit{An attention head is \underline{dormant} on a particular input if its output consists of only one (or a small number of) vector(s), repeated across every token index.}
\end{quote}
 The output of a dormant head does not respect the semantic content of the input, and essentially outputs a bias. Heads which are attention sinks are dormant attention heads, and indeed almost all (but not necessarily all) dormant attention heads are attention sinks. Our \textit{dormant heads conjecture} states that dormant heads are ubiquitous in LLMs. In particular, we say that a head which is not dormant is \textit{active}. Then, we conjecture the following:
 \begin{quote}
     \textit{\underline{Dormant heads conjecture:} for autoregressive transformer-based language models, a large fraction of heads are dormant on some inputs and active on some others.}
 \end{quote}
 In this section, we will provide evidence for this conjecture through finding a circuit in Llama 2 7B which creates dormant heads (\Cref{sub:circuit_evidence}), developing an automated detection system for attention sinks and thus showing that many heads in Llama 2 7B are empirically dormant on some inputs and active on others (\Cref{sub:lots_of_dormant_heads}), and showing that the dormant head phenomenon persists in small autoregressive transformers trained on next-token-prediction (\Cref{sub:controlled_experiments}).

\DP{TODO: description}

\subsection{Evidence 1 For Conjecture: Circuit for Dormant Heads in Llama 2} \label{sub:circuit_evidence}

\DP{TODO: description}

\begin{figure}[t]
  \centering
  % \begin{minipage}{0.24\textwidth}
  %     \centering
  %     \subcaption{\small Attention weights}
  %     \label{fig:circuit-attn-weights}
  %     \vspace{-.2em}
  %     \includegraphics[width=\linewidth]{Figures/figures_circuit/attn_weights_dormant.pdf}
  % \end{minipage}
  % \hspace{-1em}
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Attention logits}
      \label{fig:circuit-attn-logits}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/logits.pdf}
  \end{minipage}~
  % \hspace{-1em}
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Output norm}
      \label{fig:circuit-massive-norm}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/massive.pdf}
  \end{minipage}
  \hspace{-1em}
  \begin{minipage}{0.33\textwidth}
      \centering
      \subcaption{\small Value states norm}
      \label{fig:circuit-value-norm}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_circuit/values.pdf}
  \end{minipage}
  \vspace{-1em}
  \caption{\small \textit{Algebraic findings.} We sample ``\bos~Summer is hot. Winter is cold.'' $+$ ``random test token'''s for $1000$ times to obtain a distribution of hidden states in \llama. Figure \ref{fig:circuit-attn-logits} presents the attention logits computed by using the test tokens as queries and the previous tokens as keys. The logits on \bos~and the first \delim are effectively positive constants, with logits on other tokens vary among different test tokens, and being mostly negative. Figure \ref{fig:circuit-massive-norm} shows the norm of the outputs across all the layers, with the \bos~and the first \delim possessing significantly massive norms from layers 2 to 29. Figure \ref{fig:circuit-value-norm} shows the norm distribution of the value states across layers 2 to 29. The norms of the \bos~and the first \delim token are effectively small constants. 
  }
  \label{figure:algebra-findings}
  \vspace{-1em}
\end{figure}



We summarize the algebraic features of \bos~ and the first \delim tokens in the computation graph, all of which point to the dormant heads conjecture. Previous works discover parts of these features separately. As a demonstration, we randomly sample 1000 tokens from the vocabulary of \llama, prefix it with ``\bos~Summer is hot. Winter is cold.'' to form one test sequence, and implement the forward pass. By collecting  hidden states for each test sequence, it provides us with a distribution of hidden states.
\ref{figure:algebra-findings} summarizes the four algebraic features:
\begin{enumerate}
    \item \textit{Attention sink}: Figure XXX visualizes the attention weights. Before the first \delim, the attention weights from all tokens on \bos~are near 1. The \delim would split half of the attention weights on \bos.
    \item \textit{Stable attention logits}: Figure \ref{fig:circuit-attn-logits} presents the attention logits from the test token (query) on tokens in the prefix (key). The distribution comes from a fixed head, L16H25, with 1000 test tokens. The attention logits on \bos~and \delim are nearly constant across all test tokens, while vary a lot on other tokens. 
    \item \textit{Massive norms}: Figure \ref{fig:circuit-massive-norm} presents the norm of hidden states across layer 0 to 31, averaged among 1000 test sequences. The \bos~and \delim have norms around 500 to 1000 times of other tokens.
    \item \textit{Small value states}: Figure \ref{fig:circuit-value-norm} shows the norm distribution of norms of value states. The distribution comes from all heads from layer 2 to 29 and with 1000 test tokens. \bos~and the first \delim both possess negligible norm.
\end{enumerate}

\tianyu{I will postpone the circuit here}
The algebraic findings depict a potential circuit of the dormant mechanism. Figure XXX illustrates the entire procedure, which we summarize as follows:
\begin{enumerate}
    \item Preparatory phase (layer 0 and 1): The $\mlp$ of layer 1 adds an output with massive norm residual streams of \bos~and the first \delim tokens. Using causal ablations, we verify the function of each components in layer 0 and 1.
    \begin{enumerate}
        \item \tianyu{We need to discuss the names here} Both the $\MLP$ in layer 0 and 1 contribute to the formation of a XXX in layer 1.
        \item $\Attn$ in both layer 0 and 1 adjust the formation of XXX. For example, shown by zero-out intervention, L1H8 both assists the initial token to be XXX and suppresses the other tokens to be XXX.
        \item The \rope in $\Attn$ heads in layer 0 and 1 suppresses the formation of XXX starting from the second delimiter tokens.
    \end{enumerate}
    \item Dormant/active phase: At this stage, the residual streams of \bos~and the first \delim remain nearly untouched, since any outputs added on the residual stream have negligible norms. At the main time, the layer norm map them to a special direction XXX, which corresponds to a sink key state which has nearly constant attention logits fitted with any queries. The direction XXX also possesses minor value states,. As a result, a test token has two modes on the attention weights:
    \begin{itemize}
        \item dormant mode: when no other keys align with its queries. After the Softmax function, \bos~and the first \delim take up a great proportion of its attention weights
        \item active mode: when there's other key that aligns with its query, which renders a attention logits comparable or even greater than the attention logits on \bos. After the Softmax function, \bos~and the first \delim take up a small proportion of its attention weights.
    \end{itemize}
    Since the value states of \bos~and \delim are notably small,
    The different modes on attention weights lead to different     \begin{itemize}
        \item dormant mode: add a minor output on the residual stream
        \item active mode: add a large output on the residual stream
    \end{itemize}
\item Recover phase: On \bos~and \delim, the $\MLP$ in the last two layers add a massive norm on the residual, while on its negative direction. As a result, The norms of \bos~and \delim become normal. There's no dormant phenomenon in last two layers.
\end{enumerate}

After the preparatory work in layers $0$ and $1$, the


\subsection{Evidence 2 For Conjecture: Abundance of Dormant Heads in Llama 2} \label{sub:lots_of_dormant_heads}

\DP{TODO: description}

\subsection{Evidence 3 For Conjecture: Dormant Heads in Small Transformers} \label{sub:controlled_experiments}

We further demonstrate that attention heads learn to be dormant even under a toy task, which we call as the \textit{dormant copy} task. As illustrated in Figure \ref{fig:pretraining-dgp}, we generate the input sequence with three steps. First, we always start with a \bos~token. Second, on normal tokens, we use a pre-determined Markov transition probability $P_e$ to predict the next token. Third, on $k$ trigger tokens, instead of using the Markov transition $P_e$, we copy the previous token to the next position. Similar to \citet{bietti2024birth}, we choose the $P_e$ and the vocabulary from the estimated character-level bigram distribution on the tiny \textit{Shakespeare} dataset. We manually add the \bos~token to the character-level vocabulary of \textit{Shakesphere}, making it to contain $N_{voc}=66$ tokens in total. 
To avoid repeat occurrence of the \bos~token, We sample the second token from the estimated unigram distribution in the \textit{Shakespeare} dataset, but drop the sequence if it's a trigger token. We fix the trigger tokens as the $k=3$ most frequent tokens in the unigram distribution.

The optimal algorithm for the \textit{dormant copy} task is to predict the next token distribution with $P_e$ on normal tokens and with previous tokens on trigger tokens. The transformer structure allows it to replicate the optimal algorithm. With the dormant conjecture in mind, since normal tokens do not require any in-context mechanism, we expect the $\Attn$ layer is dormant with only the $\MLP$ layer takes effect. The trigger tokens require the copying from the previous token, on which we expect the $\Attn$ layer is active. 

To verify our dormant/active modes mechanism, we pre-train a transformer with $1$ layer and $1$ head on the \textit{dormant copy} task using ADAM for $10000$ rounds. The resulting transformer could match the optimal algorithm on the prediction loss. More importantly, we observe clear patterns of the $\Attn$ head being dormant or active. Figures \ref{fig:pretraining-attn-weights-dormant} and \ref{fig:pretraining-attn-weights-active} visualize the attention weights on different input sequences. Figure \ref{fig:pretraining-attn-weights-dormant} shows that the \Attn head is dormant, with all attention weights are on the \bos~token when there's no trigger token. As a result, the \Attn head only adds a constant to the residual stream of normal tokens. Figure \ref{fig:pretraining-attn-weights-active} shows that the \Attn head is active and attend on the previous tokens from trigger tokens, which adds information from the previous tokens on the residual stream of trigger tokens.

\begin{figure}[t]
  \centering
  \begin{minipage}{0.4\textwidth}
      \centering
      \subcaption{\small Data generating procedure}
      \label{fig:pretraining-dgp}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_copy.pdf}
  \end{minipage}
  \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Dormant}
      \label{fig:pretraining-attn-weights-dormant}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_copy/dormant_copy_attn_weights_seq0.pdf}
  \end{minipage}
  \hspace{-1em}
  \begin{minipage}{0.3\textwidth}
      \centering
      \subcaption{\small Active}
      \label{fig:pretraining-attn-weights-active}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_copy/dormant_copy_attn_weights_seq1.pdf}
  \end{minipage}
  % \vspace{-1em}
  \caption{\small \textbf{The dormant copy experiment.} Figure \ref{fig:pretraining-dgp} illustrates the data generating procedure of the dormant copy task. We fix `t', `e', and ` ' as three trigger tokens. Figure \ref{fig:pretraining-attn-weights-dormant} shows the attention weights on an input without triggers, with the $x$-axis representing the key tokens and the $y$-axis representing the query tokens. The \bos~token takes up nearly all the attention weights among all tokens. Figure \ref{fig:pretraining-attn-weights-active} shows the attention weights on an input with triggers. The \Attn head still puts all attention weights on normal tokens. However, it is active on trigger tokens and attend to the previous tokens.}
  \label{figure:pretraining-findings}
  \vspace{-1em}
\end{figure}

Moreover, on a pre-trained transformer with $3$ layers, we could recover all the algebraic features of the dormant mechanism in large language models. Figure \ref{fig:pretraining-massive-norm} presents the distribution of output norms of layer $1$ on different tokens, sampled from $512$ input sequences with each has $256$ tokens. The output norm of \bos~(around 100) is notably greater than most tokens. Surprisingly, the token $\backslash n$ has even greater norm. Figure \ref{fig:pretraining-small-value} presents the corresponding distribution of value states. Matching the massive norms of the output, \bos~and $\backslash n$ both possess remarkably small value states. It's unclear why the token $\backslash n$ also exhibits similar features with the \bos~token. We conjecture that similar to the first \delim token in \llama, the $\backslash n$ assists the dormant mechanism with the \bos~token. We delegate attention weights plots supporting this conjecture in the appendix.

\begin{figure}[t]
  \centering
  \begin{minipage}{0.4\textwidth}
      \centering
      \subcaption{\small Massive norms}
      \label{fig:pretraining-massive-norm}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_copy/dormant_copy_L3_massive.pdf}
  \end{minipage}
  \begin{minipage}{0.4\textwidth}
      \centering
      \subcaption{\small Small value states}
      \label{fig:pretraining-small-value}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_copy/dormant_copy_L3_minor.pdf}
  \end{minipage}
  \vspace{-1em}
  \caption{\small \textbf{The norms of hidden states in the dormant copy experiment} A summary of the norm distributions of the output of layer 1 (Figure \ref{fig:pretraining-massive-norm}) and the value states of layer 2 (Figure \ref{fig:pretraining-small-value}) in a 3-layer transformer trained on the \textit{dormant copy} task. The \bos~token is at the left most, with three trigger tokens ` ', `t', and `e' following it. We then randomly choose six tokens and separately summarize their norm distributions. We pull all other tokens together, forming the distribution of the norms of others at the right most. Only the \bos~and the $\backslash n$ token possess remarkably large output norms and small value states norms.}
  \label{figure:pretraining-findings-norms}
  \vspace{-1em}
\end{figure}

The inspection on the training dynamics enriches our understanding of the emergence of the dormant mechanism. Figure \ref{figure:pretraining-dynamics} summarises the change of multiple metrics along the training dynamics, including the ICL risk, the Markov prediction risk, the proportion of tokens that only attend to the \bos~token, the average attention weights on \bos, and the scaled norm of the output of layer 1 on \bos. Figure \ref{fig:pretraining-dynamics-long} presents their change along the entire training steps. The norm of the \bos~in layer 1 keeps increasing while other metrics remain unchanged. Figure \ref{figure:pretraining-dynamics} zooms in on the first 0 to 1000 steps along the training steps. The dynamics exhibit three phases: 1. Markov learning phase (0 to 140 steps): The prediction risk on normal tokens drops; the ICL risk firstly drops then stuck at a relatively high level; there is neither large attention weights nor massive output norms on the \bos~token. 2. ICL learning phase (140 to 240 steps): The prediction risk on normal tokens has negligible decrease; the ICL risk drops sharply; at the same time, the attention weights on the \bos~token increase and the output norms of \bos~slightly decreas. 3. Attention sink and massive norm formation phase (after 240 steps): the ICL risk decreases slowly and remains unchanged after 1000 training steps; the attention weights and the proportion of dormant tokens keep increasing; the output norm of \bos~keeps increasing along all training steps.

\begin{figure}[t]
\centering
    \begin{minipage}{0.4\textwidth}
      \centering
      \subcaption{\small From 0 to 10000 steps}
      \label{fig:pretraining-dynamics-long}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_copy/dormant_copy_dynamics_long.pdf}
  \end{minipage}
    \begin{minipage}{0.4\textwidth}
      \centering
      \subcaption{\small Zoom in on 0 to 1000 steps}
      \label{fig:pretraining-dynamics}
      \vspace{-.2em}
      \includegraphics[width=\linewidth]{Figures/figures_pretraining/dormant_copy/dormant_copy_dynamics.pdf}
  \end{minipage}
  \hspace{-1em}

  \vspace{-1em}
  \caption{\small \textbf{Training dynamics of the dormant copy experiment} The ICL risk computes the prediction risk on trigger tokens; the Markov risk computes the prediction risk on normal tokens; we count the number of tokens that have attention weights on the \bos~token greater than 0.9 and get the proportion of dormant tokens; we take the average attention weights on \bos~from normal tokens; for better visualization and since only the trend is important in our message, we scale down the output norm of \bos~by $20$. The training dynamics possess three phases, with the Markov risk drops first, then the ICL risk together with the attention sink, and finally the massive norm emerges.}
  \label{figure:pretraining-dynamics}
  \vspace{-1em}
\end{figure}


==> Sections_arxiv/deprecated_sections/findings.tex <==
\section{Findings}

Attention sink phenomenon: For autoregressive LLMs such as Llama2, in intermediate layers (all but layers 0, 1, 2, and -1) and most heads, the $N\times N$ attention matrix is heavily concentrated on the initial token.

Consider a fixed (layer, head) in which ``attention sink'' happens. Let $(\bq_i, \bk_i, \bv_i)_{i\in[N]}$ denote the (query, key, value) vectors for this head. Let $(\bh_i)_{i\in[N]}$ denote the hidden state vector. Let $s_{ij}$ denote the attention score of query token $i$ with respect to KV token $j\in[i]$. Attention sink refers to the phenomenon that
\begin{align*}
    s_{i1} \approx 1, \quad s_{ij}\approx 0~~\textrm{for}~~2\le j\le i.
\end{align*}

\paragraph{Our findings}
\begin{enumerate}
    \item Value norms exhibit ``reverse sink'':
    \begin{align}
    \label{eqn:value}
        \ltwo{\bv_1} \ll \ltwo{\bv_j}~~\textrm{for}~~2\le j\le i,
    \end{align}
    and they balance out the attention sink in the sense that
    \begin{talign*}
        \ltwo{s_{i1}\bv_1} \approx \ltwo{\sum_{j=2}^i s_{ij}\bv_j},
    \end{talign*}
    where ``$\approx$'' denotes the same order of magnitude. This means that the head is still non-degenerate, and is not approximable by a fixed value vector. Also, the ``sparse attention'' interpretation~\citep{block2023llm} is wrong.

    % \yub{However, we can use this to by-pass the partition function in softmax and speed up the attention computation (even in FlashAttention?)}

    \item Hidden state norms exhibit a sink:
    \begin{align*}
        \ltwo{\bh_1} \gg \ltwo{\bh_j}~~\textrm{for}~~2\le j\le i.
    \end{align*}
    Combined with~\cref{eqn:value}, it must happen that the value matrix $\bV$ is nearly orthogonal to $\bh_1$, compared with to $(\bh_j)_{j\ge 2}$.
\end{enumerate}

Ablations:
\begin{enumerate}
\item Most LLMs exhibit this phenomenon (this is more exacerbated with RoPE embedding, but standard trainable positional encoding schemes like GPT-2 also exhibits this).

\item This phenomenon shows up very early in training, but not at init. 
\end{enumerate}

==> Sections_arxiv/deprecated_sections/linear-algebra.tex <==


\section{Linear algebraic mechanisms behind sink tokens}

\tianyu{Massive tokens are not necessarily sink tokens in OOD?}

\yub{better title?}

\yub{In each subsection, we give a set of plots (in 1 - 2 lines), and give some explanation. If there is some further studies that naturall come after the initial set of plots, we give another set of plots.}

Throughout the rest of this section, we use LlaMa2-7B~\citep{touvron2023llama}.

\subsection{Birth of sink tokens}

\paragraph{How are sink tokens produced?}
% ~\yub{mostly done.}

\cref{fig:mlp1} shows that $\MLP_1$ produces the sink tokens, i.e. makes certain tokens have massive norms.


LlaMa's MLP layer is defined by three weight matrices $\sets{\Wgate, \Wdown, \Wup}$~\yub{dimensions} with the SwiGLU activation~\citep{shazeer2020glu}:
\begin{align}
    f_{\mlp}(\bh) = \Wdown \paren{ \silu\paren{ \Wgate\bh } \odot \paren{\Wup\bh} }.
\end{align}
Above, $\silu(t) \defeq t\cdot \sigmoid(t)$ denotes the SiLU (or Swish) activation~\citep{ramachandran2017searching}.

\begin{figure}[H]
\centering
\begin{minipage}{.32\textwidth}
\centering
    % \subcaption{{\footnotesize BLAH}}\label{fig:11}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/Summer/layer_1_attn_output.pdf}
\end{minipage}
% \hfill
\begin{minipage}{.32\textwidth}
    \centering
    % \subcaption{{\footnotesize BLAH}}\label{fig:12}
    %\vspace{-.7em}
    \includegraphics[width=.95\textwidth]{Figures/Summer/layer_1_attn_output_post_residual.pdf}
\end{minipage}
% \hfill
% \begin{minipage}{.24\textwidth}
%     \centering
%     \subcaption{{\footnotesize BLAH}}\label{fig:13}
%     %\vspace{-.7em}
%     \includegraphics[width=.95\textwidth]{Figures/Summer/layer_1_attn_output_post_ln.pdf}
% \end{minipage}
\begin{minipage}{.32\textwidth}
    \centering
    % \subcaption{{\footnotesize BLAH}}\label{fig:14}
    %\vspace{-.7em}
    \includegraphics[width=.95\textwidth]{Figures/Summer/layer_1_mlp_output.pdf}
\end{minipage}
\caption{
\small
Sink tokens (token 0 and token 3) are produced by $\MLP_1$. Sentence: ``Summer is warm. Winter is cold.''
\yub{maybe a better illustration is to track the evolution of all 8 tokens, one on each curve, x axis is the module name (along forward pass), y axis is norm.}
}
\label{fig:mlp1}
\vspace{-1em}
\end{figure}

% Group of plots for $\MLP_1$. Plot 0: Narrow it down to MLP1. Plot 1: Some flowchart. Plot 2 (maybe with one other plot that shows the shape of $W3[:, 7890]$): How massive tokens activate the $W_{\{1,2\}}[7890, :]$, and how $W3[:, 7890]$ produces massive entries at $1415, 2533$.


\begin{figure}[H]
\centering
\begin{minipage}{.32\textwidth}
\centering
    \subcaption{{\footnotesize Histogram of $\sets{\ltwos{\Wgate[i, :]}}_{i}$}}\label{fig:w1-norm}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/Summer/w1_norm_hist.pdf}
\end{minipage}
% \hfill
\begin{minipage}{.32\textwidth}
    \centering
    \subcaption{{\footnotesize $\<\bh_j, \Wgate[i, :]\>$}}\label{fig:corr-w1}
    %\vspace{-.7em}
    \includegraphics[width=.95\textwidth]{Figures/Summer/corr_with_w.pdf}
\end{minipage}
% \hfill
% \begin{minipage}{.24\textwidth}
%     \centering
%     \subcaption{{\footnotesize BLAH}}\label{fig:13}
%     %\vspace{-.7em}
%     \includegraphics[width=.95\textwidth]{Figures/Summer/layer_1_attn_output_post_ln.pdf}
% \end{minipage}
\begin{minipage}{.32\textwidth}
    \centering
    \subcaption{{\footnotesize $\Wdown[:, i]$}}\label{fig:w3}
    %\vspace{-.7em}
    \includegraphics[width=.95\textwidth]{Figures/Summer/w3.pdf}
\end{minipage}
\caption{
\small
Mechanisms of $\MLP_1$. (a) Neuron 7890 has the largest norm among all neurons in $\Wgate$. (b) $\Wgate[7890, :]$ has large positive inner products with sink tokens, and large negative inner products with non-sink tokens. (c) $\Wdown[:, 7890]$ has large entries at $[1415, 2533]$-th coordinate.
Sentence: ``Summer is warm. Winter is cold.''
}
\label{fig:special-neuron}
\vspace{-1em}
\end{figure}

\textbf{What does the special neuron tell us?} By computing the correlations of hidden states and $\Wgate[7890, :]$, we can detect important sub-layers that contribute to the massive tokens.

\begin{figure}[H]
\centering
\begin{minipage}{.24\textwidth}
\centering
    \subcaption{Layer 0 with ROPE}\label{fig:l0-rope-corr}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/tianyu_tentative/layer0wrope.png}
\end{minipage}
% \hfill
\begin{minipage}{.24\textwidth}
\centering
    \subcaption{Layer 1 with ROPE}\label{fig:l1-rope-corr}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/tianyu_tentative/layer1wrope.png}
\end{minipage}
\begin{minipage}{.24\textwidth}
\centering
    \subcaption{Layer 0 without ROPE}\label{fig:l0-norope-corr}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/tianyu_tentative/layer0norope.png}
\end{minipage}
\begin{minipage}{.24\textwidth}
\centering
    \subcaption{Layer 1 without ROPE}\label{fig:l0-rope-corr}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/tianyu_tentative/layer1norope.png}
\end{minipage}
\caption{
\small
Bar-plots of correlations between hidden states and $\Wgate[7890, :]$.
}
\label{fig:special-neuron}
\vspace{-1em}
\end{figure}


\paragraph{Why does the initial token always become a sink token?}
Our approach is to examine the forward pass of all 32K tokens in LlaMa tokenizer.

% Do all the 32000 tokens get to be attention sinks when placed at the initial position?~\yub{vast majority, but not all.}

\begin{figure}[H]
\centering
\begin{minipage}{.25\textwidth}
\centering
    \subcaption{{\footnotesize Norm after Layer 1}}\label{fig:initial-layer1-norm}
    %\vspace{-.7em}
    \includegraphics[width=\textwidth]{Figures/initial_token/token_0_layer_1_out_norms.pdf}
\end{minipage}
% \hfill
\begin{minipage}{.25\textwidth}
    \centering
    \subcaption{{\footnotesize Norm of embeddings}}\label{fig:initial-embed-norm}
    %\vspace{-.7em}
    \includegraphics[width=\textwidth]{Figures/initial_token/token_0_embed_norms.pdf}
\end{minipage}
% \hfill
% \begin{minipage}{.24\textwidth}
%     \centering
%     \subcaption{{\footnotesize BLAH}}\label{fig:13}
%     %\vspace{-.7em}
%     \includegraphics[width=.95\textwidth]{Figures/Summer/layer_1_attn_output_post_ln.pdf}
% \end{minipage}
\begin{minipage}{.48\textwidth}
    \centering
    \subcaption{Inner product with $\bw_\star$}\label{fig:ph}
    %\vspace{-.7em}
    \includegraphics[width=\textwidth]{Figures/initial_token/evolution_initial_token.pdf}
\end{minipage}
\caption{
\small
Evolution of token 0 along the forward pass. Here each sentence just consists of a single token.
}
\label{fig:special-neuron}
\vspace{-1em}
\end{figure}

% \yub{TODO(yub): Evolution of initial token to be aligned with $\bw_\star$. Choose one regular token, and one small token. Also work out a common plot scheme for evolution plots.}

% Plot 1. Out of the 32000 tokens, about 31800 of them gets to be massive when placed at the initial token (maybe use one plot). Plot 2: Evolution of initial token to be aligned with $\bw_\star$.

\yub{TODO(Tianyu): exhaust the list of delimiter tokens (among 32K tokens), defined as any token that becomes massive at non initial locations.}

\paragraph{Which head turns token 0 into sink token?}

\yub{Tianyu has some findings here (Attn1, Head8).}~\yub{Made a plot for Attn1 in~\cref{fig:attn1-heads-rope}.}

Head 8 in $\Attn_1$ is the main symmetry breaker here. See~\cref{fig:attn1-heads-rope}.

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{Figures/attn_0/attn_1_inner_prod_wstar.pdf}
    \caption{\small The inner product between $\Attn_1$'s \emph{OV output} in each head, and $\bw_\star$. We plot both across heads $m\in[M]$, and across tokens $\bh_i$ in the sequence. Sentence: ``Summer. Summer. Summer. Summer. Summer.'' We also consider a NoRoPE version where the RoPE in $\Attn_0$ is disabled. Observe that {\bf Head 8} produces a large output on the initial token.}
    \label{fig:attn1-heads-rope}
\end{figure}


\yub{Do we have an answer now for why initial token becomes massive? Based on Head 8}

\paragraph{Which head identifies delimiter tokens?}

When feeding LLM with a single token, the attention weights reduces to a point mass, and the attention output reduces to the summation of ``OV'' projections:
\begin{align}
    \Attn_0(\sets{\bh_0}) = \sum_{m=1}^M \bO_m\bV_m \bh_0, \quad \bO_m\in\R^{d\times (d/M)},~\bV_m\in\R^{(d/M)\times d}.
\end{align}

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{Figures/attn_0/attn_0_corr_wstar.pdf}
    \caption{\small The correlation of $\sets{\bO_m\bV_m\bh_0}_{m,\bh_0}\subset \R^d$ with $\bw_\star$ across both different heads $m\in[M]$, and across different tokens $\bh_0$ (corresponding to post-layernorm of the 32K token embeddings). Several heads identify the period token $29889$ (`.'). }
\end{figure}



\paragraph{Why the \emph{first} delimiter only?}
why does first delimiter become sink, and other layers not become sink?~\yub{TODO, some more symmetry breaking analysis with attention}

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{Figures/attn_0/attn_0_inner_prod_wstar.pdf}
    \caption{\small The inner product between $\Attn_0$'s \emph{OV output} in each head, and $\bw_\star$. We plot both across heads $m\in[M]$, and across tokens $\bh_i$ in the sequence. Sentence: ``Summer. Summer. Summer. Summer. Summer.'' We also consider a NoRoPE version where the RoPE in $\Attn_0$ is disabled. Observe that for {\bf Head 28}, the versions with and without RoPE differ significantly in their patterns.}
    \label{fig:attn0-heads-rope}
\end{figure}

% $w_\star^{(0)}=W_1^{(0)}[7374, :]$
Message: 1. We find, Head 28 in Attn 0 actually got impacted a lot by Rope. First, for period token, its OV state by head 28 produces a large negative correlation with $\bw_\star$ (see~\cref{fig:attn0-heads-rope}). Then, if there is rope in head 28 (as in regular LLM), then second period onward will attend significantly to prevoius period tokens. As a result, the attention output gives get large negative correlation. However, if there is no rope in head 28, then basiccally this negative correlation won't affect things, and period tokens would have positive correlation with $w_\star^{(0)}$. 

\begin{figure}[H]
\centering
\begin{minipage}{.32\textwidth}
\centering
    \subcaption{Attention weights of head 28 in layer 0}\label{fig:l0-h28-attn}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/tianyu_tentative/attn1 28.png}
\end{minipage}
% \hfill
\begin{minipage}{.32\textwidth}
\centering
    \subcaption{Cumulative correlations with $\bW_0[7374, :]$ across attention layer 0}\label{fig:attn-head-corr}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/tianyu_tentative/attn2 cum corr.png}
\end{minipage}
\begin{minipage}{.32\textwidth}
\centering
    \subcaption{Correlations between value states and $\bW_0[7374, :]$}\label{fig:value-corr}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/tianyu_tentative/values_w0star corr.png}
\end{minipage}
\caption{
\small
Mechanisms for the break of symmetry on the second delimiter.
}
\label{fig:special-neuron}
\vspace{-1em}
\end{figure}

\begin{figure}[H]
\centering
% \hfill
\begin{minipage}{.45\textwidth}
\centering
    \subcaption{Cumulative correlations with $\bW_1[7890, :]$ across attention layer 1}\label{fig:attn1-head-corr}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/tianyu_tentative/attn1 cum corr.png}
\end{minipage}
\begin{minipage}{.45\textwidth}
\centering
    \subcaption{Correlations between value states and $\bW_1[7890, :]$}\label{fig:value1-corr}
    %\vspace{-.7em}
    \includegraphics[width=0.95\textwidth]{Figures/tianyu_tentative/values w1star corrs.png}
\end{minipage}
\caption{
\small
Mechanisms for the break of symmetry on the second token.
}
\label{fig:special-neuron}
\vspace{-1em}
\end{figure}




The later mechanism in $\MLP_0$ and consequently $\MLP_1$ dictates that, a positive correaltion with $w_\star^{(0)}$ makes the token massive.


\subsection{Attention concentration}

\yub{Put initial plots + study in more depth.}

\subsection{Value anti-concentration}

\yub{Put initial plots + study in more depth.}

\subsection{Something else...?}

\yub{what happens for other architectures? Mainly mistral 7B.}

\yub{training dynamics? (can do this for either GPT2, or XGen-7B), for which we can obtain the model checkpoints.}

==> Sections_arxiv/deprecated_sections/sink-tokens.tex <==
\section{Sink tokens in LLMs}

\subsection{Transformers}

\subsection{Sink tokens}

\yub{Formalize language: what we mean by ``initial token'', ``delimiter token'', etc, is the hidden states vectors in the middle.}

==> Sections_arxiv/deprecated_sections/sparsify.tex <==
\section{Attention sparsification for accelerated inference}

\yub{Question: how does it reconcile with the value anti-concentration thing.}

\yub{Normalize could have played a role?}

==> Sections_arxiv/deprecated_sections/theory.tex <==
\section{Theory}
Let \( N^{(\ell)} \) be the number of $(\ell)$ tokens in front of a Markov token, let \( \beta^{(\ell)} \be_{\ell} \) be the corresponding value state. 
state, and let \( p_{k} \) be the Markov transition probability, i.e., $P( k \mid \text{current term})$.

\[
\text{Loss} = \sum_k p_k \left[ \log \left( \sum_{\ell} p_\ell e^{\frac{\beta^{(\ell)}N^{(\ell)}}{e^y+N}}\right) - \frac{\beta^{(\ell)}N^{(\ell)}}{e^y+N} - \log p_k\right].
\]

(I later realized that we should use $e^x\approx 1+x+x^2/2$ and $\log(1+x)\approx x$ to approximate.

==> Sections_arxiv/discussion.tex <==
\section{Discussion and Implications}\label{sec:discussion}



==> Sections_arxiv/intro.tex <==
\section{Introduction}
%Large language models (LLMs) \citep{brown2020language,touvron2023llama,dubey2024llama} have demonstrated remarkable capabilities, including text comprehension \citep{devlin2018bert}, generation \citep{radford2019language,goyal2020evaluating,roziere2023code}, and reasoning \citep{raffel2020exploring,wei2022chain}. A significant proportion of LLMs research focuses on external behaviors, such as task-based evaluations \citep{srivastava2022beyond,bubeck2023sparks} and designing prompts to enhance performance \citep{liu2021generated,wang2022self}. However, the inner mechanisms of LLMs remain largely unexplored, with ongoing concerns about the validity of their interpretability \citep{ghorbani2019interpretation,wen2024transformers}, and the theoretical understanding of transformers \citep{vaswani2017attention}, the core components of LLMs, is still limited.

Recent analyses of transformer-based open-source large language models (LLMs), such as GPT-2 \citep{radford2019language}, Llama-2 \citep{touvron2023llama}, Llama-3 \citep{dubey2024llama}, Mixtral \citep{jiang2023mistral}, Pythia \citep{biderman2023pythia}, and OLMo \citep{groeneveld2024olmo}, have revealed several intriguing phenomena: 
\begin{itemize}[leftmargin=2em]
\setlength\itemsep{0pt}
\item \textbf{Attention sinks} \citep{xiao2023efficient}: In many attention heads, the initial token consistently attracts a large proportion of attention weights. In certain LLMs, other special tokens, such as the delimiter token, also draw significant attention. We refer to these as \textit{sink tokens}. 
\item \textbf{Value state drains} \citep{guo2024attention}: The value states of sink tokens are consistently much smaller than those of other tokens. 
\item \textbf{Residual state peaks} \citep{sun2024massive}: The intermediate representations of sink tokens, excluding those from the first and last layers, exhibit a significantly larger norm than other tokens.
\end{itemize}
These phenomena often appear simultaneously, and we collectively refer to them as the \textbf{extreme-token phenomena}. Figure \ref{figure:extreme-token} illustrates these phenomena using a fixed prompt: ``\bos~Summer is warm. Winter is cold.'' in Llama-3.1-8B-Base, where the first token, \bos, the beginning-of-sentence token, serves as the sink token. We note that the first token does not have to be \bos~to function as a sink token, as in GPT-2, where other tokens, being the initial token, can also serve this role. Furthermore, in models like Llama-2, a delimiter token can also act as the sink token. Despite the consistency of these observations, no prior work has provided a satisfying explanation for the mechanisms behind these phenomena. As a tentative explanation, \citet{xiao2023efficient} suggested that models tend to dump unnecessary attention values to specific tokens. 

This work aims to demystify the extreme-token phenomena in LLMs. We show that the extreme-token phenomena are manifestations of the \textit{active-dormant mechanism} of attention heads. We support this claim through studies on simplified transformer architectures and tasks, a dynamical theory of simplified models, and experiments on pre-trained LLMs. Our contributions are as follows: 
\begin{enumerate}[leftmargin=2em]
\setlength\itemsep{0pt}
\item In \Cref{sec:bb_task}, we train one-to-three-layer transformers on the \textit{Bigram-Backcopy} (BB) task, which also exhibits extreme-token phenomena similar to those observed in LLMs. We show that attention sinks and value-state drains are driven by the \activedormant~mechanism. Both theoretically and empirically, we demonstrate that the mutual reinforcement dynamics underpin the extreme-token phenomena: attention sinks and value-state drains reinforce each other, leading to a stable phase where all query tokens produce identical attention logits for the keys of extreme tokens. Empirical evidence further shows that residual state peaks result from the interaction between this mutual reinforcement mechanism and Adam. 
\item In \Cref{sec:llm}, we demonstrate the \textit{\activedormant}~mechanism in LLMs by identifying an interpretable active-dormant head (Layer 16, Head 25 in Llama 2-7B-Base \citep{touvron2023llama}), confirmed through causal intervention analyses. We also discover circuits in LLMs related to extreme tokens that partially align with models trained on the BB task. Examining the dynamics of OLMo-7B-0424 \citep{groeneveld2024olmo}, we observe the same mutual reinforcement mechanism and stable phase, consistent with predictions from the BB task. 
\item Through causal interventions, we isolate the extreme-token phenomena to architecture and optimization strategy. Specifically, we show that replacing SoftMax with ReLU activations in attention heads can eliminate extreme-token phenomena in the BB task, and switching from Adam to SGD removes the residual-state peak phenomenon in the BB task. Our work demonstrates potential classes of modifications to mitigate extreme-token phenomena in LLMs. %\tianyu{I still feel that this looks not so strong.} %\DP{The phrasing should be like: We conclusively demonstrate that the extreme-token phenomenon is a property of the specific architecture and optimization procedure, and show this via two ablation tests in the BB task: replacing SoftMax with ReLU in the attention mechanism and switching Adam to SGD. Our work demonstrates potential classes of mechanisms to mitigate extreme-token phenomena in LLMs.}
\end{enumerate}

\yub{We release our code at the following anonymous repo: XXX.}
% \begin{enumerate}[leftmargin=2em]
% \setlength\itemsep{0pt}
% \item We design the \textit{Bigram-Backcopy} (BB) task, train one-to-three layer transformers, and recapitulate the extreme token phenomena, offering a framework for understanding the \activedormant. Both theoretically and empirically, we demonstrate the mutual reinforcement dynamics of the extreme token phenomena. Our key finding is that the attention sinks and value state drains reinforce each other in the dynamics, leading to the stable phase consists of identical attention logits from all query tokens to the key of extreme tokens. With empirical evidence, we demonstrate that residual state peaks result from the interaction of this mutual reinforcement mechanism with Adam.
% \item Extending the findings from small models to LLMs, we first discover an interpretable active-dormant head (Layer 16 Head 25 in Llama 2-7B-Base \citep{touvron2023llama}), verified through causal interventions. We also discover circuits in LLMs for the extreme tokens that partially match the models trained for the BB task. We inspect the dynamics of OLMo-7B-0424 \citep{groeneveld2024olmo}, identifying the same mutual reinforcement mechanism and stable phase, consistent with predictions from the BB task analysis.
% \item As broader implications, we demonstrate potential design choices to mitigate extreme-token phenomena in LLMs. we propose two methods to eliminate the extreme-token phenomena based on the discovered mechanisms: replacing SoftMax with ReLU activations in attention heads and switching Adam to SGD, both verified in the BB task. \tianyu{I still feel that this looks not so strong.} \DP{The phrasing should be like: We conclusively demonstrate that the extreme-token phenomenon is a property of the specific architecture and optimization procedure, and show this via two ablation tests in the BB task: replacing SoftMax with ReLU in the attention mechanism and switching Adam to SGD. Our work demonstrates potential classes of mechanisms to mitigate extreme-token phenomena in LLMs.}
% \end{enumerate}



\begin{figure}[t]
  \centering
  \begin{subfigure}[t]{0.32\textwidth}
      \centering 
      \caption{\small Attention weights at L24.}
      \includegraphics[width=\textwidth]{Figures/demo_attn_sink.png}
      \label{fig:attention_sinks_wide_random}
  \end{subfigure}
  \hfill
  % \begin{subfigure}[t]{0.32\textwidth}
  %     \centering 
  %     \includegraphics[width=\textwidth]{Figures/attn_logits_random_tokens.png}
  %     \caption{\small Attention logits \(\langle \bm{q}_{\mathrm{test}}, \bm{k}_{j}\rangle\).}
  %     \label{fig:attention_logits_random}
  % \end{subfigure}
  \begin{subfigure}[t]{0.3\textwidth}
      \centering 
      \caption{\small Norms of residual states.}
      \includegraphics[width=\textwidth]{Figures/residual_norms.png}
      \label{fig:token_norms_massive}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.3\textwidth}
      \centering 
      \caption{\small Norms of value states.}
      \includegraphics[width=\textwidth]{Figures/value_state_norms.png}
      \label{fig:value_norms_zeroed}
  \end{subfigure}
  
  % \begin{minipage}{0.33\textwidth}
  %     \centering
  %     \subcaption{\small Attention logits}
  %     \label{fig:circuit-attn-logits}
  %     \vspace{-.2em}
  %     \includegraphics[width=\linewidth]{Figures/figures_circuit/logits.pdf}
  % \end{minipage}~
  % % \hspace{-1em}
  % \begin{minipage}{0.33\textwidth}
  %     \centering
  %     \subcaption{\small Residual states norm}
  %     \label{fig:circuit-massive-norm}
  %     \vspace{-.2em}
  %     \includegraphics[width=\linewidth]{Figures/figures_circuit/massive.pdf}
  % \end{minipage}
  % \hspace{-1em}
  % \begin{minipage}{0.33\textwidth}
  %     \centering
  %     \subcaption{\small Value states norm}
  %     \label{fig:circuit-value-norm}
  %     \vspace{-.2em}
  %     \includegraphics[width=\linewidth]{Figures/figures_circuit/values.pdf}
  % \end{minipage}
  \vspace{-2em}
  \caption{\small \textbf{Extreme-token phenomena in Llama 3.1-8B-Base.}
  %\tianyu{bigger text size; remove all labels in the middle of fig (a); notations; thicker lines;  remove all test tokens. backup plan: include more heads} 
  We evaluate the sentence ``\bos~Summer is warm. Winter is cold.'' on the Llama 3.1-8B-Base model. \textit{Left (a):} The value of the attention weights across multiple heads at Layer 24. We demonstrate that there are \textit{attention sinks}: the key state associated with the \bos{} token attracts the most attention from query states in these (and most) heads. 
 % Figure \ref{fig:attention_logits_random} displays the distribution of attention logits \(\langle \bm{q}_{\mathrm{test}}, \bm{k}_{i}\rangle\) across all heads and test tokens at Layer 24. %\sm{which head?}. 
  %The logits for the \bos~token 
  %~and the first \delim~
  %are concentrated at large values, while those for other tokens are smaller and fluctuate across different random test tokens. 
  \textit{Middle (b):} The norm of the (residual stream) hidden states, measured at the output of each layer. We observe a \textit{residual state peak} phenomenon: the \bos~token's residual states have significantly larger norms than those of other tokens from layers 1 to 30. 
  %\sm{1 to 30?} \DP{Yes, 1-30}
  \textit{Right (c):} The distribution of the norms of value states corresponding to each token at all layers 
  %\sm{all or 1-30?} \DP{all}
  and all heads. We observe the \textit{value state drain} phenomenon: across many attention heads, the value state of the \bos~token is much smaller than those of other tokens on average. %\sm{Edit figure}
  }
  \label{figure:extreme-token}
  \vspace{-1em}
\end{figure}



% \yub{LLMs...}~\yub{a sophisticated but extremely powerful system}~\yub{however are there any structural biases?}

% \yub{some recent works identify an intruiging phenomenon in trained LLMs.}~\yub{describe the sink token phenomenon.}~\yub{two features: massive in norm, and caused by massive in specific entries~\citep{sun2024massive}, and attract attention scores (give rigorous description)~\citep{xiao2023efficient,darcet2023vision}}~\yub{Has been used in applications such as Streaming LLM generation~\citep{xiao2023efficient,han2023lm}.}

% Despite the intriguing findings, the understanding is still~\yub{at a surface level}, with many questions unanswered.~\yub{1. what tokens get to be sink tokens, and how is this process related to the position of the tokens in the sequence?}~\yub{second delimiter thing...}~\yub{2. is attention concentration phenomenon a consequence of the massive norms?}~\yub{3. Does attention concentration imply that non-sink tokens are not important to the final attention output?}


% In this work, we provide a more in-depth understanding on how sink tokens arise and take effect in trained LLMs. Our contributions can be summarized as follows.
% \begin{itemize}
%     \item BLAH.
% \end{itemize}



\subsection{Notation}
We denote the SoftMax attention layer with a causal mask as $\attn$, the MLP layer as $\mlp$, and the transformer block as $\TF$. The query, key, value states, and residuals of a token $\tok$ are represented as $\query_\tok$, $\key_\tok$, $\val_\tok$, and $\res_\tok$, respectively, with the specific layer and head indicated in context. We use \bos~to refer to the "Beginning of Sequence" (bos) token. Throughout the paper, we employ zero-indexing (i.e., attention head and layer indices start from 0 rather than 1) for consistency between code and writing. 


==> Sections_arxiv/llm.tex <==
\section{Extending Predictions of the BB Model to LLMs} \label{sec:llm}

%\DP{TODO for SONG: rewrite this paragraph}
% \DP{TODO for DRUV: check again after Song finishes}

In this section, we examine extreme-token phenomena in open-source pre-trained LLMs. In \Cref{sub:active_dormant}, we analyze the static behavior of these phenomena in Llama 2-7B-Base \citep{touvron2023llama}, confirming that certain attention heads in LLMs exhibit both active and dormant phases. Notably, we identify a specific head that is active on GitHub samples but dormant on Wikipedia samples, illustrating the \textit{active-dormant mechanism}. In \Cref{sub:olmo_dynamics}, we explore the dynamic behavior of extreme-token phenomena during the pre-training process of OLMo-7B \citep{groeneveld2024olmo}. We show that the attention logits, value state norms, and residual state norms of the sink token(s) in OLMo mirror their behavior in the simpler BB model. Specifically, the simultaneous formation of attention sinks and value state drains gives evidence for the \textit{mutual reinforcement mechanism}.

% It turns out that our exploration into the BB task in \Cref{sec:bb_task} may actually shed light upon the origin of attention sinks, small value states, and massive norms in full-fledged large language models trained on massive amounts of text. To verify this claim, we once again summarize and elaborate the observations we made in the BB task model:
% \begin{enumerate}[leftmargin=2em]
% \setlength\itemsep{0pt}
%     \item The attention sinks and value state drains are external manifestations of the active-dormant mechanism in LLMs. 
%     \item The lower-layer components (e.g., attentions and MLPs) of the LLM contribute to all three extreme-token phenomena.     
%     \item The attention heads go through the attention-increasing and value-state-shrinking phase. They converge to the stable phase, with identical attention logits on the \bos~token. Meanwhile, the residual state norm corresponding to the \bos{} token linearly increase during pre-training.
% \end{enumerate}

% We will confirm each of these observations in this section.\footnote{Here, we mention that in order to achieve this checklist, we had to do a certain amount of translating from the setting of the BB model to the setting of LLMs. For example, the BB model identifies trigger tokens as the (semantically) important tokens in that the model should change behavior after seeing them. In the context of LLMs, almost every token fits this description for a suitable context, but tokens like \bos{} do not. 
% %\tianyu{I think we should say that each token could be trigger or non-trigger, depending on the context? If every tokens are triggers, there's no dormant phase.}
% } Namely, in \Cref{sub:active_dormant} we will confirm point 1; in \Cref{sub:circuits} we confirm point 2; and in \Cref{sub:olmo_dynamics} we confirm point 3.


\subsection{Active-Dormant Mechanism in LLMs}\label{sub:active_dormant}

Our study of the BB model leads to the following prediction about the extreme-token phenomena, which we hypothesize also applies to LLMs:  
\begin{center}
    \textit{Attention heads are controlled by an active-dormant mechanism. Attention sinks and value state drains indicate that an attention head is in dormant phase.}
    %\textit{If all tokens at a head do not have helpful value states for predicting the next token, then attention mass will concentrate on tokens which are generally unhelpful for next-token prediction (like \bos). \sm{Attention heads are controlled by the active-dormant mechanism; attention sinks and value state drains are the dormant phases of attention heads. }}
\end{center}

This hypothesis suggests that in LLMs, attention heads become sinks or not depending on the context: the value vector can be totally non-informative towards picking likely next tokens for token distributions (e.g., tasks) in a particular context but not in others. This is a concrete instantiation vis-a-vis large-scale LLMs of the active-dormant dichotomy in \Cref{sec:bb_task}, where this phenomenon was shown to occur in the context of small next-token predictors and the BB task. 

Accordingly, we strive to find instances of heads in pretrained LLMs which satisfy this principle, i.e., which are dormant on some domains and active on others. In \Cref{fig:dormant_heads_domain_dependent}, we show a particular attention head -- Layer 16 Head 25 of Llama 2-7B-Base \citep{touvron2023llama} --- which has an extremely clear active-dormant distinction across two distinct contexts (e.g., tokens from RedPajama \citep{together2023redpajama} drawn from the GitHub subset versus the Wikipedia subset). While there are many such attention heads which are context-dependent --- we provide some in \Cref{sec:more_heads} --- we demonstrate this one because the conditions under which it is active are simple and interpretable, while others have more involved or complex criteria to become active. We observe that this attention head is \textit{dormant} (i.e., an attention sink) on samples from Wikipedia, which more closely resemble prose, and \textit{active} (i.e., not an attention sink) on samples from Github, which more closely resemble code. We also observe that this attention head, in general, contributes significantly to the performance of the model on code sequences, but has negligible impact on the performance of the model on prose sequences (\Cref{fig:github_wikipedia_zero_out}). This is a further justification, from a practical perspective, of why this head is sometimes dormant and sometimes active --- in some contexts we can ablate it from the model entirely with no effect, but in other contexts ablating the head leads to huge performance drops. %\footnote{Llama 2-7B-Base has two sink tokens (\bos~and one more) in its attention sink heads, while Llama 3.1-8B-Base only has one (\bos). We discuss a potential reason in \Cref{sub:multiple_sinks_discussion}. \sm{Why we put this remark here?}} \sm{Talk about other heads also has dormant and active phase, though not interpretable. Ablation figures in appendix. } \DP{@SM: the first part is already in the paragraph.} \sm{It would be good to link to figures for other heads. } \DP{sure will add to appendix, and comment out this comments when done}
We include more detail in \Cref{sec:circuit}, where we extract a circuit for extreme-token phenomena in order to analyze the dormant-active mechanism and its interaction with the semantics of the input tokens.

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \caption{\small Attention weights for GitHub/Wikipedia data.}% \sm{Maybe 2 by 2? }}
        \includegraphics[width=\textwidth]{Figures/L16_H25/attn_weights_l16h25_github_revised.png}
        
        \includegraphics[width=\textwidth]{Figures/L16_H25/attn_weights_l16h25_wikipedia_revised.png}
        \label{fig:github_wikipedia_weights}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.44\textwidth}
        \caption{\small Zero-out-head intervention outcomes.}
        \label{fig:github_wikipedia_zero_out}
        \includegraphics[width=\textwidth]{Figures/BBM/LLM_interventions.pdf}
    \end{subfigure}
    \vspace{-1.5em}
    %\includegraphics[width=0.5\linewidth]{}
    \caption{\small \textbf{Attention heads in LLMs are active on some domains and dormant on others.} For example, on Llama 2-7B-Base, we identify that Layer 16 Head 25 is active when the context contains many tokens related to programming, and dormant in other contexts such as prose. We use RedPajama-1T \citep{together2023redpajama} Wikipedia and Github subsets for our data in this figure, truncating all samples to 64 tokens for demonstration purposes. \textit{Left:} Sample weights from four randomly selected samples from each domain. \textit{Right:} Result of an intervention study, i.e., change in cross-entropy of the input sequence when the attention head's output (concretely, the value states for this head) is manually set to zero, across sequences in both domains. We observe that the model's performance, measured by cross-entropy, strongly depends on the output of the attention head on coding data.
    % heads are sinks in one domain and not others (Llama 2 7B L16H25, Github vs Wikipedia) \DP{TODO...}
    % \DP{Plan: two figures. Left: attn sink visualization for Github on left and Wikipedia (4x4 (adjust to be visually appealing) samples visualize L16H25). Right: causal intervention, zeroing out head vs cross entropy delta taken across many samples from Github and Wikipedia.}
    }
    \label{fig:dormant_heads_domain_dependent}
\end{figure}


\subsection{Training Dynamics of Extreme-Token Phenomena in LLMs}\label{sub:olmo_dynamics}


Our study of the BB model leads to the following prediction about the dynamical behavior of the extreme-token phenomena, which we hypothesize also applies to LLMs:  
\begin{center}
    \textit{The attention heads go through a attention-increasing and value-state-shrinking phase. They then go into a stable phase, with identical attention logits on the \bos~token. Meanwhile, the residual state norm of the \bos{} token linearly increases during pre-training.}
\end{center}

% We confirm these predictions below, thus demonstrating the overall validity of the BB task as a model for extreme token phenomena in LLMs. 
We confirm these predictions below. To observe the training dynamics of a large-scale LLM, we use the setup of OLMo-7B-0424 \citep{groeneveld2024olmo} (henceforth just referred to as OLMo), who have open-sourced weights at several steps during their training run. For our analysis, we inspect OLMo at a variety of training steps: every 500 steps throughout the first 10,000 steps, then 25,000 steps, then 50,000 steps, then every 50,000 steps until 449,000 steps (which is roughly the end of their training). Again, we use the input ``Summer is warm. Winter is cold.''.\footnote{Note that OLMo does not have a \bos{}~token, but attention sinks still form in the majority of heads. In particular, the first token behaves similarly to an attention sink. We discuss this in \Cref{sub:fixed_bos}.} Notice that in this prompt, token \(3\), namely ``.'', is not very semantically meaningful; it becomes a sink token along with token \(0\) (c.f. \Cref{sub:active_dormant}, \Cref{sec:circuit}, \Cref{sub:fixed_bos}).

In \Cref{fig:olmo_predictions_phase0}, we confirm that attention heads go through an attention-increasing and value-state-shrinking phase, and that the residual state norm of the \bos{} token increases linearly during pre-training. We show that, at Layer 24 of OLMo, the average attention on extreme tokens (token \(0\) and token \(3\)) increases rapidly at the beginning of training and converges to a constant, while the value state norms of extreme tokens decrease rapidly. Also, the residual states of extreme tokens also increase linearly, while the rest quickly converge. In \Cref{fig:olmo_predictions_phase1} we show that attention heads converge to a stable phase, and that all logits corresponding to the first token's value states (i.e., all tokens' value of \(\mathrm{logit}_{0}\), except possibly the value of \(\mathrm{logit}_{0}\) corresponding to token \(0\) itself) have similar distributions. These confirm our dynamics insights from the BB model (c.f. \Cref{figure:verify-assumptions}). %\sm{These echos the findings from the BB model. Link figure 3b here. }

\begin{figure}[thp]
    \centering
    \begin{subfigure}[t]{0.32\textwidth}
        \centering 
        \caption{\small Attention sink dynamics (L24).}
        \includegraphics[width=\textwidth]{Figures/olmo/olmo_sink.png}
        \label{fig:olmo_sink}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering 
        \caption{\small Value state dynamics (L24).}
        \includegraphics[width=\textwidth]{Figures/olmo/olmo_value_states.png}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \centering 
        \caption{\small Residual state dynamics (L24).}
        \includegraphics[width=\textwidth]{Figures/olmo/olmo_massive_norms.png}
    \end{subfigure}
    \vspace{-2em}
    \caption{\small \textbf{Attention-increasing and value state-decreasing phase, and residual state norms.} \textit{Left (a):} We plot the total attention mass on extreme tokens \(0\) and \(3\) at Layer 24 and averaged over all attention heads, during OLMo training. We observe that it increases rapidly and then maintains its value in \([0.9, 1]\) for the rest of training, which is in line with our predictions. \textit{Middle (b):} We plot the norm of each token's value state at Layer 24 during training, averaged over all heads. We observe that the value states of all tokens shrink initially and then converge, while the value states of the extreme tokens shrink to much lower than all other tokens. \textit{Right (c):}  We plot the norm of each token's residual state at Layer 24 during training. We observe that the residual state of token \(0\) increases linearly in magnitude during training.}
    \label{fig:olmo_predictions_phase0}
\end{figure}

\begin{figure}[thp]
    \centering
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \centering 
        \caption{\small Logit dynamics (L24).}
        \includegraphics[width=\textwidth]{Figures/olmo/olmo_logits.png}
        \label{fig:attention_logits_olmo_dynamic}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \centering 
        \caption{\small Logit statics (L24).}
        \includegraphics[width=\textwidth]{Figures/olmo/olmo_logits_static.png}
        \label{fig:attention_logits_olmo_static}
    \end{subfigure}
    \hfill
    \phantom{.}
    \vspace{-2em}
    \caption{\small \textbf{Stable phase.}  \textit{Left (a):} We plot the normalized attention logits of all tokens' query states against token \(0\)'s key state during training. We observe that the logits of all non-extreme tokens' query states against token \(0\)'s key state in OLMo's Layer 24 are stable for a large fraction of the training run, after an initialization period. This echoes the stable phase prediction made in the BB model in \Cref{sec:bb_task}. Note that this prediction makes no guarantees about the logit corresponding to the zeroth query token and zeroth key token, which will be set to \(1\) by the softmax and so its behavior is irrelevant for prediction. Also note that we use normalization, similar to \Cref{sec:bb_task}, to make all terms comparable; namely we have \(\mathrm{logit}_{i} = \langle \query_{i}, \key_{0}\rangle - \mathtt{mean}_{j}(\langle \query_{i}, \key_{j}\rangle)\). \textit{Right (b):} For this experiment, we generate \(128\) randomly sampled test tokens with IDs from \(100\) to \(50000\) in the OLMo tokenizer. We append each token separately to the test phrase ``Summer is warm. Winter is cold.'', creating \(128\) different samples, which we feed to the LLM to record the model behavior. We plot the distribution of (un-normalized) dot products \(\langle \query_{\mathrm{test}}, \key_{j}\rangle\) across all heads at Layer 24 and all test tokens. We observe that logits of all regular tokens have very similar distributions, and the distributions of the logits corresponding to extreme tokens \(0\) and \(3\) are also similar. This confirms the hypothesis that at the end of training, attention heads converge to the stable phase, with similar logits on extreme tokens.}
    \label{fig:olmo_predictions_phase1}
\end{figure}



% Outline:
% \begin{itemize}
%     \item OLMo value states at a middle layer are roughly constant over time except for bos token and first delimiter
%     \item Massive norm keeps increasing over time 
%     \item Attention sink occurs very rapidly and stays constant over time
% \end{itemize}

% \begin{figure}
%     \centering
%     %\includegraphics[width=0.5\linewidth]{}
%     \caption{Training dynamics of value states, massive norm, and attention sink via OLMo
%     \DP{TODO: for attention logits plot, put linear plot for first 10k epochs (halfway through axis) and log plot for remaining epochs; do the same for value states; plot multiple heads for value plot}}
%     \label{fig:enter-label}
% \end{figure}














==> Sections_arxiv/plans.tex <==
\section*{Outline}
\begin{itemize}
    \item \sm{Title: Birth of Attention Sink in Large Language Models}
    \item \tianyu{Title: Switching Attention Heads: Mechanistically Demystifying Outlier Phenomena in LLMs}
    \item \DP{Title: Outlier Phenomena in Large Language Models}
\end{itemize}
% \paragraph{Some concepts: }
% \begin{itemize}
%     \item Dormant attention head: given an input, a head that effectively outputs a bias, i.e., doesn't have cross token interactions
%     \item Active attention head: a head which is not dormant on the particular input
%     \item Relate dormant attention head to attention sink: the attention sink is nearly the only possible mechanism for a head to be dormant while remaining the ability to be active
%     \item Functional head: head which has some defined function(s) during forward pass
%     \item Indexing: from 0
%     \item Attention weights: The attention weight from token $i$ to the BOS is large.
%     \item Massive token \& Massive activation (need to clarify in the preliminaries)
%     \item Dormant head token score = attention score of BOS + all delimiter tokens
%     \item Dormant head detection metric = (maximum/mean) dormant head token score over all tokens in the sample
%     \item Dormant head detection thresholds = bound for dormant head detection metric, above (resp.~below) which the head is classified as dormant (resp.~active) on the given sample
%     \item \sm{Suggested name for "Dormant copy model": Bigram-Backcopy Model (BBM) or Markov Backcopy Model (MBM). }
%     \item  \sm{Message: The observed sink heads are not always dormant. Every head has a dormant phase and an active phase. In the active phase, the head transports information from previous tokens to the current one. In the dormant phase, the head behaves as if it is constantly biased. Plot the histogram of dormant metric for every head over different prompts. Use L16H25 Llama 2 as a concrete example. }
%     \item \sm{Title: Birth of Attention Sink in Large Language Models}
%     \item \tianyu{Title: Attention heads learn to have dormant phase: demystifying (attention sink; massive norm; value states) extreme values in LLMs}
% \end{itemize}

% \paragraph{Outline: }
% \begin{itemize}
%     \item Section 1: Intro and related work
%     \begin{itemize}
%         \item Introduction (TODO: DP)
%         \item Related work (TODO: SM? + DP)
%     \end{itemize}
%     \item Section 2: Case study as motivation for conjecture
%     \begin{itemize}
%         \item Notations (TODO: DP)
%         \item Preliminaries (what is a transformer, what is attention, etc) (TODO: DP)
%         \item Preliminaries part 2 (what are massive activations, what are massive tokens, what are attention sinks) --- point out the figure for Layer 16 Head 25, point out it's massive activation, massive token, attention sink properties (TODO: DP)
%         \item Llama2 Layer 16 Head 25: what do we observe about its behavior on Wiki vs coding? Use the best precision we can give in the time remaining  (TODO: DP)
%         \begin{itemize}
%             \item Two side-by-side figures of attention weights on this head on Wikipedia and Github
%             inputs (TODO: DP)
%             \item Same for logits (TODO for figure generation: DP, for detailed analysis: TG)
%         \end{itemize}
%     \end{itemize}
%     \item Section 3: Conjecture and evidence 
%     \begin{itemize}
%         \item Describe dormant head conjecture in as precise language as possible (TODO: DP + TG?)
%         %\item Theoretical evidence: linear algebraic mechanism + empirical evidence: attention sinks + massive activation (TODO: DP + TG)
%         \begin{itemize}
%             \item Attention sink is nearly the only possible mechanism to keep head dormant on some inputs and active on others
%         \end{itemize}
%         \item Evidence 1: circuit in Llama2 which causes dormant head (TODO: TG)
%         \begin{itemize}
%             \item a flowchart (TG + DP)
%             \item some supporting findings: norm bar-plot of tokens? table of (mean, var) of attention logits on bos tokens and other tokens (some randomly selected tokens) 
%         \end{itemize}
        
%         \item Evidence 2: intervention study on Llama 2. Goals: show that our automated dormant head detection system is very effective with strong quantitative behavior connecting to qualitative observations, and then show that it finds many heads (TODO: DP)
%         \begin{itemize}
%             \item Graph all heads. x axis = max metric among 32 samples of Wikipedia + 32 samples of Github, y axis = min metric, top right = always dormant, bottom left = always active, etc. Red color for L16H25. (TODO: DP)
%             \item Display \# of heads detected on Wikipedia, Github, and Wikipedia+Github (TODO: DP; also include common crawl?)
%         \end{itemize}
%         \item Evidence 3: pretraining on simple tasks? (TODO: TG)
%         \begin{itemize}
%             \item Attention weights heatmap for the ``dormant copy'' experiment;
%             \item Training Dynamics of the ``dormant copy'' experiment;
%         \end{itemize}
%     \end{itemize}
%     \item Section 4: Discussions, implications on interpretability? (TODO: DP? + TG)
%     \begin{itemize}
%         \item Conjecture on the emergence of dormant heads during pretraing: task variety -> value states monosemanticity -> dormant mechanism (the supporting experiment is in appendix)
%         \item Conjecture on massive tokens and massive activations
%         \item Some parts of Circuit are not fully understood.
%         \item Contradicting observations of dormant conjecture: Relationship of dormant head to head irrelevant for task (i.e., zeroing out doesn't change PPL)?
%         \begin{itemize}
%             \item Table documenting the perplexity before and after zeroing out L16H25 on Wikipedia and Github
%             \item Table relating attention sink score to PPL difference when zeroing out; shows weak trend (\DP{TODO: need to do it for new metrics})
%         \end{itemize}
%     \end{itemize}
%     \item Section 5: Conclusion (TODO: DP)

%     \item Appendix:
%     \begin{itemize}
%         \item Supporting results for Evidence 1:
%         \begin{itemize}
%             \item An illustration figure to explain the method to find the circuit
%         \end{itemize}
%         \item Supporting results for Evidence 2:
%         \begin{itemize}
%             \item Include plots for 32 samples on Wiki/Github for the given special head L16H25
%             \item Ablation on the different dormant head token score mechanism + dormant head detection metric --- lots of figures, pretty convincing that these choices are fairly robust
%         \end{itemize}
%         \item Supporting results for Evidence 3:
%         \begin{itemize}
%             \item Ablations: Biette's setting;
%             \item Ablations part2: another one;
%             \item Interpolating between dormant copy and dormant markov
%             \item Massive tokens
%         \end{itemize}
%     \end{itemize}
%     \item REMEMBER LLAMA3 EXPS
% \end{itemize}

% \paragraph{New outline: }
% \begin{itemize}
%     \item Section 1: Intro and related work
%     \begin{itemize}
%         \item Introduction (TODO: DP)
%         \item Related work (TODO: SM + DP)
%     \end{itemize}
%     \item Section 2: Case study as motivation for investigation
%     \begin{itemize}
%         \item Notations (TODO: DP)
%         \item Preliminaries (what is a transformer, what is attention, etc) (TODO: DP)
%         \item Preliminaries part 2 (what are massive activations, what are massive tokens, what are attention sinks (TODO: DP)
%         \item  \sm{Our preliminary findings: The observed sink heads are not always dormant. Every head has a dormant phase and an active phase. In the active phase, the head transports information from previous tokens to the current one. In the dormant phase, the head behaves as if it is constantly biased. Plot the histogram of dormant metric for every head over different prompts. }
%         \item An example of the above point: Llama2 Layer 16 Head 25: what do we observe about its behavior on Wiki vs coding? Use the best precision we can give in the time remaining  (TODO: DP)
%         \begin{itemize}
%             \item Two side-by-side figures of attention weights on this head on Wikipedia and Github
%             inputs (TODO: DP)
%             \item Same for logits (TODO for figure generation: DP, for detailed analysis: TG)
%         \end{itemize}
%     \end{itemize}
%     \item Section 3: Static mechanism of attention sink, small value state, and massive norm. 
%     \begin{itemize}
%     \item Mechanism in Llama 2. 
%     \item Mechanism in Llama 3.1. 
%     \item Pretraining of Bigram-Backcopy task. One-layer TF demonstrates the attention sink and small value state phenomena. Three-layer TF demonstrates the massive norm phenomenon. 
%     \end{itemize}
%     \item Section 4: Dynamical mechanism of attention sink, small value state, and massive norm. 
%     \begin{itemize}
%     \item Statement of the mechanism: For any attention head with a certain prompt, if the value vector of any seen token is not useful in predicting the next token, the gradient dynamics, together with the softmax mechanism, will push the attention weights to the token with a small value vector. For tokens that are non-useful in predicting the next token in all prompts, since their attention weights are large, gradient dynamics will push down their value vector norm. So, large attention weights and small value vector norms reinforce each other, making such tokens sink tokens. Gradient dynamics favors pushing early tokens to be sink tokens. \sm{How to state the mechanism of the massive norm? }
%     \item Experimental evidence in BBM. (ReLU attention does not exhibit the behavior. ) 
%     \item Theoretical explanation in BBM. 
%     \item Experimental evidence in the pre-training checkpoint of Pythia. 
%     \end{itemize}
%     \item Section 5: Conclusion (TODO: DP)
% \end{itemize}

% \paragraph{New outline-copy: }
% \begin{itemize}
%     \item Section 1: Intro and related work
%     \begin{itemize}
%         \item Introduction (TODO: DP)
%         \item Related work (TODO: SM + DP)
%         \item Notations (TODO: DP)
%         \item Preliminaries (what is a transformer, what is attention, etc) (TODO: DP)
%         \item Preliminaries part 2 (what are massive activations, what are massive tokens, what are attention sinks (TODO: DP
%     \end{itemize}
%     \item Section 2: State our ``conjecture'' and show all experiments on LLMs.
    
% )
% \begin{itemize}
%         \item  \sm{Our preliminary findings: The observed sink heads are not always dormant. Every head has a dormant phase and an active phase. In the active phase, the head transports information from previous tokens to the current one. In the dormant phase, the head behaves as if it is constantly biased. Plot the histogram of dormant metric for every head over different prompts. }
%         \item An example of the above point: Llama2 Layer 16 Head 25: what do we observe about its behavior on Wiki vs coding? Use the best precision we can give in the time remaining  (TODO: DP)
%         \begin{itemize}
%             \item Two side-by-side figures of attention weights on this head on Wikipedia and Github
%             inputs (TODO: DP)
%             \item Same for logits (TODO for figure generation: DP, for detailed analysis: TG)
%         \end{itemize}
%     \item Mechanism in Llama 2. 
%     \item Mechanism in Llama 3.1. 
%     \item Experimental evidence in the pre-training checkpoint of Pythia. 
%     \end{itemize}
%     \item Section 3: Controlled experiments. 
%     \begin{itemize}
%     \item Pretraining of Bigram-Backcopy task. One-layer TF demonstrates the attention sink and small value state phenomena. Three-layer TF demonstrates the massive norm phenomenon. 
%     \item dynamics
%     \item (the importance of value states meaning)
%     \end{itemize}
%     \item Section 4: Dynamical mechanism of attention sink, small value state, and massive norm. 
%     \begin{itemize}
%     \item Theoretical explanation in BBM. (motivated by the results in Section 3)
%     \item (Statement of the mechanism): For any attention head with a certain prompt, if the value vector of any seen token is not useful in predicting the next token ({\color{red} the value vectors for seen tokens are useful for a different task}), the gradient dynamics, together with the softmax mechanism, will push the attention weights to the token with a small value vector. For tokens that are non-useful in predicting the next token in all prompts, since their attention weights are large, gradient dynamics will push down their value vector norm. So, large attention weights and small value vector norms reinforce each other, making such tokens sink tokens. Gradient dynamics favors pushing early tokens to be sink tokens. \sm{How to state the mechanism of the massive norm? }
%     \item massive norm: (1. related to attention sink; 2. the influence function is constant; 3. the Adam update is constant.)
%     \item (with our theory, we predict some experimental results): Show more experimental evidence in BBM. (ReLU attention does not exhibit the behavior; Simplified model shows similar dynamics (+value state, +massive norm); SGD eliminates the massive norms. )
    
    
%     \end{itemize}
%     \item Section 5: Conclusion (TODO: DP)
% \end{itemize}

Some token is a $\{$attention sink, value-state drain, residual-state peak$\}$. 

Some token has $\{$dominant attention score, small value state, massive residual state$\}$. 

"Outlier phenomena" vs "Extreme-value phenomena" vs "Extreme-token phenomena" vs "Sink Phenomena". 

"Active phase and dormant phase", "Active phase and idle phase". 

Mechanism: "active-dormant mechanism", "active-idle mechanism", "switching mechanism". 

Dynamical mechanism: "Cyclic-Reinforcement Mechanism", "Mutual Reinforcement Mechanism"


\paragraph{NEW New outline-copy (based on Tianyu's Slack proposal): }
\begin{itemize}
    \item Section 1: Intro and related work
    \begin{itemize}
        \item Introduction (TODO: DP)
        \item Related work (TODO: SM + DP)
        \item Notations (TODO: DP)
        \item Preliminaries (what is a transformer, what is attention, etc) (TODO: DP)
        \item Preliminaries part 2 (what are massive activations, what are massive tokens, what are attention sinks (TODO: DP
    \end{itemize}

    \item Section 2: Bigram-Backcopy task to isolate attention sink phenomenon. Statics and Dynamics.
    \begin{itemize}
    \item Motivate Bigram-Backcopy task. The optimal implementation should result in a ``controlled'' attention sink.
    \item Theoretical results of training dynamics in bigram-backcopy task.
    \item Empirical results of pretraining in BB task.
    \begin{itemize}
        \item Statics. One-layer TF demonstrates the attention sink and small value state phenomena. Three-layer TF demonstrates the massive norm phenomenon. 
        \item Circuit analysis and dynamics. Statement of the mechanism of attention sink in BB task: For any attention head with a certain prompt, if the value vector of any seen token is not useful in predicting the next token ({\color{red} the value vectors for seen tokens are useful for a different task}), the gradient dynamics, together with the softmax mechanism, will push the attention weights to the token with a small value vector. For tokens that are non-useful in predicting the next token in all prompts, since their attention weights are large, gradient dynamics will push down their value vector norm. So, large attention weights and small value vector norms reinforce each other, making such tokens sink tokens. Gradient dynamics favors pushing early tokens to be sink tokens. \sm{How to state the mechanism of the massive norm? } 
        \item massive norm: (1. related to attention sink; 2. the influence function is constant; 3. the Adam update is constant.) When there are multiple layers (>=3), the output of the first layer (both attn and mlp) facilitates the formation of attention sink in the upper layers (denote this output as $\boldsymbol{m}$)-> the scale of the $\nabla_{\text{Params in layer 0}} \ltwo{\boldsymbol{m}}$ remains constant -> due to the layer norm in upper layers, the norm of the projection of $\nabla_{\text{Params in layer 0}} \text{Loss} $ onto the direction of $\nabla_{\text{Params in layer 0}} \ltwo{\boldsymbol{m}}$ shrinks quickly. -> due to Adam, the small gradients lead to constant update. \DP{Check this in OLMO...}
        
        \item Additional predictions from this theoretical understanding. Show more experimental evidence in BBM. (ReLU attention does not exhibit the behavior; Simplified model shows similar dynamics (+value state, +massive norm); SGD eliminates the massive norms. )
        \item \DP{Major point: the predictions made in this section NEED to transfer to LLMs.}
    \end{itemize}
    \end{itemize}

    \item Section 3: Show that predictions from BB task translate to LLMs.
    \begin{itemize}
        \item  \sm{Our preliminary findings: The observed sink heads are not always dormant. Every head has a dormant phase and an active phase. In the active phase, the head transports information from previous tokens to the current one. In the dormant phase, the head behaves as if it is constantly biased. Plot the histogram of dormant metric for every head over different prompts. }
        \item An example of the above point: Llama2 Layer 16 Head 25: what do we observe about its behavior on Wiki vs coding? Use the best precision we can give in the time remaining  (TODO: DP) \DP{Characterize dormant vs active phase in Llama 2 L16H25}
        \begin{itemize}
            \item Two side-by-side figures of attention weights on this head on Wikipedia and Github
            inputs (TODO: DP)
            \item Same for logits (TODO for figure generation: DP, for detailed analysis: TG)
        \end{itemize}
    \item Mechanism in Llama 2. 
    \item Mechanism in Llama 3.1. \DP{this is substantially easier; the main point is to note that the mechanism presents differently with multiple layers, but the idea carries through.}
    \item Experimental evidence in the pre-training checkpoint of OLMo. \DP{all dynamics results: value state norms, attention weights, and norms of tokens.}
    \end{itemize}
    \item Section 4: Conclusion (TODO: DP)
\end{itemize}


% \begin{itemize}
% \item Prelim, report existing findings.
% \item Linear algebraic mechanism
% \begin{itemize}
% \item Attention concentration (correlation, not massive norm), value anti-concentration.
% \item Birth of sink tokens: mechanism of MLP1, effect of Rope, ...
% \end{itemize}
% \item Dormant head hypothesis
% \begin{itemize}
% \item Dormant head in LlaMa2: L16H25.~\yub{Need a bunch of control experiments.}~\yub{Ideally, find other dormant heads, say still use RedPajama dataset to identify.}
% \item \yub{something else?} (Find more signals for dormant head in LlaMa2.)
% \item \yub{For \emph{every} attention sink head (can use some heuristic method to define what an attention sink head is), can we find sentence to activate it and sentence to deactivate it?}
% \item \yub{Theory? e.g. approximation results for specific kinds of heads with/without attention sink (or BOS token). }
% \item \yub{Any attention head can be modified to a dormant head, which is the same head on some input sequence, and deactivated on some other input sequence (with some separation from the original inputs).}
% \end{itemize}
% \item Pretraining with small transformers and synthetic data
% \begin{itemize}
% \item Dormant head phenomenon in Bietti's experiment
% \begin{itemize}
% \item Attention concentration -> massive norm -> massive activation.~\yub{Any experiments that show this quantitatively?}
% % ~\yub{GPT2 does not use RoPE, so do not expect massive activation. But massive activation paper they report massive activation for GPT2??? LayerNorm also makes standard coordinates special.}
% \end{itemize}
% \item 50-50 mixture of pure Markov transition prediction and pure induction head phenomenon.~\yub{Intuition: In RepICL where every sequence requires the same task (Rep + ridge regression), there is no attention sink. }
% \item \yub{TODO: Try full sequence copying after some special trigger token.}
% \item 50-50 mixture of any two tasks. Can get you more deactivated heads / attention sink.
% \item \yub{Try ReLU transformer on Bietti's experiment.}
% \end{itemize}
% \item Qualitative difference between LlaMa2 and LlaMa3?
% \end{itemize}

% \section*{TODOs}

% \begin{itemize}
%     % \item Conjecture: Where attention sink appears $\approx$ that layer is not very important, does some simple functional. Can we characterize that functional in function space?
%     \item Attention sink $\equiv$ bias (added after QKV)?
%     \begin{align*}
%         \bh_i' = \bh_i + \sum_{j=1}^i \softmax\paren{ (\<\bq_i, \bk_j\>)_{j=1}^i }_j \bv_j \approx \bh_i + \sum_{j=2}^i \softmax\paren{ (\<\bq_i, \bk_j\>)_{j=1}^i }_j \bv_j + \bbb
%     \end{align*}
%     Conjecture: Training an architecture with bias, can alleviate all the unbalancedness, and get rid of the streaming LLM problem.

%     \item Training dynamics of GPT2?
%     \begin{itemize}
%         \item Plot the gradient.
%     \end{itemize}
% \end{itemize}
